BanditPAM: Almost Linear Time $k$-Medoids Clustering via Multi-Armed Bandits

Clustering is a ubiquitous task in data science. Compared to the commonly used $k$-means clustering, $k$-medoids clustering requires the cluster centers to be actual data points and support arbitrary distance metrics, which permits greater interpretability and the clustering of structured objects. Current state-of-the-art $k$-medoids clustering algorithms, such as Partitioning Around Medoids (PAM), are iterative and are quadratic in the dataset size $n$ for each iteration, being prohibitively expensive for large datasets. We propose BanditPAM, a randomized algorithm inspired by techniques from multi-armed bandits, that reduces the complexity of each PAM iteration from $O(n^2)$ to $O(n \log n)$ and returns the same results with high probability, under assumptions on the data that often hold in practice. As such, BanditPAM matches state-of-the-art clustering loss while reaching solutions much faster. We empirically validate our results on several large real-world datasets, including a coding exercise submissions dataset, the 10x Genomics 68k PBMC single-cell RNA sequencing dataset, and the MNIST handwritten digits dataset. In these experiments, we observe that BanditPAM returns the same results as state-of-the-art PAM-like algorithms up to 4x faster while performing up to 200x fewer distance computations. The improvements demonstrated by BanditPAM enable $k$-medoids clustering on a wide range of applications, including identifying cell types in large-scale single-cell data and providing scalable feedback for students learning computer science online. We also release highly optimized Python and C++ implementations of our algorithm.

==> old/algorithm06-02.tex <==
\section{Algorithm}
\label{algo}

\begin{algorithm}[t]
\caption{\texttt{UltraPAM\_BUILD($X, k, d, batch\_size$):} 
%\Comment{Dataset $X$ of size $N$, number of medoids $k_{max}$, distance function $d$} 
\label{alg:ultrapam-build}}
\begin{algorithmic}[1]
\For{$l = 1, 2, ..., k$}
    \State $\mathcal{M} = \emptyset$
    \State $arms \leftarrow [n]$
    \State $T \leftarrow (0, \dots, 0)$ \Comment{Number of times each arm has been pulled}
    \State $B, M, U = (-\infty, \dots, -\infty), (0, 0, 0), (\infty, \dots, \infty)$ \Comment{Initial means and confidence bounds}
    \State Draw a sample of $batch\_size$ reference points, $\{x_{\rm ref}\}$, uniformly at random
    \ForAll{arms $i$}
    \State $\sigma_i$ \leftarrow STDEV($\{\Delta L_{x_i}(x_{\rm ref})\}$) \Comment{Estimate $\sigma_i$} for each arm
    \EndFor
    
    \While{$arms \neq \emptyset$}
        % Question: should we even include this case in the pseudocode?
        \ForAll{arms $i$ where $T_i + batch\_size \geq N$} \State Compute $\sum_{j = 1}^N \Delta L_{x_i}(x_j)$ exactly \Comment Over all datapoints
        \State Set $B_i = M_i = U_i = \sum_{j = 1}^N \Delta L_{x_i}(x_j)$ \Comment Arm return is known exactly
        \EndFor
        \State Draw a new sample of $batch\_size$ reference points, $\{x_{\rm ref}\}$, uniformly at random
        \ForAll{arms $i$ where $T_i + batch\_size < N$}
        \State $M_i \leftarrow \frac{ T_iM_i + \sum_{x_{\rm ref}}\Delta L_{x_i}(x_{\rm ref})}{T_i + batch\_size}$ \Comment{Update running average}
        \State $T_i \leftarrow T_i + batch\_size$
        \State $C_i \leftarrow \sigma_i \sqrt{ \frac{ \log(\frac{1}{\delta}) } {T_i}}$
        \State $B_i \leftarrow M_i - C_i$, $U_i \leftarrow M_i + C_i$ \Comment{Update confidence interval}
        \EndFor

    \State $arms \leftarrow \{i : B_i \leq \min_i(U_i)\}$ \Comment{Arms to pull must overlap with lowest CI}
    \EndWhile
    \State Append $x_i$ to $\mathcal{M}$, where $i = \argmin_iB_i$
\EndFor
\State \textbf{return} $\mathcal{M}$
\end{algorithmic}
\end{algorithm}






\begin{algorithm}[t]
\caption{\texttt{UltraPAM\_SWAP($X, \mathcal{M}, d, batch\_size$):} 
%\Comment{Dataset $X$ of size $N$, number of medoids $k_{max}$, distance function $d$} 
\label{alg:ultrapam-swap}}
\begin{algorithmic}[1]
\Repeat
    \State $arms \leftarrow \mathcal{\mathcal{M} \times (\mathcal{X} \setminus \mathcal{M})}$ \Comment Arms are indexed by tuple $(m, o)$
    \State $T \leftarrow (0, \dots, 0)$ \Comment{Number of times each arm has been pulled}
    \State $B, M, U = (-\infty, \dots, -\infty), (0, 0, 0), (\infty, \dots, \infty)$ \Comment{Initial means and confidence bounds}
    \State Draw a sample of $batch\_size$ reference points, $\{x_{\rm ref}\}$, uniformly at random
    \ForAll{arms ${(m,o)}$}
    \State $\sigma_{(m,o)}$ \leftarrow STDEV($\{\Delta L_{(m, o)}(x_{\rm ref})\}$) \Comment{Estimate $\sigma_i$} for each arm
    \EndFor
    \While{$arms \neq \emptyset$}
        % Question: should we even include this case in the pseudocode?
        \ForAll{arms $(m, o)$ where $T_{(m,o)} + batch\_size \geq N$ } \State Compute $\sum_{j = 1}^N \Delta L_{(m, o)}(x_j)$ exactly
        \State Set $B_{(m, o)} = M_{(m, o)} = U_{(m, o)} = \sum_{j = 1}^N \Delta L_{(m, o)}(x_j)$
        \EndFor
        \State Draw a new sample of $batch\_size$ reference points, $\{x_{\rm ref}\}$, uniformly at random
        \ForAll{arms $(m, o)$ where $T_{(m,o)} + batch\_size < N$}
        \State $M_{(m, o)} \leftarrow \frac{ T_{(m, o)}M_{(m, o)} + \sum_{x_{\rm ref}}\Delta L_{(m, o)}(x_{\rm ref})}{T_{(m, o)} + batch\_size}$ \Comment{Update running mean}
        \State $C_{(m, o)} \leftarrow \sigma \sqrt{ \frac{ \log(\frac{1}{\delta}) } {T_i}}$
        \State $B_{(m, o)} \leftarrow M_{(m, o)} - C_{(m, o)}$ \Comment{Update LCB}
        \State $U_{(m, o)} \leftarrow M_{(m, o)} + C_{(m, o)}$ \Comment{Update UCB}
        \State $T_{(m, o)} \leftarrow T_{(m, o)} + batch\_size$
        \EndFor

    \State $arms \leftarrow \{(m, o) : L_{(m, o)} \leq \min_{(m, o)}U_{(m,o)}\}$ \Comment{Arms must overlap with lowest CI}
    \EndWhile
    \State Remove $m$ from $\mathcal{M}$ and add $o$ to $\mathcal{M}$ \Comment{Perform the best swap}
\Until{convergence}
\State \textbf{return} $\mathcal{M}$
\end{algorithmic}
\end{algorithm}


UltraPAM, shown in Algorithm 1, is an algorithm to $k$ medoids of a given dataset. It uses techniques from the MAB literature, specifically the Upper Confidence Bound (UCB) algorithm, to identify the same medoids as prior approaches, such as PAM and FastPAM, with high probability, while running in significantly less time. The algorithmic complexity of UltraPAM is $O(kNlogN)$ in the BUILD step and each SWAP step, compared to $O(kN^2)$ in the BUILD and each SWAP step of PAM and FastPAM. \martin{Include the success probability because this is an probabilistic algorithm.}

In the UltraPAM BUILD step, we intialize each medoid of the $k_{max}$ medoids one by one. 
At each step in the outer loop, our goal is to find the non-medoid for which choosing it as the new medoid would lower the total loss the most. Intuitively, conditioned on the prior $k - 1$ medoids \ilan{I don't like this use of the word conditioned}, we view the non-medoids as "arms" in the MAB framework. 
Pulling an arm corresponding to point $x_i$ corresponds to computing the change in Total Loss (Equation 1) that would be induced on a single reference point, $x_{\rm ref}$ \martin{$x_{\text{ref}}$} by choosing $x_i$ as the $k^{th}$ \martin{$k$th} medoid. 
Rather than computing this change in loss for every non-medoid candidate $x_i$ and every possible reference point $x_{\rm ref}$ as in PAM, we expend computation \textit{intelligently} \ilan{no need to italicize}. 
Specifically, we build confidence intervals for each $\Delta TD_i$ and only sample additional reference points $x_{\rm ref}$s for the most promising candidates, as determined by those with low confidence intervals for $\Delta TD_i$. 
Intuitively, we do not spend unnecessary computations and distance calculations for those points which have a very high corresponding$\Delta TD_i$; such points are not valuable to investigate as potential medoids. ${x_i}$ is assigned as the $k^{th}$ medoid if and only if its corresponding confidence interval $[\Delta TD_i - C_i(t), \Delta TD_i + C_i(t)]$ is both lower than and disjoint from any other confidence interval.

\ilan{
I feel like we already chatted about this in the past, but would it make sense to use the same $x_{\rm ref}$ for all candidate medoids in BUILD? 
I think that's a natural question that a reader may have when reading through the algorithm.
}


The UltraPAM SWAP step is similar to the BUILD step. 
\ilan{we probably shouldn't say that as the SWAP step is arguably more complicated, and we don't want to trivialize our contribution}
In the SWAP step, the algorithm attempts to identify the \textit{medoid-nonmedoid pair} $(x_m, x_i)$ for which removing $x_m$ as a medoid and assigning $x_i$ as a medoid would lower the total loss the most. Intuitively, each of the $k(N-k)$ such pairs $(x_m, x_i)$ are viewed as "arms", and pulling an arm corresponds to computing the change in total loss Equation 3 that would be induced for a single reference point $x_{\rm ref}$. As before, we build initial confidence intervals $[\Delta TD_{i,j} - C_{i,j}(t), \Delta TD_{i,j} + C_{i,j}(t)]$ for each medoid-nonmedoid pair (hence the two subscripts to $\Delta TD_{i,j}$ and $C_{i,j}(t)$, and continue to sample those that have "low" confidence intervals (specifically, those that overlap with the current lowest confidence interval). A SWAP is performed when a single confidence interval, corresponding to a specific medoid-nonmedoid pair $(x_m, x_i)$, is lower than and disjoint from all other confidence intervals; $x_m$ is then removed as a medoid and $x_i$ is designated a medoid. The SWAP step is iterated until convergence, when no more swaps can be performed to lower the total loss.

We also note a small point of potential confusion: though our algorithm is inspired by the \textit{Upper} Confidence Bound (UCB) algorithm from the MAB literature, in our setting we are attempting to find the \textit{lowest} confidence bound to find the operation (build or swap) which will lower our total loss the most.

Intuitively, UltraPAM only performs additional distance computations on the most promising points to assign as medoids in the BUILD step, and the most promising swaps to perform in the SWAP steps, thereby saving computation on unpromising candidates. In the following sections, we formalize this argument and provide theoretical guarantees under which UltraPAM will return the same results as PAM and FastPAM. We also experimentally validate our approach on several real-world datasets.

==> old/algorithm06-04.tex <==
% !TEX root = 0-main.tex

\section{\algnamenospace \label{sec:algo}}
At the core of the PAM algorithm is the $O(n^2)$ BUILD search \eqref{eqn:build-next-medoid}, which is repeated $k$ times for initialization and the $O(kn^2)$ SWAP search \eqref{eqn:next-swap}, which is repeated until convergence. 
We first show that both searches share a similar mathematical structure, and then show such a structure can be optimized efficiently using a bandit-based randomized algorithm, thus giving rise to \algnamenospace. 

Rewriting the BUILD search \eqref{eqn:build-next-medoid} and the SWAP search \eqref{eqn:next-swap} in terms of the change in total loss yields
\begin{align}
    \text{BUILD~search:~~~~}& \argmin_{x \in \mathcal{X} \setminus \mathcal{M}_{l}} \frac{1}{n} \sum_{j=1}^n \left[ \left(d(x, x_j) - \min_{m' \in \mathcal{M}_{l}} d(m', x_j) \right)  \wedge 0\right], \label{eqn:build_search}\\
    \text{SWAP~search:~~~~}& \argmin_{(m,x) \in \mathcal{M} \times (\mathcal{X} \setminus \mathcal{M}) } \frac{1}{n} \sum_{j=1}^n \left[ \left(d(x, x_j) - \min_{m' \in \mathcal{M}\setminus \{m\}} d(m', x_j) \right)\wedge 0\right].  \label{eqn:swap_search}
\end{align}
One may notice that the above two problems share the following similarities.
First, both are searching over a finite set of parameters, $n-l$ points for the BUILD search and $k(n-k)$ swaps for the SWAP search. 
Second, both objective functions have the form of an average of an $O(1)$ function evaluated over a finite set of reference points. 
Therefore, we can describe a shared structure between the two problems as:
\begin{align} \label{eqn:genetic_optimiation}
    \text{Shared Problem:~~~~} \argmin_{x \in \mathcal{S}_{\text{tar}} } \frac{1}{\vert \mathcal{S}_{\text{ref}} \vert } \sum_{x_j \in \mathcal{S}_{\text{ref}}} g_x(x_j), 
\end{align}
for target points $\mathcal{S}_{\text{tar}} $, reference points $\mathcal{S}_{\text{ref}}$, and an objective function $g_x(\cdot)$ that dependents on the target point $x$. Then both the BUILD search and the SWAP search can be written as instances of Problem \eqref{eqn:genetic_optimiation} with:
\begin{align}
    & \text{BUILD~search:~~} 
    \mathcal{S}_{\text{tar}}=\mathcal{X} \setminus \mathcal{M}_{l},~
    \mathcal{S}_{\text{ref}} = \mathcal{X},~
    g_x(x_j) = \left(d(x, x_j) - \min_{m' \in \mathcal{M}_{l}} d(m', x_j) \right)  \wedge 0, \label{eqn:build_instance}\\
    & \text{SWAP~search:~~} 
    \mathcal{S}_{\text{tar}}=\mathcal{M} \times (\mathcal{X} \setminus \mathcal{M}),~
    \mathcal{S}_{\text{ref}} = \mathcal{X},~
    g_x(x_j) =  \left(d(x, x_j) - \min_{m' \in \mathcal{M} \setminus \{m\}} d(m', x_j) \right)\wedge 0. \label{eqn:swap_instance}
\end{align}
\mo{Previous eqn spills into margin. acceptable?}
Crucially, in the SWAP search, each \textit{pair} of medoid-and-non-medoid points $(m,x)$ is treated as one target point in $\mathcal{S}_{\text{tar}}$ in this new formulation.


\subsection{Adaptive Search for Problem \eqref{eqn:genetic_optimiation}}
Recall that the computation of $g(x_j)$ is $O(1)$.
A naive method would need $O(\vert \mathcal{S}_{\text{tar}} \vert \vert \mathcal{S}_{\text{ref}} \vert)$ computations to solve Problem \eqref{eqn:genetic_optimiation}. 
However, as shown in previous works \cite{bagaria2018medoids,bagaria2018adaptive}, a randomized search would return the correct result with high confidence in $O( \vert \mathcal{S}_{\text{tar}}\vert \log  \vert \mathcal{S}_{\text{ref}} \vert)$ time, under certain assumptions.

Specifically, for each parameter $x$ in Problem \eqref{eqn:genetic_optimiation}, let $\mu_x = \frac{1}{\vert \mathcal{S}_{\text{ref}} \vert } \sum_{x_j \in \mathcal{S}_{\text{ref}}} g(x_j)$ denote its objective function. Computing $\mu_x$ takes $O(\vert \mathcal{S}_{\text{ref}} \vert)$, but we can instead estimate $\mu_x$ with fewer computations. Specifically, let $J_1,J_2,...,J_{n'}$ be 
\ilan{indices drawn uniformly and independently at random from $\{1,...,|\mathcal{S_{\text{ref}}}|\}$}
points uniformly and independently sampled with replacement from $\mathcal{S}_{\text{ref}}$. Then, $\mathbb{E}[g(x_{J_i})] = \mu_x$; $\mu_x$ can be estimated as $\hat{\mu}_x = \frac{1}{n'} \sum_{i=1}^{n'} g(x_{J_i})$; and $n'$ determines the estimation accuracy. 

Furthermore, if we change our goal to estimating the solution in Problem \eqref{eqn:genetic_optimiation} with high confidence, then we can choose to sample different points in $\mathcal{S}_{\text{tar}}$ with different accuracy. 
Intuitively, promising points with small values of $\mu_x$ should be estimated with high accuracy while less promising ones can be discarded without being evaluated on too many reference points. 
The specific adaptive estimation procedure is described in Algorithm \ref{alg:bandit_based_search}. 
It can be viewed as a batch version of the conventional UCB algorithm \cite{lai1985asymptotically,zhang2019adaptive} and is friendlier to implementation.

The algorithm uses the set $\mathcal{S}_{\text{solution}}$ to track all potential solutions to Problem \eqref{eqn:genetic_optimiation}; $\mathcal{S}_{\text{solution}}$ is initialized as the set of all target points $\mathcal{S}_{\text{tar}}$. In addition, for each potential solution $x\in \mathcal{S}_{\text{solution}}$, the algorithm maintains its mean objective estimate $\hat{\mu}_x$ as well as a confidence interval $C_x$; the latter depends on the exclusion probability $\delta$ as well as the dispersion parameter $\sigma_x$.

In each iteration, a new batch of reference points $\mathcal{S}_{\text{ref\_batch}}$ is evaluated for all potential solutions in $\mathcal{S}_{\text{solution}}$, making the estimates $\hat{\mu}_x$ and $C_x$ more accurate. 
Based on the current estimate, if a point's lower confidence bound $\hat{\mu}_x - C_x$ is still greater than the upper confidence bound of the most promising point $\min_{y}(\hat{\mu}_{y} + C_{y})$, we know it will not be the final solution and remove it from the set $\mathcal{S}_{\text{solution}}$. 

The iteration continues until there is only one point in $\mathcal{S}_{\text{solution}}$ or we have sampled more points than in the whole reference set; in the latter case, we know that the difference between the remaining points in $\mathcal{S}_{\text{solution}}$ become so subtle that an exact computation is more efficient. So we compute their objectives exactly and return the best point in the set. 

\begin{algorithm}[t]
\caption{\texttt{Adaptive-Search} ($\mathcal{S}_{\text{tar}}, \mathcal{S}_{\text{ref}}, g_x(\cdot), \batchsize$, $\delta$, $\sigma_x$): 
\label{alg:bandit_based_search}}
\begin{algorithmic}[1]
\State $\mathcal{S}_{\text{solution}} \leftarrow \mathcal{S}_{\text{tar}}$ \Comment{Set of potential solutions to Problem \eqref{eqn:genetic_optimiation}}
\State $n_{\text{used\_ref}} \gets 0$  \Comment{Number of reference points evaluated}
\State For all $x \in  \mathcal{S}_{\text{tar}}$, set $\hat{\mu}_x \leftarrow 0$, $C_x \leftarrow \infty$  \Comment{Initial mean and confidence interval for each arm}

\While{$n_{\text{used\_ref}} < \vert \mathcal{S}_{\text{ref}} \vert $ and $|\mathcal{S}_{\text{solution}}| > 1$} % and $C_y > 0$ for some arm $y$}
        \State Draw a batch of $\batchsize$ samples with replacement from reference $\mathcal{S}_{\text{ref\_batch}} \subset \mathcal{S}_{\text{ref}}$ 
        \ForAll{$x \in \mathcal{S}_{\text{solution}} $}
            \State $\hat{\mu}_x \leftarrow \frac{ n_{\text{used\_ref}} \hat{\mu}_x + \sum_{y \in \mathcal{S}_{\text{ref\_batch}}} g_x(y)}{n_{\text{used\_ref}} + \batchsize }$ \Comment{Update running mean}
            \State $C_x \gets \sigma_x \sqrt{  \frac{ 2 \log(\frac{1}{\delta}) } {n_{\text{used\_ref}} + \batchsize }}$
            \Comment{Update confidence interval}        
        \EndFor
    \State $\mathcal{S}_{\text{solution}} \leftarrow \{x : \hat{\mu}_x - C_x \leq \min_{y}(\hat{\mu}_{y} + C_{y})\}$ \Comment{Remove points that can no longer be solution}
    \State $n_{\text{used\_ref}} \leftarrow n_{\text{used\_ref}} + \batchsize$
\EndWhile
\If{$\vert \mathcal{S}_{\text{solution}} \vert$ = 1}
    \State \textbf{return} $x^* \in \mathcal{S}_{\text{solution}}$
\Else
    \State Compute the exact $\mu_x$ for all $x \in \mathcal{S}_{\text{solution}}$
    \State \textbf{return} $x^* = \argmin_{x \in \mathcal{S}_{\text{solution}}} \mu_x$
\EndIf
\end{algorithmic}
\end{algorithm}

\subsection{Algorithmic Details}
\label{subsec:algdetails}

% \martin{Mo, I think we can put all remaining details of \algname in this subsection. What do you think and could you help me add them?}

\algname uses Algorithm \ref{alg:bandit_based_search} in both the BUILD search and the SWAP search, with input parameters defined in \eqref{eqn:build_instance} and \eqref{eqn:swap_instance}. In practice, $\sigma_x$ is not known a priori. As such, we estimate $\sigma_x$, \ilan{for each $x \in |\mathcal{S}_{\text{tar}}|$}, from the data itself. In the first batch of sampled reference points in Algorithm \ref{alg:bandit_based_search}, we estimate each $\sigma_x$ as:

\begin{equation}
\label{eqn:sigma_est}
    \sigma_x = {\rm STD}_{y \in \mathcal{S}_{\text{ref\_batch}}}g_x(y)
\end{equation}

where ${\rm STD}$ denotes standard deviation. Intuitively, this allows for smaller confidence intervals in later iterations, especially in the BUILD step, when we expect the average arm returns to become smaller as we add more medoids (since we are taking the minimum over a larger set on the RHS of Equation \eqref{eqn:build-next-medoid}). We also allow for arm-dependent $\sigma_x$, as opposed to a fixed global $\sigma$, which allows for narrower confidence intervals for arms whose returns are heavily concentrated (e.g. distant outliers). 
Empirically, this results in significant speedups and results in fewer arms being computed exactly (Line 14 in Algorithm \ref{alg:bandit_based_search}). 
Allowing for arm-dependent $\sigma_x$ and re-estimating each $\sigma_x$ in each iteration also presents a difference between our approach and prior work {\bf \{citation\}}. Details about these techniques are discussed further in Section \ref{exps}. 


% We make the following additional changes to the vanilla version of Algorithm \ref{alg:bandit_based_search} to further improve speed. 

% The parameter $\sigma_x$ for the confidence intervals are estimated from data. Specifically, %\martin{Mo: could you add more information?}.
% We found that having different parameters for different steps of PAM will greatly improve speed. 
% We also found that the speed can be further improved by allowing a different parameter for different target points in $\mathcal{S}_{\text{tar}}$. 
% \martin{(As demonstrated in ...)}

Algorithm \ref{alg:bandit_based_search} can also be combined with the FastPAM1 optimization \cite{schubert2019faster} to further reduce the number of computations in each SWAP iteration. 
% to $O(n^2)$. \mo{O(n^2) is kind of unclear -- if we're omitting k, it's already O(n^2) before FP1. If we're not omitting k, we should include the dependence on k (still exists)}%\martin{Mo: could you add more information?}
For a given candidate swap $(m, o)$, we rewrite $g_{(m,o)}(x_j)$ from Equation \eqref{eqn:swap_instance} as:

\begin{equation}
    \label{eqn:fastpam1-trick}
    g_{m,o}(x_j) = \mathbbm{1}_{x_j \notin C_m}\min[d_1(x_j),d(o,x_j)] + \mathbbm{1}_{x_j \in C_m}\min[d_2(x_j), d(o, x_j)]
\end{equation}

where $C_m$ denotes the set of points whose closest medoid is $m$, $d_1(x_j)$ (respectively, $d_2(x_j)$) is the distance from $x_j$ to its nearest (respectively, \textit{second} nearest) medoid before the swap is performed. If we cache the values $d_1(x_j), d_2(x_j)$, and the cluster assignments $C_m$, then Equation \eqref{eqn:fastpam1-trick} no longer depends on $m$, instead depending only on $\mathbbm{1}_{x_j \in C_m}$, which is cached. This allows for an $O(k)$ speedup in each SWAP iteration.




% \clearpage
% UltraPAM, shown in Algorithm 1, is an algorithm to $k$ medoids of a given dataset. It uses techniques from the MAB literature, specifically the Upper Confidence Bound (UCB) algorithm, to identify the same medoids as prior approaches, such as PAM and FastPAM, with high probability, while running in significantly less time. The algorithmic complexity of UltraPAM is $O(kNlogN)$ in the BUILD step and each SWAP step, compared to $O(kN^2)$ in the BUILD and each SWAP step of PAM and FastPAM. \martin{Include the success probability because this is an probabilistic algorithm.}

% In the UltraPAM BUILD step, we intialize each medoid of the $k_{max}$ medoids one by one. 
% At each step in the outer loop, our goal is to find the non-medoid for which choosing it as the new medoid would lower the total loss the most. Intuitively, conditioned on the prior $k - 1$ medoids \ilan{I don't like this use of the word conditioned}, we view the non-medoids as "arms" in the MAB framework. 
% Pulling an arm corresponding to point $x_i$ corresponds to computing the change in Total Loss (Equation 1) that would be induced on a single reference point, $x_{\rm ref}$ \martin{$x_{\text{ref}}$} by choosing $x_i$ as the $k^{th}$ \martin{$k$th} medoid. 
% Rather than computing this change in loss for every non-medoid candidate $x_i$ and every possible reference point $x_{\rm ref}$ as in PAM, we expend computation \textit{intelligently} \ilan{no need to italicize}. 
% Specifically, we build confidence intervals for each $\Delta TD_i$ and only sample additional reference points $x_{\rm ref}$s for the most promising candidates, as determined by those with low confidence intervals for $\Delta TD_i$. 
% Intuitively, we do not spend unnecessary computations and distance calculations for those points which have a very high corresponding$\Delta TD_i$; such points are not valuable to investigate as potential medoids. ${x_i}$ is assigned as the $k^{th}$ medoid if and only if its corresponding confidence interval $[\Delta TD_i - C_i(t), \Delta TD_i + C_i(t)]$ is both lower than and disjoint from any other confidence interval.

% \ilan{
% I feel like we already chatted about this in the past, but would it make sense to use the same $x_{\rm ref}$ for all candidate medoids in BUILD? 
% I think that's a natural question that a reader may have when reading through the algorithm.
% }


% The UltraPAM SWAP step is similar to the BUILD step. 
% \ilan{we probably shouldn't say that as the SWAP step is arguably more complicated, and we don't want to trivialize our contribution}
% In the SWAP step, the algorithm attempts to identify the \textit{medoid-nonmedoid pair} $(x_m, x_i)$ for which removing $x_m$ as a medoid and assigning $x_i$ as a medoid would lower the total loss the most. Intuitively, each of the $k(N-k)$ such pairs $(x_m, x_i)$ are viewed as "arms", and pulling an arm corresponds to computing the change in total loss Equation 3 that would be induced for a single reference point $x_{\rm ref}$. As before, we build initial confidence intervals $[\Delta TD_{i,j} - C_{i,j}(t), \Delta TD_{i,j} + C_{i,j}(t)]$ for each medoid-nonmedoid pair (hence the two subscripts to $\Delta TD_{i,j}$ and $C_{i,j}(t)$, and continue to sample those that have "low" confidence intervals (specifically, those that overlap with the current lowest confidence interval). A SWAP is performed when a single confidence interval, corresponding to a specific medoid-nonmedoid pair $(x_m, x_i)$, is lower than and disjoint from all other confidence intervals; $x_m$ is then removed as a medoid and $x_i$ is designated a medoid. The SWAP step is iterated until convergence, when no more swaps can be performed to lower the total loss.

% We also note a small point of potential confusion: though our algorithm is inspired by the \textit{Upper} Confidence Bound (UCB) algorithm from the MAB literature, in our setting we are attempting to find the \textit{lowest} confidence bound to find the operation (build or swap) which will lower our total loss the most.

% Intuitively, UltraPAM only performs additional distance computations on the most promising points to assign as medoids in the BUILD step, and the most promising swaps to perform in the SWAP steps, thereby saving computation on unpromising candidates. In the following sections, we formalize this argument and provide theoretical guarantees under which UltraPAM will return the same results as PAM and FastPAM. We also experimentally validate our approach on several real-world datasets.


% \begin{algorithm}[t]
% \caption{\texttt{\algnamenospace.BUILD($X, k, d, batch\_size$):} 
% %\Comment{Dataset $X$ of size $N$, number of medoids $k_{max}$, distance function $d$} 
% \label{alg:ultrapam-build}}
% \begin{algorithmic}[1]
% \For{$l = 1, 2, ..., k$}
%     \State $\mathcal{M} = \emptyset$
%     \State $arms \leftarrow [n]$
%     \State $T \leftarrow (0, \dots, 0)$ \Comment{Number of times each arm has been pulled}
%     \State $B, M, U = (-\infty, \dots, -\infty), (0, 0, 0), (\infty, \dots, \infty)$ \Comment{Initial means and confidence bounds}
%     \State Draw a sample of $batch\_size$ reference points, $\{x_{\rm ref}\}$, uniformly at random
%     \ForAll{arms $i$}
%     \State $\sigma_i$ $\leftarrow$ STDEV($\{\Delta L_{x_i}(x_{\rm ref})\}$) \Comment{Estimate $\sigma_i$} for each arm
%     \EndFor
    
%     \While{$arms \neq \emptyset$}
%         % Question: should we even include this case in the pseudocode?
%         \ForAll{arms $i$ where $T_i + batch\_size \geq N$} \State Compute $\sum_{j = 1}^N \Delta L_{x_i}(x_j)$ exactly \Comment Over all datapoints
%         \State Set $B_i = M_i = U_i = \sum_{j = 1}^N \Delta L_{x_i}(x_j)$ \Comment Arm return is known exactly
%         \EndFor
%         \State Draw a new sample of $batch\_size$ reference points, $\{x_{\rm ref}\}$, uniformly at random
%         \ForAll{arms $i$ where $T_i + batch\_size < N$}
%         \State $M_i \leftarrow \frac{ T_iM_i + \sum_{x_{\rm ref}}\Delta L_{x_i}(x_{\rm ref})}{T_i + batch\_size}$ \Comment{Update running average}
%         \State $T_i \leftarrow T_i + batch\_size$
%         \State $C_i \leftarrow \sigma_i \sqrt{ \frac{ \log(\frac{1}{\delta}) } {T_i}}$
%         \State $B_i \leftarrow M_i - C_i$, $U_i \leftarrow M_i + C_i$ \Comment{Update confidence interval}
%         \EndFor

%     \State $arms \leftarrow \{i : B_i \leq \min_i(U_i)\}$ \Comment{Arms to pull must overlap with lowest CI}
%     \EndWhile
%     \State Append $x_i$ to $\mathcal{M}$, where $i = \argmin_iB_i$
% \EndFor
% \State \textbf{return} $\mathcal{M}$
% \end{algorithmic}
% \end{algorithm}

% \begin{algorithm}[t]
% \caption{\texttt{\algnamenospace.SWAP($X, \mathcal{M}, d, batch\_size$):} 
% %\Comment{Dataset $X$ of size $N$, number of medoids $k_{max}$, distance function $d$} 
% \label{alg:ultrapam-swap}}
% \begin{algorithmic}[1]
% \Repeat
%     \State $arms \leftarrow \mathcal{\mathcal{M} \times (\mathcal{X} \setminus \mathcal{M})}$ \Comment Arms are indexed by tuple $(m, o)$
%     \State $T \leftarrow (0, \dots, 0)$ \Comment{Number of times each arm has been pulled}
%     \State $B, M, U = (-\infty, \dots, -\infty), (0, 0, 0), (\infty, \dots, \infty)$ \Comment{Initial means and confidence bounds}
%     \State Draw a sample of $batch\_size$ reference points, $\{x_{\rm ref}\}$, uniformly at random
%     \ForAll{arms ${(m,o)}$}
%     \State $\sigma_{(m,o)}$ $\leftarrow$ STDEV($\{\Delta L_{(m, o)}(x_{\rm ref})\}$) \Comment{Estimate $\sigma_i$} for each arm
%     \EndFor
%     \While{$arms \neq \emptyset$}
%         % Question: should we even include this case in the pseudocode?
%         \ForAll{arms $(m, o)$ where $T_{(m,o)} + batch\_size \geq N$ } \State Compute $\sum_{j = 1}^N \Delta L_{(m, o)}(x_j)$ exactly
%         \State Set $B_{(m, o)} = M_{(m, o)} = U_{(m, o)} = \sum_{j = 1}^N \Delta L_{(m, o)}(x_j)$
%         \EndFor
%         \State Draw a new sample of $batch\_size$ reference points, $\{x_{\rm ref}\}$, uniformly at random
%         \ForAll{arms $(m, o)$ where $T_{(m,o)} + batch\_size < N$}
%         \State $M_{(m, o)} \leftarrow \frac{ T_{(m, o)}M_{(m, o)} + \sum_{x_{\rm ref}}\Delta L_{(m, o)}(x_{\rm ref})}{T_{(m, o)} + batch\_size}$ \Comment{Update running mean}
%         \State $C_{(m, o)} \leftarrow \sigma \sqrt{ \frac{ \log(\frac{1}{\delta}) } {T_i}}$
%         \State $B_{(m, o)} \leftarrow M_{(m, o)} - C_{(m, o)}$ \Comment{Update LCB}
%         \State $U_{(m, o)} \leftarrow M_{(m, o)} + C_{(m, o)}$ \Comment{Update UCB}
%         \State $T_{(m, o)} \leftarrow T_{(m, o)} + batch\_size$
%         \EndFor

%     \State $arms \leftarrow \{(m, o) : L_{(m, o)} \leq \min_{(m, o)}U_{(m,o)}\}$ \Comment{Arms must overlap with lowest CI}
%     \EndWhile
%     \State Remove $m$ from $\mathcal{M}$ and add $o$ to $\mathcal{M}$ \Comment{Perform the best swap}
% \Until{convergence}
% \State \textbf{return} $\mathcal{M}$
% \end{algorithmic}
% \end{algorithm}

==> old/exp06-04.tex <==
% !TEX root = 0-main.tex

\begin{table}
  \caption{Description of Datasets}
  \label{table:datasets}
  \centering
  \begin{tabular}{llll}
    \toprule
    Name     & Size ($n_{\text{max}}$) & Distance Metric & Dimensionality \\
    \midrule
    MNIST & 70000  & $l_2$, cosine distance  & 784     \\
    % MNIST & 70000  & cosine distance & 784     \\
    scRNA-seq & 40000  & $l_1$ & 10170     \\
    % scRNA-PCA & 40000  & $L2$ & 10     \\
    Hour Of Code \#4 & 3,360  & Tree edit distance & $\infty$     \\
    \bottomrule
  \end{tabular}
\end{table}


\section{Datasets and Experiments \label{sec:exps}}

% \subsection{Datasets}

We run experiments on three real-world datasets to validate the expected behavior of \algnamenospace: the MNIST hand-written digits dataset \cite{}, the 10x Genomics 68k PBMCs scRNA-seq dataset \cite{}, and the Code.org Hour Of Code \#4 (HOC4) dataset, all of which are publicly available. The datasets, and their corresponding distance metrics, are summarized in Table \ref{table:datasets}. \martin{add references}

The MNIST dataset \{citation\} consists of 70,000 black-and-white images of handwritten digits, where each digit is represented as a 784 dimensional vector. Popular distance metrics for the MNIST dataset include $l_2$ distance and cosine distance \{citation\}, both of which we consider here.
The scRNA-seq dataset contains the gene expression levels of 10170 different genes in each of 40000 cells sequenced in a single individual.
%; scRNA-PCA is the same dataset where each datapoint is projected onto the top 10 principal components of the scRNA-seq dataset. 
Prior work \{citation\} has often processed scRNA-seq datasets with $l_1$ distance. Finally, the Hour of Code \#4 dataset from Code.org \{citation\} is a publicly available consisting of 3360 unique solutions to a block-based programming exercise on Code.org. Solutions to the programming exercise are represented as abstract syntax trees (ASTs), and tree edit distance measures the distance between solutions. % Put an example of the trees here?

\subsection{Experiments and results}
We first provide demonstrate that \algname finds solutions of comparable quality to state-of-the-art algorithms such as PAM and FastPAM, almost always matching PAM's results exactly.
We then show that \algname scales roughly linearly with the dataset size. We further show that this scaling behavior is consistent even when choosing alternative distance metrics or increasing the number of medoids $k$. 

\textit{Remark:} In all experiments, the error probability $\delta$ is set to $\delta = \frac{1}{1000\vert \mathcal{S}_{\text{tar}} \vert}$ in Algorithm \ref{alg:bandit_based_search}. Empirically, this setting of $\delta$ is low enough that \algname recovers the same results in PAM in almost all cases.%, while still demonstrating the expected $O(\frac{n}{\log n})$ speedup.

% In all plots, points are plotted on a log-log scale. individual points represent different random samples of size $n$ drawn from the dataset (if $n = n_{\text{max}}$, the points are only shuffled between runs). Jitter has been added to the x-coordinates for clarity, and a line of best fit has also been overlaid.

\begin{figure}[h!]
    \centering
    \includegraphics[scale=0.5]{./figures/loss_plot.pdf}
    \caption{Final clustering loss of various $k$-medoids algorithms, normalized to the loss of PAM, for different random subsets of size $n$ of MNIST with $k = 5$. Error bars represent 95\% confidence intervals, where the midpoint is the mean over 10 different subsamples. Due to its inherent randomness, FastPAM occassionally finds better solutions than PAM but always requires $O(n^2)$ distance computations.} 
    \label{fig:losses}
\end{figure}

\subsubsection{Clustering/loss quality}
\label{subsec:loss}
%Baselines: PAM, CLARANS/CLARA, FastPAM, Voronoi Iteration
%The results from section \ref{Nscaling} show that each substep \algname scales almost linearly in dataset size. %Naturally, one might ask if there is a concession in final clustering quality that must be made for the $O(n/\log n)$ speedup of \algname. 

Figure \ref{fig:losses} shows the losses of \algname and three other baselines (FastPAM, CLARANS, and Voronoi Iteration) normalized to the loss of PAM for various random subsets of MNIST. We observe that \algname finds solutions of equivalent quality to PAM, as does FastPAM, and that these solutions are better than the other baselines. Indeed, in 59 of the 60 experiments, \algname tracks the exact optimization path and returns the exact same results as PAM; the single discrepancy arises in a single SWAP iteration of several hundred, which is in line with our choice of $\delta$.

\mo{Need to describe hyperparameters for CLARANS?}

\subsubsection{Scaling with $n$}
\label{subsec:scaling}

\begin{figure}[ht]
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=\linewidth]{./figures/MNIST-cosine-k5.pdf}  
  %\caption{Put your sub-caption here}
  \label{fig:scaling1}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=\linewidth]{./figures/SCRNA-L1-k5.pdf}   
  %\caption{Put your sub-caption here}
  \label{fig:scaling2}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=\linewidth]{./figures/HOC4-tree-k2.pdf}   
  %\caption{Put your sub-caption here}
  \label{fig:scaling3}
\end{subfigure}
\caption{Average number of distance calls per iteration vs $n$, for MNIST and cosine distance (left), scRNA-seq and $l_1$ distance (middle), and HOC4 and tree edit distance (right), on a log-log scale. Lines of best fit (black) are plotted, as are reference lines demonstrating the expected scaling of PAM (red).}
\label{fig:scaling}
\end{figure}

%When assessing the scaling of \algnamenospace, we treat the entire BUILD step as a single SWAP iteration. Indeed, the entire BUILD procedure for the $k$-medoids problem on dataset $\mathcal{X}$ can be reduced to a single SWAP iteration for the $k+1$-medoids problem on the dataset $\mathcal{X}$ augmented with $k+1$ equal points infinitely far away from $\mathcal{X}$.


Figure \ref{fig:scaling} shows the scaling of the average number of distance calls per iteration (BUILD subroutine or SWAP step) of \algname with $n$ on a log-log scale for three dataset and metric pairs: MNIST and cosine distance, scRNA-seq and $l_1$ distance, HOC4 and tree edit distance. The slopes of the lines of best fit (1.018, 0.899, and 1.046) suggest that \algname scales roughly linear in $n$ for all three datasets.

\mo{Can we somehow make this more clear that the *whole* build step is treated on the same footing as a single SWAP step? See comments in latex above previous paragraph}


\subsubsection{Different distance metrics and increasing $k$}
\label{subsec:mods}

\begin{figure}[ht]
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{./figures/MNIST-L2-k5.pdf}  
  \label{fig:mods1}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{./figures/MNIST-L2-k10.pdf}   
  \label{fig:mods2}
\end{subfigure}
\caption{Average number of distance calls per iteration vs $n$, for MNIST and $l_2$ distance with $k=5$ (left) and $k=10$ (right) on a log-log scale. Lines of best fit (black) are plotted, as are reference lines demonstrating the expected scaling of PAM (red).}
\label{fig:mods}
\end{figure}

% Naturally, one might ask if \algname only demonstrates the expected speedup for a particular choice of metric for a given dataset. Figure \ref{fig:fig1} shows the scaling of the average number of distance calls in the BUILD step (Algorithm 1) and SWAP step (Algorithm 2) of \algname with $n$ for the MNIST dataset, but using cosine distance instead of $l_2$. \algname still runs in near-linear time; the slopes of the lines of best fit is 1.2 in BUILD and 1.1 in SWAP. These results suggest the algorithmic speedup of \algname is not dependence on the choice of distance metric used for a given dataset.

Empirically, we observe that \algname exhibits almost-linear scaling for various choices of $d$, even for the same dataset. Whereas Figure \ref{fig:scaling} (left) suggested that \algname scales linearly on MNIST when using cosine distance, Figure \ref{fig:mods} (left) suggests that \algname also scales linearly when considering $l_2$ distance on MNIST; the slope of the line of best fit is 0.979. Additionally, we find that the scaling of \algname is not too sensitive to $k$, as long as $k \ll n$. Figure \ref{fig:mods} (right) demonstrates the scaling of \algname when $k$ is increased to 10; the slope of the line of best fit (0.930) still suggests roughly linear scaling in $n$.

%\mo{Mo: Add plots for MNIST,L2 k = 10 too}










% We consider two different settings for each dataset. The first setting is that in which UltraPAM must return the same results as PAM. In this setting, we find that UltraPAM demonstrates significant algorithmic speedups over PAM, while returning the same results with high probability. In the second setting, we relax this requirement that UltraPAM returns the same results as PAM. In the latter setting, we find that UltraPAM demonstrates an even greater speedup over PAM, while finding final medoid assignments that are nearly the same quality as those found by PAM and occasionally even better.


==> old/intro-06-05.tex <==
% !TEX root = 0-main.tex

% \martin{START of martin's version of Intro+Formulation}

% \martin{Introduction outline: 
% \begin{itemize}
%     \item Clustering is important and k-mean is one of the most popular clustering method. 
%     \item k-mean has two drawbacks.
%     \item First, it is only fast (linear for finding the centroid) when using $l_2^2$ or $l_1$ distance (the latter corresponds to k-median). However, for different applications, a different distance metric may be more appropriate (e.g. the editing distance for code.org)
%     \item Second, centroid is not a point in the dataset, while for some applications, having a representative for each cluster is important (e.g., a representative cell for single-cell RNA-seq)
%     \item Other clustering methods that allow for a user-defined distance matrix, like k-medoid, graph-based clustering methods (Louvain), requires precomputing of the distance matrix, which can be computationally and disk-space intensive. 
%     \item We consider an PAM  empirically preferable k-medoid algorithm PAM. (ref from wiki)
%     \item It is slow (need to quantify). We made it faster.
%     \item The algorithmic contributions are:
%     \item 1. We converted a deterministic computation problem into a random sampling problem, and used MAB to solve it. 
%     \item 2. The trick is to view each SWAP, instead of each data point, as an arm. 
%     \item 3. We adaptively chose the sub-Gaussian parameter for each stage and each arm to further increase speed. 
% \end{itemize}}

\section{Introduction}
\label{intro}

Many modern data science applications require clustering of very-large-scale data. 
Due to its computational efficiency, 
% and for this reason, 
$k$-means clustering \cite{macqueen1967some,lloyd1982least} is one such popular clustering algorithm.
% because of its computational efficiency.
% \mo{Not clear to me that large scale data makes $k$-means popular -- maybe just say $k$-means is a popular example method?}
The $k$-means clustering algorithm alternates between assigning points to their nearest cluster centers and recomputing those centers. 
% \mo{$k$-means "alternates between reassigning points to their nearest cluster centers and recomputing those centers"}
Central to its success is the specific choice of the cluster center: for a set of points, $k$-means defines the cluster center as the point with the smallest average \emph{squared Euclidean distance} to all other points in the set. 
Under such a definition, the cluster center is the arithmetic mean of the cluster's points, and this mean can be computed efficiently. 
% \mo{remove the word "very"?}

% \martin{include k-medians here?} \ilan{I would say no. I like the flow as is}

While commonly used in practice, $k$-means clustering suffers from several drawbacks. 
First, while one can efficiently compute the cluster centers under squared Euclidean distance, it is not straightforward to generalize $k$-means clustering to other distance metrics. 
% \mo{replace "However" with "Indeed"?} 
In different applications, other distance metrics may be desirable.
For example, $l_1$ and cosine distance is often used in sparse data, such as in recommendation systems \cite{leskovec2020mining} and single-cell RNA-seq analysis \cite{ntranos2016fast}; string edit distance in text data \cite{navarro2001guided}; or graph metrics in social network data \cite{mishra2007clustering}. For such distance metrics other than squared Euclidean distance, $k$-means algorithms are significantly less efficient \{citation\}.
Second, the cluster center in $k$-means clustering is in general not a point in the dataset and may not be interpretable in many applications. This is especially problematic when the data is structured, such as for parse trees in context-free grammars, sparse data in recommendation systems \cite{leskovec2020mining}, or images in computer vision where the mean image is simply noise \{citation\}. 

Alternatively, $k$-\underline{medoids} clustering algorithms \cite{kaufman1987clustering,kaufman1990partitioning} use the \emph{medoid} to define the cluster center for a set of point. Given an arbitrary distance function and a set of points, the medoid is the point \emph{in the set} that minimizes the average distance to all the other points.
Note that the distance metric can be arbitrary -- indeed, it need not be a distance metric at all and could be an asymmetric dissimilarity measure -- which addresses the first shortcoming of $k$-means outlined above.
% So $k$-medoids clustering algorithms work for arbitrary distances \mo{I think this sentence can be changed to "Note that the distance metric can be arbitrary; indeed, it need not be a metric at all and could be an asymmetric dissimilarity measure"}. 
Moreover, unlike $k$-means, the cluster centers in $k$-medoids, i.e. the medoids, are restricted to be points in the dataset, thus addressing the second shortcoming of $k$-means clustering. 

\mo{Need to make point that until now, PAM is $O(n^2)$, or you have to settle for suboptimal loss}
\mo{Also need to make the point that $k$-medoids has been largely unpopular due to its computational inefficiency}

More formally, for $n$ data points $\mathcal{X} =  \{ x_1, x_2, \cdots, x_n \}$ and a user-specified distance function $d(\cdot, \cdot)$, the $k$-medoids problem is to find a set of $k$ medoids $\mathcal{M} = \{m_1, \cdots, m_k \} \subset \mathcal{X}$ to minimize the overall distance of points from their closest medoids: 
\begin{equation} \label{eqn:sec_intro_total-loss}
	L(\mathcal{M}) =  \sum_{i=1}^n \min_{m_l \in \mathcal{M}} d(m_l, x_i)
\end{equation}
This problem is unfortunately NP-hard in general \cite{schubert2019faster}.
% \mo{in general. The Partionining Around Medoids...}., and the
The Partitioning Around Medoids (PAM) algorithm \cite{kaufman1987clustering, kaufman1990partitioning} is one of the most widely used heuristic algorithms for $k$-medoids clustering. PAM is split into two subroutines: BUILD and SWAP.
First, in the BUILD step, PAM aims to find an initial set of $k$ medoids by greedily and iteratively selecting points that minimize the overall loss in \eqref{eqn:sec_intro_total-loss}. 
Next, in the SWAP step, PAM considers all $k(n-k)$ possible pairs of medoid and non-medoid points and swaps the pair that reduces the $k$-medoids clustering loss (Equation \eqref{eqn:sec_intro_total-loss}) the most. 
The SWAP step is repeated until no further improvements can be made.

PAM has been empirically shown to produce better results than other popular $k$-medoids clustering algorithms \cite{reynolds2006clustering,schubert2019faster}. However, it can be prohibitively expensive to run, especially for large datasets. 
The BUILD subroutine takes $O((n-k)^2)$ distance evaluations to initialize each of the $k$ medoids, resulting in a complexity of $O(k(n-k)^2)$
%\ilan{prev sentence out of place?}
Each SWAP iteration also takes $O(k(n-k)^2)$ distance evaluations, in order to compute the change in loss for each of the $k(n-k)$ medoid-and-non-medoid pairs with respect to the remaining $n-k$ non-medoid points. 
Indeed, most of the runtime of PAM is spent in distance evaluations \{citation\}, which suggests it is desirable to lower this complexity.
% \mo{Need to add a point that most of the program time is spent in distance computations}

% \mo{Move this to related work}
% \martin{I prefer to have it here because it sets the right context without being too long. People need some background to underground our contribution, and more detailed background are in the related work section.}
Randomized algorithms like CLARA \cite{kaufman1990partitioning} and CLARANS \cite{ng2002clarans} have been proposed to improve computational efficiency, but at the cost of deteriorated clustering quality.
More recently, Schubert et al.~proposed a deterministic algorithm FastPAM \cite{schubert2019faster} that guarantees the same output as PAM but improves the complexity to $O(n^2)$ when the cluster sizes are similar. The factor $O(k)$ improvement is particularly important for large values of $k$. Apart from Section \ref

In the rest of the paper, we treat $k$ as fixed and assume $k \ll n$.
\martin{What happens to the FastPAM trick?}

\paragraph{Main Contributions:} In this work, we:
\begin{enumerate}
    \item Propose \algnamenospace, a randomized $k$-medoids algorithm that takes $O(n \log n)$ in the BUILD step and $O(n \log n )$ for each SWAP step, while returning the same result as PAM, with high probability under reasonable assumptions on the data,
    \item Experimentally validate our results on a number of real-world datasets, including Code.org Hour of Code, single-cell RNA-seq, and the MNIST handwritten digits datasets. 
    \item Provide publicly available C++ and Python implementations of \algnamenospace
\end{enumerate}

%\mo{Is our proof for different arm variances also novel?}

Crucially, \algname takes $O(n \log n)$ distance evaluations in each iteration, effectively improving each step from quadratic to almost linear. On MNIST, the state-of-the-art implementation of FastPAM caches the pairwise distance matrix and runs in approximately 3 hours; \algname runs in less than an hour and returns the same results. Furthermore, \algname does not cache the pairwise distance matrix, resulting in an $O(n^2)$ savings in space.
%\algname reduces to FastPAM for a large value of $k$. \mo{I don't think this is true}

% \ilan{apx, or app may be better than apr}
% We also propose a variation \algaprname that slightly deviates from the PAM solution but is significantly faster.
% \martin{Update this paragraph after finishing the main paper} \mo{Looks like we can remove -apr variant for this submission. Also, worth mentioning the python implementations of CLARANS that we release? As well as C++/Python B-PAM?}

Intuitively, \algname works by recasting each step of PAM from a \emph{deterministic computational problem} to a \emph{statistical estimation problem}. 
In each BUILD step medoid assignment, for example, we need to choose the point amongst all $n-k$ non-medoids that will lead to the lowest overall loss \{ref\} if chosen as the next medoid. Mathematically, we wish to find $x$ to minimize:
\begin{equation} \label{eqn:sec_intro_build_loss}
	L(x; \mathcal{M}) = \sum_{j=1}^n \min_{m \in \mathcal{M} \cup \{x\}} d(m, x_j) \overset{\text{def}}{=} \sum_{j=1}^n g(x_j),
\end{equation}


% In the SWAP step, for example, we need to decide among $k(n-k)$ possible medoid-and-non-medoid swaps, which one leads to the smallest loss. 
% If we swap, for example, medoid $m_l$ and and non-medoid $x_i$, the new set of medoids after excluding $m_l$ and including $x_i$ would be $\mathcal{M}-\{m_l\} + \{x_i\}$,
% and the corresponding loss:
% \begin{equation} \label{eqn:sec_intro_swap_loss}
% 	L(m_l, x_i; \mathcal{M}) = \sum_{j=1}^n \min_{m_l \in \mathcal{M}-\{m_l\} + \{x_i\}} d(m_l, x_j) \overset{\text{def}}{=} \sum_{j=1}^n g(x_j),
% \end{equation}
where $g(\cdot)$ is a function that depends on $\mathcal{M}$, $x$, and $x_i$.
Eq.~\eqref{eqn:sec_intro_build_loss} shows that the loss of a new medoid assignment $L(\mathcal{M}; x)$ can be written as the summation of the value of the function $g(\cdot)$ evaluated on all $n$ points in the dataset. Though approaches such as PAM compute $L(\mathcal{M}; x)$ exactly for each $x$, \algname \textit{adaptively estimates} this quantity by sampling reference points $x_j$ for the most promising candidates. Indeed, computing $L(\mathcal{M}; x)$ exactly for every $x$ is not required; promising candidates can be estimated with higher accuracy (more $x_j$s) and less promising ones can be discarded early without requiring further unnecessary computation.

% Recall that the goal of the SWAP step is to find the medoid-and-non-medoid swap with the smallest loss, which is different from computing the exact loss for every possible swap. 
% So an estimation of the best swap with high confidence would suffice. 
% Intuitively,  promising swaps with smaller loss should be estimated with a higher accuracy and less promising ones can be discarded without being evaluated on too many randomly-sampled data points. 

To design the adaptive sampling strategy, we show that the BUILD step and each SWAP iteration can be formulated as a best-arm identification problems from the multi-armed bandits (MAB) literature \cite{audibert2010best,even2002pac,jamieson2014lil,jamieson2014best}. 
In the typical version of the best-arm identification problem, we have $m$ arms. At each timestep $t = 0,1,\cdots,$ we decide to pull an arm $A_t\in \{1,\cdots,m\}$, and receive a reward $R_t$ with $E[R_t] = \mu_{A_t}$. The goal is to identify the arm with the largest expected reward with high probability while expending the fewest number of total arm pulls.
In the BUILD step, we view each candidate medoid $x$ as an arm in a best-arm identification problem. The arm parameter corresponds $E[g]$, and by pulling an arm, we observe the loss evaluated on a randomly sampled data point $x_j$. Using this reduction, the best candidate medoid can be estimated using existing best-arm algorithms like the Upper Confidence Bound (UCB) algorithm \cite{lai1985asymptotically}.
% In the context of the PAM SWAP step, we can think of each possible medoid-and-non-medoid swap as an arm in the best-arm problem, totaling $k(n-k)$ arms. The arm parameter corresponds to the loss of the swap, and by pulling an arm, we observe the loss evaluated on a randomly sampled data point. 
% Then, the best swap can be estimated using existing best-arm algorithms like the Upper Confidence Bound (UCB) algorithm \cite{lai1985asymptotically}.

\subsection{Related work}

\mo{RAND and other baselines in Meddit paper (TOPRANK?) necessary to mention?}

The $k$-means clustering algorithm is one of the \emph{centroid}-based clustering methods, where the centroid of a set of points for a distance metric is defined as the point \emph{in the space}
% \mo{"among the datapoints"?}
that minimizes the overall distance to other points.
%So the key difference between centroid and medoid is that a centroid does not need to be one of the points in the set. 
$k$-means uses the centroid for squared Euclidean distance to define the cluster center, which is the arithmetic mean and can be computed in linear time. 
Centroid for Bregman divergence is also the arithmetic mean and centroid for $l_1$ distance is the component-wise median; the latter is used by the $k$-medians clustering algorithm \cite{bradley1997clustering,jain1988algorithms}.
However, the centroid for other distances is in general hard to compute.
For example, the centroid for the unsquared Euclidean distance corresponds to the much harder Weber problem with no closed-form solution \cite{bradley1997clustering,overton1983quadratically}. 
%\martin{Maybe delete this paragraph if we don't have enough space}
\mo{I think we can move this above to where this is first discussed}
\martin{I prefer to put it here because there are a bit detailed. These are used to justify PAM and people don't need them to understand out contribution.}

There are a large variety of $k$-medoids clustering algorithms. Park et al.~\cite{park2009simple} proposed a $k$-means-like algorithm that alternates between reassigning the points to their closest medoid and recomputing the medoid for each cluster, until the $k$-medoids clustering loss can no longer be improved. CLARA and CLARANS \{citation \} are algorithms that...
However, all of these approaches have been empirically to produce less satisfactory results than PAM \cite{reynolds2006clustering,schubert2019faster}. 
Other proposals include optimizations for Euclidean space and tabu search heuristics \cite{estivill2001robust}.
\mo{Mention PAMAE/distributed PAM?}
\martin{Yes. Could you add them?}

The idea of algorithm acceleration by converting a computational problem into a statistical estimation problem and designing the adaptive sampling procedure via multi-armed bandits has
witnessed a few successes, such as in Monte Carlo tree search \cite{chang2005adaptive,kocsis2006bandit}, hyper-parameter tuning \cite{li2016hyperband,jamieson2016non}, discrete optimization \cite{bagaria2018adaptive}, and permutation-based multiple hypothesis testing \cite{zhang2019adaptive}. 
In the context of $k$-medoids clustering, previous works \cite{bagaria2018medoids,baharav2019ultra} have considered finding the \textit{single} medoid of a set points (the $1$-medoid problem).
In these works, the $1$-medoid problem was also formulated as a best-arm identification problem, with each point being an arm and its average distance to other points being the arm parameter. 
% \mo{Maybe join this last sentence with paragraph below?}

While the $1$-medoid problem considered in prior work can be solved exactly, the $k$-medoids problem is NP-Hard and is therefore only tractable with heuristic solutions. Hence, this paper focuses on improving the computational efficiency an existing heuristic solution, PAM, that has been empirically observed to be superior to other techniques.
% In addition, it is not straighforward to generalize the best-arm problem formulation to the $k$-medoid problem neither.
Moreover, instead of having a single best-arm identification problem, we reformulate PAM as a sequence of best-arm problems. We treat different objects as arms in different steps of PAM; in the BUILD step, each point corresponds to an arm, whereas in the SWAP step, each medoid-and-non-medoid pair corresponds to an arm.
% Building on top of this, 
We further notice that the intrinsic difficulties of this sequence of best-arm problems are different, which can be exploited to further speed up the algorithm, as demonstrated in Section \ref{exps}.

% Last but not the least, as demonstrated in the later part the paper, the intrinsic difficulty of different best-arm problems are different, and we can adapt to this to make significant improvement.   

The rest of the paper is organized as follows. In Section \ref{sec:prelims}, we formally describe the $k$-medoids problem and the PAM algorithm. In Section \ref{sec:algo}, we describe our proposed algorithm, \algnamenospace. In section \ref{sec:theory}, we provide theoretical guarantees for when \algname will demonstrate the expected computational speedup while returning the same results and tracking the same optimization trajectory as PAM. In Section \ref{sec:exps}, we experimentally validate \algnamenospace's performance on a number of datasets. We discuss the results of these experiments in Section \ref{sec:discussion}. We conclude with a discussion of future research directions and the broader impact of our work in Sections \ref{sec:future}
 and \ref{sec:impact}, respectively.


% \subsection{Partitioning Around Medoids}
% PAM \cite{kaufman1987clustering, kaufman1990partitioning} first initializes the set of $k$ medoids via the BUILD step and then repeatedly performs the SWAP step to improve the loss until convergence. 

% \paragraph{BUILD step:} Select an initial set of $k$ medoids by greedily adding one point at a time so as to minimize the overall loss \eqref{eqn:sec_intro_total-loss}. 
% The first point to add is the medoid of all $n$ points.
% Given the current set of $l-1$ medoids $\mathcal{M}_{l-1} = \{m_1, \cdots, m_{l-1}\}$, the next point to add $m_l$ can be written as
% \begin{equation}
% \label{eqn:build-next-medoid}
%     m_l = \argmin_{x \in \mathcal{X} \setminus \mathcal{M}_{l-1}} \sum_{j=1}^n \min[d(x, x_j), \min_{m' \in \mathcal{M}_{l-1}} d(m', x_j)]. 
% \end{equation}

% Computing $m_l$ from Eq.~\eqref{eqn:build-next-medoid} requires computing the distance $d$ between each candidate point $x \in \mathcal{X}\setminus\mathcal{M}_{l-1}$ and all other points in the dataset---effectively $O(n^2)$ computations. 
% PAM BUILD step repeats such a search $k$ times, totaling $O(kn^2)$ distance computations. This is prohibitively expensive when the distance evaluation is costly, e.g., high-dimensional data or complicated choices of $d$ such as the Wasserstein distance.

% \paragraph{SWAP step:} Among all possible $k(n-k)$ pairs of medoid and non-medoid points, swap the one that would reduce the loss the most.
% Let $\mathcal{M}$ be the current set of $k$ medoids. The best pair to swap is then
% \begin{equation}
% \label{eqn:next-swap}
%     (m^*, x^*) = \argmin_{(m,x) \in \mathcal{M} \times (\mathcal{X} \setminus \mathcal{M}) } \sum_{j=1}^n \min[d(x, x_j), \min_{m' \in \mathcal{M}\setminus \{m\}} d(m', x_j)]. 
% \end{equation}

% The SWAP step is repeated until no improvement can be made. 
% Similar to the BUILD step, each SWAP step requires $O(k(n-k)^2)$ distance computations.


% \subsection{Formal $k$-medoids Problem Statement}
% Formally, let $\mathcal{X} =  \{ x_1, x_2, \cdots, x_N \}$ be a set of $N$ points in $d$ dimensions, $k$ be the number of clusters to find, and $d(\cdot, \cdot)$, a distance function. For a given set of $k$ medoids $\mathcal{M} = \{m_1, \cdots, m_k \} \subset \mathcal{X}$, the objective function of the $k$-medoids problem is the sum of distances from each point to its closest medoid: \martin{Both $N$ and $n$ are used to denote the number of data points. I suggest to consistently use $n$ because other quantities like $d$ and $k$ are both lower-case.} \martin{$d$ was used to denote both the number of dimensions and the distance metric. Schubert et al. 2018 also overloaded $d$, but this hurts clarity. Maybe changing the distance function to $dist$?}
% \begin{equation}
% \label{eqn:total-loss}
% 	L(\mathcal{M}) =  \sum_{i=1}^n \min_{m_l \in \mathcal{M}} d(m_l, x_i)
% \end{equation}

% The $k$-medoids problem is then to determine the optimal assignment of medoids $\mathcal{M}$, i.e. $\argmin_{\mathcal{M}}L({\mathcal{M}})$

% Note that while $d$ is often a distance metric such as $L_2$ distance, it need not be so; in fact, any arbitrary dissimilarity metric (even an asymmetric one) could be provided above. In general, this problem is NP-Hard \ref{citation}. As such, this problem is generally tackled with greedy iterative algorithms, which we discuss Section \ref{priorwork}.

% \subsection{Comparison to $k$-means}

% At first glance, the problem specification of $k$-medoids may appear very similar to $k$-means, where a similar objective function is used:

% \begin{equation}
% \label{eqn:total-loss-means}
% 	L_{kmeans}(\{\mu_1, \dots, \mu_k\}) =  \sum_{i=1}^n \min_{\mu \in \{\mu_1, \dots, \mu_k\}} ||d(\mu, x_i)||^2
% \end{equation}

% Crucially, however, in $k$-means the optimization of $L_{kmeans}$ is performed over all possible sets of vectors $U = \{\mu_1, \dots, \mu_k\} \subset \mathbb{R}^d$ and the means $\mu_i$ are not required to be actual datapoints. \martin{Use text format for subscript that is not a variable, e.g. $L_{\text{kmeans}}$.}

% Naturally, one might ask if we could reduce the $k$-medoids problem to the $k$-means problem by choosing the medoids to be the real datapoints closest to the means $\{\mu_1, \dots, \mu_k\}$. However, this approach is more susceptible to outliers due to the squaring of the individual loss terms in \ref{eqn:total-loss-means} and will not return the same results as the $k$-medoids problem. It is straightforward to construct small examples where the results of this approach disagree with the solution of the $k$-medoids problem. In fact, it is well-known that $k$-means is more susceptible to noise and outliers than $k$-medoids \ref{citation}.

% In the $k$-means algorithm, $d$ in Equation \ref{eqn:total-loss-means} is usually $L_2$ distance. For completeness, we also mention the \textbf{$k$-medians} problem, in which $d$ is instead the $L_1$ distance, which is less susceptible to noise and outliers than the usual $L_2$ distance. This (rather specific) problem permits an EM-style decomposition which results in an algorithmic complexity similar to the one shown in this paper \ref{citation}; however, the loss function being optimized is different from that in the $k$-medoids problem. Furthermore, the approach presented in our work applies more generally to arbitrary $d$, even those which are not metrics such as $L_1$ or other popular metrics.

% \ilan{The paragraph above is not very clear to me. Are we sure that $k$-medians is generally understood to be $k$-means with $L_1$ instead $L_2$ distances?}

% \section{Prior Work} \martin{Put prior work as a subsection of the Introduction section}
% \label{priorwork}

% \subsection{Partitioning Around Medoids (PAM)}
% The $k$-medoids problem is, in general, NP-hard. As such, iterative greedy algorithms are often used.  The state-of-the-art algorithm for the $k$-medoids problem, Partitioning Around Medoids (PAM), takes a greedy approach, divided into two steps: BUILD and SWAP. In the BUILD step, medoids are initialized one-by-one by choosing each new medoid to be the one that would lower the loss (Equation \ref{eqn:total-loss}) the most. In the SWAP step, we consider swapping each of the medoid assignments with a non-medoid and perform the swap which would lower the loss (Equation \ref{eqn:total-loss}) the most. The BUILD step is run once and then the SWAP step is run multiple times until convergence.

% \subsubsection{PAM BUILD step}
% In the BUILD step, each of the medoids is greedily initialized by choosing the $l$th medoid, conditioned on the previous $l-1$ medoids, that reduces the total loss of every other point. 
% \ilan{}
% More formally, suppose the current set of medoids is $\mathcal{M} = \{m_1, \cdots, m_{l-1}\}$ and we wish to add the $l$th medoid $m_l$. Our goal is to identify a new medoid $m_l$ such that:

% \begin{equation}
% \label{eqn:build-next-medoid}
%     m_l = \argmin_{x \in \mathcal{X} \setminus \mathcal{M}} \sum_{j=1}^n \min[d(x, x_j), \min_{m' \in \mathcal{M}} d(m', x_j)]. 
% \end{equation}

% Equivalently, we can find the find $m_l$ that minimizes the change in total loss:

% \begin{equation}
% \label{eqn:build-next-medoid-td}
%     m_l = \argmin_{x \in \mathcal{X} \setminus \mathcal{M}} \sum_{j=1}^n  \Delta L_{x}(x_j)
% \end{equation}

% where

% \begin{equation}
% \label{eqn:build-td}
%     \Delta L_{x}(x_j) = \min[d(x, x_j) - \min_{m' \in \mathcal{M}} d(m', x_j), 0]
% \end{equation}

% \ilan{Should we instead be defining the change to be positive? 
% Saying ``minimizes the change in total loss'' sounds a bit weird to me, because it sounds like you want to make as little change as possible.}

% represents the change in total loss for reference point $x_j$ induced by choosing $x$ as a new medoid. \martin{$\Delta L_{x}(x_j)$ is not well-defined because the dependency on $\mathcal{M}$ was omitted. How about $\Delta L_{x, \mathcal{M}}(x_j)$?} 

% Computing $m_l$ from Equation \ref{eqn:build-next-medoid} \martin{Use \eqref{eqn:build-next-medoid}} requires computing $d$ for each candidate point $x \in \mathcal{X}\setminus\mathcal{M}$ to each other point in the dataset -- an $O(N^2)$ operation. Furthermore, this process must be repeated for each of the $k$ initial medoid assignments. As such, the PAM BUILD step requires $O(kN^2)$ computations of the distance function $d$; this is prohibitively expensive for complicated choices of $d$ such as Wasserstein distance.
% \ilan{Maybe ``This is prohibitively expensive when the data is very high dimensional or for complicated choices of $d$ such as the Wasserstein distance.'' We don't want to give the impression that this is only relevant for non-trivial distances}

% \subsubsection{PAM SWAP Step}
% In the SWAP step, we consider swapping the assignment of any of the $k$ medoids with any of the $N-k$ non-medoids. For each of the possible $k(N-k)$ swaps, we calculate the total change in loss for each of the $N$ datapoints. We then perform the swap that would lower the total loss for the dataset. 

% Specifically, our goal is to find a medoid-nonmedoid pair $(m^*, x^*)$ such that:

% \begin{equation}
% \label{eqn:next-swap}
%     (m^*, x^*) = \argmin_{(m,x) \in \mathcal{M} \times (\mathcal{X} \setminus \mathcal{M}) } \sum_{j=1}^n \min[d(x, x_j), \min_{m' \in \mathcal{M}\setminus \{m\}} d(m', x_j)]. 
% \end{equation}

% Equivalently, we can find $(m^*, x^*)$ that minimizes:

% \begin{equation}
% \label{eqn:next-swap-td}
%     (m^*, x^*) = \argmin_{(m,x) \in \mathcal{M} \times (\mathcal{X} \setminus \mathcal{M}) } \sum_{j=1}^n \Delta L_{m, x_i}(x_j)
% \end{equation}

% where

% \begin{equation}
% \label{eqn:swap-td}
%     \Delta L_{m, x_i}(x_j) = \min[d(x_i, x_j) - \min_{m' \in \mathcal{M}\setminus \{m\}} d(m', x_j), 0]
% \end{equation}

% represents the induced change in loss for point $x_j$ by removing $m$ from the list of medoids and choosing $x_i$ as a new medoid. \martin{$\Delta L_{m, x_i}(x_j)$ is not well-defined because the dependency on $\mathcal{M}$ was omitted. How about $\Delta L_{m, x_i,\mathcal{M}}(x_j)$? Also, this is very similar to the $\Delta L$ in the BUILD step. Consider changing them to $\Delta L^{\text{BUILD}}$ and $\Delta L^{\text{SWAP}}$ for clarity.} 

% The SWAP step is iterated until convergence. Similar to the BUILD step, each SWAP step requires $O(kN^2)$ distance computations, which is prohibitively expensive for complicated choices of $d$.

% \subsection{FastPAM1}

% Accelerating the PAM algorithm is an active area of research. Perhaps most closely related to our work is \ref{FastPAM}, which presents three independent optimizations to the original PAM algorithm. Of these three, only one (dubbed FastPAM1) optimization applied to the SWAP step, preserves the results as the original PAM algorithm.

% In the FastPAM1 optimization, the distance from each point $x_j$ to its nearest medoid, $d_1(x_j)$, and to its \textit{second nearest} medoid, $d_2(x_j)$ is used to rewrite \ref{eqn:swap-td} \martin{\eqref{eqn:swap-td}} as:

% \begin{equation}
% \label{eqn:FastPam1-eqn}
%     \Delta L_{m, x_i}(x_j) = - d_1(x_j)\mathbbm{1}_{x_j \in C_m} + d(x_i, x_j)\mathbbm{1}_{x_j \in C_{x_i}} + d_2(x_j)\mathbbm{1}_{x_j \notin C_{x_i}}
% \end{equation}

% \ilan{I find the notation with $x_i$ and $x_j$ a bit confusing. It's a bit weird that $m$ and $x_i$ are the things being swapped, while $x_j$ is just a general point}

% where $C_m$ is the set of points assigned to medoid $m$ before the swap, and $C_{x_i}$ is the set of points that would be assigned to the new medoid $x_i$ if the swap were performed. 
% Note that now the quantities $d_1(x_j)$ and $d_2(x_j)$ can be cached and that (\ref{eqn:FastPam1-eqn}) no longer depends on $m$. \ilan{I don't see that right away}
% This optimization reduces the complexity of PAM by $O(k)$ in each SWAP step, but only when the clusters are roughly similar in size, each containing about $O(\frac{1}{k})$ points \textbf{why is balanced cluster distro necessary? Eqn 8 doesn't suggest that}. 
% In our algorithm, UltraPAM, we see a $O(\frac{N}{logN})$ speedup under relatively mild assumptions and do not require the clusters to be balanced. \ilan{not the best place to mention UltraPAM for the first time.}
% Furthermore, it is possible to combine the FastPAM1 optimization with UltraPAM; indeed, we do so in our reference implementation available at \{githublink\}.

% \martin{Use $\mathcal{C}$ font to denote sets.}

% \martin{Could you double check \eqref{eqn:FastPam1-eqn}? I have a different answer. Divide the points into four categories based on which medoid it assigned to before and after the SWAP: 
% \begin{itemize}
% \item Before $m$ and after $x_i$; point set $C_m \cap C_{x_i}$; delta loss $d(x_i,x_j) - d_1(x_j)$.
% \item Before $m$ and after other medoids; point set $C_m \cap C_{x_i}^c$; delta loss $d_2(x_j) - d_1(x_j)$.
% \item Before other medoids and after $x_i$; point set $C_m^c \cap C_{x_i}$; delta loss $d(x_i,x_j) - d_1(x_j)$.
% \item Before other medoids and other medoids; point set $C_m^c \cap C_{x_i}^c$; delta loss $0$.
% \end{itemize}
% Therefore, 
% \begin{equation}
%     \Delta L_{m, x_i}(x_j) = - d_1(x_j)\mathbbm{1}_{\{x_j \in C_m \cup C_{x_i}\}} + d(x_i, x_j)\mathbbm{1}_{\{x_j \in C_{x_i}\}} + d_2(x_j)\mathbbm{1}_{\{x_j \in C_{m}\cap C_{x_i}^c\}}
% \end{equation}
% }

% \ilan{
% I checked, and I agree with this.
% In particular, if $x_j$'s previous closest medoid was some $m' \ne m$ and $d(x_j,m') < d(x_j,x_i)$, the delta should be 0. In this case, $x_j \notin C_m$, $x_j \notin C_{x_i}$, so equation (9) gives $d_2(x_j)$, while (10) gives 0.
% } 

% \martin{\eqref{eqn:FastPam1-eqn} is hard to follow. Add more details (like the one I mentioned above). }

% \subsection{Theoretical Motivation: Multi-Armed Bandits}

% Add description of MAB problem. Theory from the multi-armed bandit (MAB) literature suggests that best arm among $N$ arms can be found with $O(NlogN)$ \martin{$O(N\log N)$} arm pulls, as in the UCB algorithm \{citation\}. \martin{Be more precise here. Include the success probability $\delta$ and the gaps between the best arm and other arms $\delta \mu_i$ in the expression.} This observation motivates the approach presented in this paper, in which we use an adaptation of the UCB algorithm to find medoids more quickly. 

% \ilan{we take too long to get here}

% Intuitively, in the BUILD step, we consider each of the $N$ candidate datapoints as an "arm", where an arm pull corresponds to computing the induced loss on a single reference datapoint by choosing the candidate in question as a medoid.  The multi-armed bandit (MAB) literature then suggests that we can identify the best medoid to assign with $O(NlogN)$ distance computations in each of the $k$ BUILD steps.

% Similarly, in the SWAP step, we consider each of the $k(N-k)$ medoid-nonmedoid pairs as an "arm", and an arm pull corresponds to computing the loss induced on a reference point by swapping the medoid with the non-medoid. The multi-armed bandit (MAB) literature then suggests that we can identify the best swap to perform with $O(kNlogN)$ distance computations in each SWAP step.

% Intuitively, in each of the BUILD and SWAP steps, we convert the computation of the sum for each candidate $m_l$ in \ref{eqn:build-next-medoid} or $(m,x)$ in \ref{eqn:swap-td} into a sampling problem. Instead of computing the sums exactly, we compute confidence intervals that contain the sum with high probability and explore promising arms more while expending less computation on unpromising arms. We expect such a UCB-based approach to recover the true best arm, thus matching the results of the greedy algorithm PAM, with high probability.  We formally describe the algorithm in Section \ref{algo}, along with theoretical guarantees for correctness in Section \ref{theory}.

% \subsection{Main Contributions}

% In this work, we:

% \begin{enumerate}
%     \item Propose a new algorithm, \algnamenospace, that uses a UCB-based algorithm to find a solution to the $k$-medoids problem,
%     \item Provide theoretical guarantees as to when UltraPAM will return the same results as current state-of-the-art methods such as PAM, and
%     \item Experimentally validate our approach on a number of real-world datasets.
% \end{enumerate}


% \martin{END of martin's version of Intro+Formulation}

==> old/intro05-29.tex <==
\section{Introduction}
\label{intro}
% 1. Comparison to k means -- see Wikipedia [a. more robust to outliers and noise, b. works with arbitrary dissimilarities]
% 2. Explanation of k-means-then-nearest-neighbor baseline
% 3. Formal problem statement
% 4. In general, this is an NP-hard or NP-complete algorithm, so use greedy

Clustering large, high-dimensional datasets is an active area of research with applications in computer vision, natural language processing, reinforcement learning, and more \ref{need citations}. The $k$-medoids problem is an example of such a task in which the cluster centers are required to be actual datapoints. In this section, we provide a formal statement of the $k$-medoids problem, a description of existing approaches, and comparisons to other clustering methods such as $k$-means.

\ilan{I think we should discuss why one would want representative points that are themselves data points here, and already talk about specific applications like representative images in a set of images, representative gene expression profile in sc-RNAseq data.}


\subsection{Formal $k$-medoids Problem Statement}
Formally, let $\mathcal{X} =  \{ x_1, x_2, \cdots, x_N \}$ be a set of $N$ points in $d$ dimensions, $k$ be the number of clusters to find, and $d(\cdot, \cdot)$, a distance function. For a given set of $k$ medoids $\mathcal{M} = \{m_1, \cdots, m_k \} \subset \mathcal{X}$, the objective function of the $k$-medoids problem is the sum of distances from each point to its closest medoid: \martin{Both $N$ and $n$ are used to denote the number of data points. I suggest to consistently use $n$ because other quantities like $d$ and $k$ are both lower-case.} \martin{$d$ was used to denote both the number of dimensions and the distance metric. Schubert et al. 2018 also overloaded $d$, but this hurts clarity. Maybe changing the distance function to $dist$?}
\begin{equation}
\label{eqn:total-loss}
	L(\mathcal{M}) =  \sum_{i=1}^n \min_{m_l \in \mathcal{M}} d(m_l, x_i)
\end{equation}

The $k$-medoids problem is then to determine the optimal assignment of medoids $\mathcal{M}$, i.e. $\argmin_{\mathcal{M}}L({\mathcal{M}})$

Note that while $d$ is often a distance metric such as $L_2$ distance, it need not be so; in fact, any arbitrary dissimilarity metric (even an asymmetric one) could be provided above. In general, this problem is NP-Hard \ref{citation}. As such, this problem is generally tackled with greedy iterative algorithms, which we discuss Section \ref{priorwork}.

\subsection{Comparison to $k$-means}

At first glance, the problem specification of $k$-medoids may appear very similar to $k$-means, where a similar objective function is used:

\begin{equation}
\label{eqn:total-loss-means}
	L_{kmeans}(\{\mu_1, \dots, \mu_k\}) =  \sum_{i=1}^n \min_{\mu \in \{\mu_1, \dots, \mu_k\}} ||d(\mu, x_i)||^2
\end{equation}

Crucially, however, in $k$-means the optimization of $L_{kmeans}$ is performed over all possible sets of vectors $U = \{\mu_1, \dots, \mu_k\} \subset \mathbb{R}^d$ and the means $\mu_i$ are not required to be actual datapoints. \martin{Use text format for subscript that is not a variable, e.g. $L_{\text{kmeans}}$.}

Naturally, one might ask if we could reduce the $k$-medoids problem to the $k$-means problem by choosing the medoids to be the real datapoints closest to the means $\{\mu_1, \dots, \mu_k\}$. However, this approach is more susceptible to outliers due to the squaring of the individual loss terms in \ref{eqn:total-loss-means} and will not return the same results as the $k$-medoids problem. It is straightforward to construct small examples where the results of this approach disagree with the solution of the $k$-medoids problem. In fact, it is well-known that $k$-means is more susceptible to noise and outliers than $k$-medoids \ref{citation}.

In the $k$-means algorithm, $d$ in Equation \ref{eqn:total-loss-means} is usually $L_2$ distance. For completeness, we also mention the \textbf{$k$-medians} problem, in which $d$ is instead the $L_1$ distance, which is less susceptible to noise and outliers than the usual $L_2$ distance. This (rather specific) problem permits an EM-style decomposition which results in an algorithmic complexity similar to the one shown in this paper \ref{citation}; however, the loss function being optimized is different from that in the $k$-medoids problem. Furthermore, the approach presented in our work applies more generally to arbitrary $d$, even those which are not metrics such as $L_1$ or other popular metrics.

\ilan{The paragraph above is not very clear to me. Are we sure that $k$-medians is generally understood to be $k$-means with $L_1$ instead $L_2$ distances?}

\section{Prior Work} \martin{Put prior work as a subsection of the Introduction section}
\label{priorwork}

\subsection{Partitioning Around Medoids (PAM)}
The $k$-medoids problem is, in general, NP-hard. As such, iterative greedy algorithms are often used.  The state-of-the-art algorithm for the $k$-medoids problem, Partitioning Around Medoids (PAM), takes a greedy approach, divided into two steps: BUILD and SWAP. In the BUILD step, medoids are initialized one-by-one by choosing each new medoid to be the one that would lower the loss (Equation \ref{eqn:total-loss}) the most. In the SWAP step, we consider swapping each of the medoid assignments with a non-medoid and perform the swap which would lower the loss (Equation \ref{eqn:total-loss}) the most. The BUILD step is run once and then the SWAP step is run multiple times until convergence.

\subsubsection{PAM BUILD step}
In the BUILD step, each of the medoids is greedily initialized by choosing the $l$th medoid, conditioned on the previous $l-1$ medoids, that reduces the total loss of every other point. 
\ilan{}
More formally, suppose the current set of medoids is $\mathcal{M} = \{m_1, \cdots, m_{l-1}\}$ and we wish to add the $l$th medoid $m_l$. Our goal is to identify a new medoid $m_l$ such that:

\begin{equation}
\label{eqn:build-next-medoid}
    m_l = \argmin_{x \in \mathcal{X} \setminus \mathcal{M}} \sum_{j=1}^n \min[d(x, x_j), \min_{m' \in \mathcal{M}} d(m', x_j)]. 
\end{equation}

Equivalently, we can find the find $m_l$ that minimizes the change in total loss:

\begin{equation}
\label{eqn:build-next-medoid-td}
    m_l = \argmin_{x \in \mathcal{X} \setminus \mathcal{M}} \sum_{j=1}^n  \Delta L_{x}(x_j)
\end{equation}

where

\begin{equation}
\label{eqn:build-td}
    \Delta L_{x}(x_j) = \min[d(x, x_j) - \min_{m' \in \mathcal{M}} d(m', x_j), 0]
\end{equation}

\ilan{Should we instead be defining the change to be positive? 
Saying ``minimizes the change in total loss'' sounds a bit weird to me, because it sounds like you want to make as little change as possible.}

represents the change in total loss for reference point $x_j$ induced by choosing $x$ as a new medoid. \martin{$\Delta L_{x}(x_j)$ is not well-defined because the dependency on $\mathcal{M}$ was omitted. How about $\Delta L_{x, \mathcal{M}}(x_j)$?} 

Computing $m_l$ from Equation \ref{eqn:build-next-medoid} \martin{Use \eqref{eqn:build-next-medoid}} requires computing $d$ for each candidate point $x \in \mathcal{X}\setminus\mathcal{M}$ to each other point in the dataset -- an $O(N^2)$ operation. Furthermore, this process must be repeated for each of the $k$ initial medoid assignments. As such, the PAM BUILD step requires $O(kN^2)$ computations of the distance function $d$; this is prohibitively expensive for complicated choices of $d$ such as Wasserstein distance.
\ilan{Maybe ``This is prohibitively expensive when the data is very high dimensional or for complicated choices of $d$ such as the Wasserstein distance.'' We don't want to give the impression that this is only relevant for non-trivial distances}

\subsubsection{PAM SWAP Step}
In the SWAP step, we consider swapping the assignment of any of the $k$ medoids with any of the $N-k$ non-medoids. For each of the possible $k(N-k)$ swaps, we calculate the total change in loss for each of the $N$ datapoints. We then perform the swap that would lower the total loss for the dataset. 

Specifically, our goal is to find a medoid-nonmedoid pair $(m^*, x^*)$ such that:

\begin{equation}
\label{eqn:next-swap}
    (m^*, x^*) = \argmin_{(m,x) \in \mathcal{M} \times (\mathcal{X} \setminus \mathcal{M}) } \sum_{j=1}^n \min[d(x, x_j), \min_{m' \in \mathcal{M}\setminus \{m\}} d(m', x_j)]. 
\end{equation}

Equivalently, we can find $(m^*, x^*)$ that minimizes:

\begin{equation}
\label{eqn:next-swap-td}
    (m^*, x^*) = \argmin_{(m,x) \in \mathcal{M} \times (\mathcal{X} \setminus \mathcal{M}) } \sum_{j=1}^n \Delta L_{m, x_i}(x_j)
\end{equation}

where

\begin{equation}
\label{eqn:swap-td}
    \Delta L_{m, x_i}(x_j) = \min[d(x_i, x_j) - \min_{m' \in \mathcal{M}\setminus \{m\}} d(m', x_j), 0]
\end{equation}

represents the induced change in loss for point $x_j$ by removing $m$ from the list of medoids and choosing $x_i$ as a new medoid. \martin{$\Delta L_{m, x_i}(x_j)$ is not well-defined because the dependency on $\mathcal{M}$ was omitted. How about $\Delta L_{m, x_i,\mathcal{M}}(x_j)$? Also, this is very similar to the $\Delta L$ in the BUILD step. Consider changing them to $\Delta L^{\text{BUILD}}$ and $\Delta L^{\text{SWAP}}$ for clarity.} 

The SWAP step is iterated until convergence. Similar to the BUILD step, each SWAP step requires $O(kN^2)$ distance computations, which is prohibitively expensive for complicated choices of $d$.

\subsection{FastPAM1}

Accelerating the PAM algorithm is an active area of research. Perhaps most closely related to our work is \ref{FastPAM}, which presents three independent optimizations to the original PAM algorithm. Of these three, only one (dubbed FastPAM1) optimization applied to the SWAP step, preserves the results as the original PAM algorithm.

In the FastPAM1 optimization, the distance from each point $x_j$ to its nearest medoid, $d_1(x_j)$, and to its \textit{second nearest} medoid, $d_2(x_j)$ is used to rewrite \ref{eqn:swap-td} \martin{\eqref{eqn:swap-td}} as:

\begin{equation}
\label{eqn:FastPam1-eqn}
    \Delta L_{m, x_i}(x_j) = - d_1(x_j)\mathbbm{1}_{x_j \in C_m} + d(x_i, x_j)\mathbbm{1}_{x_j \in C_{x_i}} + d_2(x_j)\mathbbm{1}_{x_j \notin C_{x_i}}
\end{equation}

\ilan{I find the notation with $x_i$ and $x_j$ a bit confusing. It's a bit weird that $m$ and $x_i$ are the things being swapped, while $x_j$ is just a general point}

where $C_m$ is the set of points assigned to medoid $m$ before the swap, and $C_{x_i}$ is the set of points that would be assigned to the new medoid $x_i$ if the swap were performed. 
Note that now the quantities $d_1(x_j)$ and $d_2(x_j)$ can be cached and that (\ref{eqn:FastPam1-eqn}) no longer depends on $m$. \ilan{I don't see that right away}
This optimization reduces the complexity of PAM by $O(k)$ in each SWAP step, but only when the clusters are roughly similar in size, each containing about $O(\frac{1}{k})$ points \textbf{why is balanced cluster distro necessary? Eqn 8 doesn't suggest that}. 
In our algorithm, UltraPAM, we see a $O(\frac{N}{logN})$ speedup under relatively mild assumptions and do not require the clusters to be balanced. \ilan{not the best place to mention UltraPAM for the first time.}
Furthermore, it is possible to combine the FastPAM1 optimization with UltraPAM; indeed, we do so in our reference implementation available at \{githublink\}.

\martin{Use $\mathcal{C}$ font to denote sets.}

\martin{Could you double check \eqref{eqn:FastPam1-eqn}? I have a different answer. Divide the points into four categories based on which medoid it assigned to before and after the SWAP: 
\begin{itemize}
\item Before $m$ and after $x_i$; point set $C_m \cap C_{x_i}$; delta loss $d(x_i,x_j) - d_1(x_j)$.
\item Before $m$ and after other medoids; point set $C_m \cap C_{x_i}^c$; delta loss $d_2(x_j) - d_1(x_j)$.
\item Before other medoids and after $x_i$; point set $C_m^c \cap C_{x_i}$; delta loss $d(x_i,x_j) - d_1(x_j)$.
\item Before other medoids and other medoids; point set $C_m^c \cap C_{x_i}^c$; delta loss $0$.
\end{itemize}
Therefore, 
\begin{equation}
    \Delta L_{m, x_i}(x_j) = - d_1(x_j)\mathbbm{1}_{\{x_j \in C_m \cup C_{x_i}\}} + d(x_i, x_j)\mathbbm{1}_{\{x_j \in C_{x_i}\}} + d_2(x_j)\mathbbm{1}_{\{x_j \in C_{m}\cap C_{x_i}^c\}}
\end{equation}
}

\ilan{
I checked, and I agree with this.
In particular, if $x_j$'s previous closest medoid was some $m' \ne m$ and $d(x_j,m') < d(x_j,x_i)$, the delta should be 0. In this case, $x_j \notin C_m$, $x_j \notin C_{x_i}$, so equation (9) gives $d_2(x_j)$, while (10) gives 0.
} 

\martin{\eqref{eqn:FastPam1-eqn} is hard to follow. Add more details (like the one I mentioned above). }

\subsection{Theoretical Motivation: Multi-Armed Bandits}

Add description of MAB problem. Theory from the multi-armed bandit (MAB) literature suggests that best arm among $N$ arms can be found with $O(NlogN)$ \martin{$O(N\log N)$} arm pulls, as in the UCB algorithm \{citation\}. \martin{Be more precise here. Include the success probability $\delta$ and the gaps between the best arm and other arms $\delta \mu_i$ in the expression.} This observation motivates the approach presented in this paper, in which we use an adaptation of the UCB algorithm to find medoids more quickly. 

\ilan{we take too long to get here}

Intuitively, in the BUILD step, we consider each of the $N$ candidate datapoints as an "arm", where an arm pull corresponds to computing the induced loss on a single reference datapoint by choosing the candidate in question as a medoid.  The multi-armed bandit (MAB) literature then suggests that we can identify the best medoid to assign with $O(NlogN)$ distance computations in each of the $k$ BUILD steps.

Similarly, in the SWAP step, we consider each of the $k(N-k)$ medoid-nonmedoid pairs as an "arm", and an arm pull corresponds to computing the loss induced on a reference point by swapping the medoid with the non-medoid. The multi-armed bandit (MAB) literature then suggests that we can identify the best swap to perform with $O(kNlogN)$ distance computations in each SWAP step.

Intuitively, in each of the BUILD and SWAP steps, we convert the computation of the sum for each candidate $m_l$ in \ref{eqn:build-next-medoid} or $(m,x)$ in \ref{eqn:swap-td} into a sampling problem. Instead of computing the sums exactly, we compute confidence intervals that contain the sum with high probability and explore promising arms more while expending less computation on unpromising arms. We expect such a UCB-based approach to recover the true best arm, thus matching the results of the greedy algorithm PAM, with high probability.  We formally describe the algorithm in Section \ref{algo}, along with theoretical guarantees for correctness in Section \ref{theory}.

\subsection{Main Contributions}

In this work, we:

\begin{enumerate}
    \item Propose a new algorithm, UltraPAM, that uses a UCB-based algorithm to find a solution to the $k$-medoids problem,
    \item Provide theoretical guarantees as to when UltraPAM will return the same results as current state-of-the-art methods such as PAM, and
    \item Experimentally validate our approach on a number of real-world datasets.
\end{enumerate}

==> old/intro05-30.tex <==
% !TEX root = main.tex

% \martin{START of martin's version of Intro+Formulation}

% \martin{Introduction outline: 
% \begin{itemize}
%     \item Clustering is important and k-mean is one of the most popular clustering method. 
%     \item k-mean has two drawbacks.
%     \item First, it is only fast (linear for finding the centroid) when using $l_2^2$ or $l_1$ distance (the latter corresponds to k-median). However, for different applications, a different distance metric may be more appropriate (e.g. the editing distance for code.org)
%     \item Second, centroid is not a point in the dataset, while for some applications, having a representative for each cluster is important (e.g., a representative cell for single-cell RNA-seq)
%     \item Other clustering methods that allow for a user-defined distance matrix, like k-medoid, graph-based clustering methods (Louvain), requires precomputing of the distance matrix, which can be computationally and disk-space intensive. 
%     \item We consider an PAM  empirically preferable k-medoid algorithm PAM. (ref from wiki)
%     \item It is slow (need to quantify). We made it faster.
%     \item The algorithmic contributions are:
%     \item 1. We converted a deterministic computation problem into a random sampling problem, and used MAB to solve it. 
%     \item 2. The trick is to view each SWAP, instead of each data point, as an arm. 
%     \item 3. We adaptively chose the sub-Gaussian parameter for each stage and each arm to further increase speed. 
% \end{itemize}}

\section{Introduction}
\label{intro}

Clustering is a ubiquitous task in machine learning, whose goal is to partition a set of points into "clusters" such that points within each cluster are similar.
Many modern data science applications require clustering very-large-scale data, and for this reason, $k$-means clustering \cite{macqueen1967some,lloyd1982least} has been one of the most popular choices. 
In the clustering process, $k$-means clustering iterates over recalculating the center for each cluster and reassigning points to their nearest newly-calculated cluster centers. 
Central to its success is the specific choice of the cluster center; for a set of points, k-means defines the cluster center be the point which has the smallest average \emph{squared Euclidean distance} from all other points in the set. 
Under such a definition, the cluster center turns out to be the arithmetic mean of the set of points, which can be computed very efficiently.

% \martin{include k-medians here?} \ilan{I would say no. I like the flow as is}

While commonly used, $k$-means clustering suffers from several drawbacks. 
First, while it can efficiently compute the cluster center under the squared Euclidean distance, it is not straightforward to generalize to other distance metrics. 
However, for different applications, we may want to use a different distance to quantify the similarity between points. 
Some examples would be $l_1$ and cosine distance for sparse data like in recommendation systems \cite{leskovec2020mining} and in single-cell RNA-seq analysis \cite{ntranos2016fast}; or edit distance for text data \cite{navarro2001guided}; or graph metrics for social network data \cite{mishra2007clustering}. 
Second, the cluster center in $k$-means clustering is in geenral not a point in the dataset and may not be interpretable in many applications. This is especially true when the data is structured like in computer vision, or when it is sparse like in recommendation systems \cite{leskovec2020mining}.

As an alternative choice, $k$-medoids clustering algorithms \cite{kaufman1987clustering,kaufman1990partitioning} use \emph{medoid} to define the cluster center for a set of point. Given an arbitrary distance function, the medoid of a set of point is the point \emph{in the set} that minimizes the average distance to all the other points. So $k$-medoids clustering algorithms work for arbitrary distances. Moreover, unlike $k$-means, the cluster center in $k$-medoids, i.e., the medoid, is restricted to one of the points in the dataset, thus overcoming the second drawback of k-means clustering. 

% As an alternative choice, $k$-medoids clustering algorithms \cite{kaufman1987clustering,kaufman1990partitioning} work for arbitrary distances.
% For a set of points and a distance function, cluster center is defined as the \emph{medoid}, namely the point \emph{in the cluster} that minimizes the average distance to all the other points. Moreover, the medoid is, by definition, one of the points in the dataset, thus overcoming the second drawback of k-means clustering. 

% For $n$ data points $\mathcal{X} =  \{ x_1, x_2, \cdots, x_n \}$ and a distance function $d(\cdot, \cdot)$, the $k$-medoids problem aims to partition the data into $k$ disjoint clusters $\mathcal{C}_1,\cdots,\mathcal{C}_k$. Let $m_l$ be the medoid of cluster $\mathcal{C}_l$, namely
% \begin{equation}
%     m_l = \argmin_{m \in \mathcal{C}_l} \sum_{x_i \in \mathcal{C}_l} d(m, x_i),~~~~\text{for}~l=1,\cdots,k.
% \end{equation}
% The goal is to minimize the overall deviation of points from their medoids: 
% \begin{equation}
%     L =  \sum_{l=1}^k \sum_{x_i \in \mathcal{C}_l} d(m_l, x_i).
% \end{equation}

For $n$ data points $\mathcal{X} =  \{ x_1, x_2, \cdots, x_n \}$ and a user-specified distance function $d(\cdot, \cdot)$, the $k$-medoids problem aims to find a set of $k$ medoids $\mathcal{M} = \{m_1, \cdots, m_k \} \subset \mathcal{X}$ to minimize the overall deviation of points from their closest medoids:
\begin{equation} \label{eqn:total-loss}
	L(\mathcal{M}) =  \sum_{i=1}^n \min_{m_l \in \mathcal{M}} d(m_l, x_i)
\end{equation}
This problem is unfortunately NP-hard \cite{schubert2019faster}, and the partitioning around medoids (PAM) algorithm \cite{kaufman1987clustering, kaufman1990partitioning} is one of the most widely-used heuristic $k$-medoids clustering algorithm.
In the BUILD step, it aims to find a good initial set of $k$ medoids by greedily selecting one point at a time that minimizes the overall loss in \eqref{eqn:total-loss}. 
Then in the SWAP step, it considers all $k(n-k)$ possible medoid-and-non-medoid point pairs for swap and swap the pair that reduces the loss the most; it repeats such a step until no improvement can be made. 

% As one of the most-widely-used k-medoids clustering algorithm, the partitioning around medoids (PAM) algorithm \cite{kaufman1987clustering, kaufman1990partitioning} uses a different searching strategy.
% First in the BUILD step, it greedily selects $k$ of the $n$ data points as the medoids to minimize the cost, and assigns each point to its closest medoid. 
% Then in the SWAP step, it chooses, among all $k(n-k)$ medoid-and-non-medoid pairs, the pair that reduces the loss most, and swaps them. Such a step is repeated until no improvement can be made. 
% Since the SWAP step considers all medoid-and-non-medoid pairs and is a more global search, PAM produces empirically better results than the k-means-like algorithm \cite{reynolds2006clustering,schubert2019faster}. 

PAM has been empirically shown to produce satisfactory results among popular $k$-medoids clustering algorithms \cite{reynolds2006clustering,schubert2019faster}.  
However, it can be computationally challenging, especially for large-scale datasets. 
Indeed, each SWAP iteration takes $O(k(n-k)^2)$ distance evaluations, for computing the change of loss for each of the $k(n-k)$ medoid-and-non-medoid pairs with respect to the rest $n-k$ non-medoid points. 
BUILD step is equivalent to $O(k)$ SWAP steps.
Randomized algorithms like CLARA \cite{kaufman1990partitioning} and CLARANS \cite{ng2002clarans} have been proposed to improve computational efficiency, at the cost of deteriorated clustering quality.
More recently, Schubert et al. proposed a deterministic algorithm FastPAM \cite{schubert2019faster} that guarantees the same output as PAM but improves the complexity to $O(n^2)$ when the cluster sizes are similar. 
The factor $O(k)$ improvement is particularly important for large values of $k$.

% While CLARA and CLARANS usually produce lower-quality results than PAM, FastPAM is a deterministic algorithm that guarantees the same output as PAM but improves the complexity to $O(n^2)$ under the condition that the cluster sizes are similar. 
% This is achieved by exploiting the redundancy in the PAM computation and caching some share computations, including the distance of each point to its nearest and second nearest medoids. 

\paragraph{Contribution.} We propose \algnamenospace, a new randomized $k$-medoids algorithm that takes $O(???)$ for the BUILD step and $O( \min (f(k) n\log n, n^2)  )$ for each SWAP step, while returning the same result as PAM with high probability under reasonable assumptions of the data. 
For a fixed $k$, \algname takes $O(n \log n)$ distance evaluations for each SWAP step, effectively improving the PAM SWAP step from quadratic to almost-linear. 
\algname reduces to FastPAM for a large value of $k$. 
We also propose a variation \algaprname that slightly deviates from the PAM solution but has a much faster speed.
We experimentally validate our results on a number of real-world datasets, including Code.org Hour of Code, single-cell RNA-seq, and the MNIST handwritten digits datasets. We observe speedups of up to 50x in wall clock time over state-of-the-art algorithms. \martin{Update this paragraph after finishing the main paper}

The improvement is made by reformulating each step of PAM from a \emph{deterministic computational problem} to a \emph{statistical estimation problem}. 
Taking the SWAP step for example, we need to decide among $k(n-k)$ possible medoid-and-non-medoid swaps, which one has the smallest loss. 
If we swap, e.g., medoid $m_l$ and and non-medoid $x_i$, the new set of medoids after excluding $m_l$ and including $x_i$ would be $\mathcal{M}-\{m_l\} + \{x_i\}$,
and the corresponding loss:
\begin{equation} \label{eqn:sec_intro_swap_loss}
	L(m_l, x_i) = \sum_{j=1}^n \min_{m_l \in \mathcal{M}-\{m_l\} + \{x_i\}} d(m_l, x_j) \overset{\text{def}}{=} \sum_{j=1}^n g(x_j),
\end{equation}
where $g(\cdot)$ is a function that depends on $\mathcal{M}$, $m_l$, $x_i$.
Eq. \eqref{eqn:sec_intro_swap_loss} shows that the loss of a swap $L(m_l, x_i)$ be can written as the summation of the function value $g(\cdot)$, evaluated on all $n$ points. 
Therefore, $L(m_l, x_i)$ can be estimated by evaluating on a randomly sampled $n'$<$n$ points, and the estimation accuracy depends on the size of the subsample $n'$. 

Recall that the goal of the SWAP step is to find the medoid-and-non-medoid swap with the smallest loss, which is different from computing the exact loss for every possible swap. 
So an estimation of the best swap with high confidence would suffice. 
Intuitively,  promising swaps with smaller loss should be estimated with a higher accuracy and less promising ones can be discarded without being evaluated on too many randomly-sampled data points. 

To design the adaptive sampling strategy, we show that both the BUILD step and each of the SWAP step can be formulated as a separate best-arm identification problem in the multi-armed bandits (MAB) \cite{audibert2010best,even2002pac,jamieson2014lil,jamieson2014best}. 
In a typical setting of the best-arm identification problem, we have $m$ arms. At time $t$=$0,1,\cdots,$ we decide to pull an arm $A_t\in \{1,\cdots,m\}$, and receive a reward $R_t$ with $E[R_t] = \mu_{A_t}$ . The goal is to identify the arm with the largest expected reward with high probability while pulling as few arms as possible.
In the context of the PAM SWAP step, we can think of each possible medoid-and-non-medoid swap as an arm, totaling $k(n-k)$ arms. The arm parameter corresponds to the loss of the swap, and by pulling an arm, we observed the loss evaluated on a randomly-sampled data point. 
Then, the best swap can be estimated using existing best-arm algorithms like the Upper Confidence Bound (UCB) Algorithm \cite{lai1985asymptotically}.


% (Kalyanakrishnan et al., 2012; Chen et al., 2017; Simchowitz
% et al., 2017) aims to identify the best k arms via adaptive
% sampling. For AMT, we can think of the m null hypotheses
% as arms, fMC p-values as arm parameters, and MC samples
% as observations for each arm. Then recovering the fMC
% result corresponds to identifying a subset of best arms with
% small p-values. The difference is that the size of this subset
% is not known ahead of time — it is a function of the fMC
% p-values that needs to be learned from data. Nonetheless,
% the techniques in MAB is borrowed to develop AMT.



% which can be solved using existing algorithms like the Upper Confidence Bound (UCB) Algorithm \cite{lai1985asymptotically}.


% The specific adaptive sampling procedure is developed via
% a connection to the pure exploration problem in multiarmed bandits (MAB) (Audibert & Bubeck, 2010; Jamieson
% et al., 2014). Specifically, the top-k identification problem
% (Kalyanakrishnan et al., 2012; Chen et al., 2017; Simchowitz
% et al., 2017) aims to identify the best k arms via adaptive
% sampling. For AMT, we can think of the m null hypotheses
% as arms, fMC p-values as arm parameters, and MC samples
% as observations for each arm. Then recovering the fMC
% result corresponds to identifying a subset of best arms with
% small p-values. The difference is that the size of this subset
% is not known ahead of time — it is a function of the fMC
% p-values that needs to be learned from data. Nonetheless,
% the techniques in MAB is borrowed to develop AMT.

% The specific procedure is designed via a connection to the best-arm identification problem in the multi-armed bandits (MAB) literature \cite{audibert2010best,even2002pac,jamieson2014lil,jamieson2014best}. 
% Specifically, we show that both the BUILD step and each of the SWAP step can be formulated as a separate best-arm identification problem, which can be solved using existing algorithms like the Upper


% , hence motivating the adaptive estimation procedure. 



% since the goal is the find the medoid-and-non-medoid pair that has the smallest loss, promising pairs with smaller loss should be estimated with a higher accuracy and less promising ones can be discarded without being evaluated on too many reference points, hence motivating the adaptive estimation procedure. 

% The specific procedure is designed via a connection to the best-arm identification problem in the multi-armed bandits (MAB) literature \cite{audibert2010best,even2002pac,jamieson2014lil,jamieson2014best}. 
% Specifically, we show that both the BUILD step and each of the SWAP step can be formulated as a separate best-arm identification problem, which can be solved using existing algorithms like the Upper Confidence Bound (UCB) Algorithm \cite{lai1985asymptotically}.

\subsection{Related works}

k-means clustering is one of the \emph{centroid}-based clustering algorithms, where the centroid of a set of point for a distance metric is defined as the point \emph{in the space} that minimizes the overall distance from other points. So the key difference between centroid and medoid is that centroid needs not be one of the points in the set. 
k-means uses centroid for squared Euclidean distance to define the cluster center, which is the arithmetic mean and can be computed in linear time. 
Centroid for Bregman divergence is also the arithmetic mean and centroid for $l_1$ distance is the component-wise median; the latter is used by the $k$-medians clustering algorithm \cite{bradley1997clustering,jain1988algorithms}.
However, centroid for other distances are hard to compute.
For example, centroid for the unsquared Euclidean distance corresponds to the much harder Weber problem with no closed-form solution \cite{bradley1997clustering,overton1983quadratically}. 
\martin{Maybe delete this paragraph if we don't have enough space}

For other k-medoids clustering algorithms, Park et al. \cite{park2009simple} proposed a k-means-like algorithm that iterates over recalculating the medoid for each cluster and reassigning the points to their closest newly-calculated medoid, until the total deviation can no longer be improved.
However, it has been empirically shown to produce less satisfactory results than PAM \cite{reynolds2006clustering,schubert2019faster}. 
Other proposals include optimizations for Euclidean space and tabu search heuristics \cite{estivill2001robust}.

The idea of algorithm acceleration by converting a computational problem into a statistical estimation problem and designing the adaptive sampling procedure via MAB has
witnessed a few successes,  including in Monte Carlo tree search \cite{chang2005adaptive,kocsis2006bandit}, hyper-parameter tuning \cite{li2016hyperband,jamieson2016non}, discrete optimization \cite{bagaria2018adaptive}, and permutation-based multiple testing \cite{zhang2019adaptive}. 
In the context of $k$-medoids clustering, previous works \cite{bagaria2018medoids,baharav2019ultra} have considered finding the medoid of a set points, which can be regarded of as the $1$-medoid problem.
They also formulate the problem as a best-arm identification problem, treating each point as an arm and its average distance to other points as the arm parameter. 
However, it is not straighforward to generalize the $1$-medoid problem to $k$-medoid problem.
Instead of having one best-arm identification problem, we reformulated PAM into a sequence of best-arm problems, treating different objects as the arm in different steps of PAM: each point is treated as an arm in the BUILD step and each medoid-and-non-medoid swap is treated as an arm in the SWAP step. 
As demonstrated in the later part the paper, the intrinsic difficulty of different best-arm problems are different, and we can adapt to this to make significant improvement.   

% Recall that the medoid is used to define the cluster center in k-medoids clustering.  Perhaps a straightforward heuristic solution is a k-means-like k-medoids clustering algorithm, which iterates over recalculating the medoid for each cluster and reassigning the points to their closest newly-calculated medoid, until the total deviation can no longer be improved \cite{reynolds2006clustering,park2009simple}. 
% This algorithm is computationally efficient, but has been empirically shown to produce less satisfactory results \cite{reynolds2006clustering,schubert2019faster}, possibly because the discrete nature of medoids makes it more likely to stuck in a suboptimal local minimum. 

% Randomized algorithms have been proposed to trade clustering quality for runtime. 
% CLARA \cite{kaufman1990partitioning} repeatedly applies PAM on a subset of $n' \ll n$ points to get the $k$ medoids and assigns the rest of points to their closest medoid; it then returns the result from the best run. With the recommendation $n' = 40+2k$, the runtime becomes $O(k^3)$ for each iteration, a great improvement for small $k$. 
% CLARANS \cite{ng2002clarans} randomly searches over all medoid-and-non-medoid swaps from the current solution and follows the first swap that reduces the loss; it repeats the procedure until no improvement can be made with $p$=$1.25\%k(n-k)$ attempts. 


% Taking the SWAP step for example, we can view each medoid-and-non-medoid pair $(m_l, x_i)$ as a arm, with the arm parameter the change of loss it will iccur:  


% . BanditPAM is a randomized algorithm based on a connection with the multi-armed bandit problem. We theoretically prove that Bandit-PAM tracks the exact optimization path of PAM and returns the same result with high probability. We experimentally validate our results on a number of real-world datasets, including code.org submission data, single-cell RNA-seq data, and MNIST handwritten digits data. We observe speedups up to 50x in wall clock time over state-of-the-art algorithms. \martin{Need to be precise here, with high probability, quadratic in $k$}. 


% The original PAM algorithm \cite{kaufman1987clustering,kaufman1990partitioning} consists of two algorithms, BUILD to choose an initial clustering, and the SWAP stage to further optimize the clustering towards a local optimum. The BUILD step takes $O(n^2k)$ time, while each iteration of the SWAP step takes $O((n-k)^2k)$. \martin{FASTPAM takes ..., CLARANS takes....}. 

\section{Problem formulation}

\subsection{Formal $k$-medoids Problem Statement}
Formally, let $\mathcal{X} =  \{ x_1, x_2, \cdots, x_N \}$ be a set of $N$ points in $d$ dimensions, $k$ be the number of clusters to find, and $d(\cdot, \cdot)$, a distance function. For a given set of $k$ medoids $\mathcal{M} = \{m_1, \cdots, m_k \} \subset \mathcal{X}$, the objective function of the $k$-medoids problem is the sum of distances from each point to its closest medoid: \martin{Both $N$ and $n$ are used to denote the number of data points. I suggest to consistently use $n$ because other quantities like $d$ and $k$ are both lower-case.} \martin{$d$ was used to denote both the number of dimensions and the distance metric. Schubert et al. 2018 also overloaded $d$, but this hurts clarity. Maybe changing the distance function to $dist$?}
\begin{equation}
\label{eqn:total-loss}
	L(\mathcal{M}) =  \sum_{i=1}^n \min_{m_l \in \mathcal{M}} d(m_l, x_i)
\end{equation}

The $k$-medoids problem is then to determine the optimal assignment of medoids $\mathcal{M}$, i.e. $\argmin_{\mathcal{M}}L({\mathcal{M}})$

Note that while $d$ is often a distance metric such as $L_2$ distance, it need not be so; in fact, any arbitrary dissimilarity metric (even an asymmetric one) could be provided above. In general, this problem is NP-Hard \ref{citation}. As such, this problem is generally tackled with greedy iterative algorithms, which we discuss Section \ref{priorwork}.

\subsection{Comparison to $k$-means}

At first glance, the problem specification of $k$-medoids may appear very similar to $k$-means, where a similar objective function is used:

\begin{equation}
\label{eqn:total-loss-means}
	L_{kmeans}(\{\mu_1, \dots, \mu_k\}) =  \sum_{i=1}^n \min_{\mu \in \{\mu_1, \dots, \mu_k\}} ||d(\mu, x_i)||^2
\end{equation}

Crucially, however, in $k$-means the optimization of $L_{kmeans}$ is performed over all possible sets of vectors $U = \{\mu_1, \dots, \mu_k\} \subset \mathbb{R}^d$ and the means $\mu_i$ are not required to be actual datapoints. \martin{Use text format for subscript that is not a variable, e.g. $L_{\text{kmeans}}$.}

Naturally, one might ask if we could reduce the $k$-medoids problem to the $k$-means problem by choosing the medoids to be the real datapoints closest to the means $\{\mu_1, \dots, \mu_k\}$. However, this approach is more susceptible to outliers due to the squaring of the individual loss terms in \ref{eqn:total-loss-means} and will not return the same results as the $k$-medoids problem. It is straightforward to construct small examples where the results of this approach disagree with the solution of the $k$-medoids problem. In fact, it is well-known that $k$-means is more susceptible to noise and outliers than $k$-medoids \ref{citation}.

In the $k$-means algorithm, $d$ in Equation \ref{eqn:total-loss-means} is usually $L_2$ distance. For completeness, we also mention the \textbf{$k$-medians} problem, in which $d$ is instead the $L_1$ distance, which is less susceptible to noise and outliers than the usual $L_2$ distance. This (rather specific) problem permits an EM-style decomposition which results in an algorithmic complexity similar to the one shown in this paper \ref{citation}; however, the loss function being optimized is different from that in the $k$-medoids problem. Furthermore, the approach presented in our work applies more generally to arbitrary $d$, even those which are not metrics such as $L_1$ or other popular metrics.

\ilan{The paragraph above is not very clear to me. Are we sure that $k$-medians is generally understood to be $k$-means with $L_1$ instead $L_2$ distances?}

% \section{Prior Work} \martin{Put prior work as a subsection of the Introduction section}
% \label{priorwork}

\subsection{Partitioning Around Medoids (PAM)}
The $k$-medoids problem is, in general, NP-hard. As such, iterative greedy algorithms are often used.  The state-of-the-art algorithm for the $k$-medoids problem, Partitioning Around Medoids (PAM), takes a greedy approach, divided into two steps: BUILD and SWAP. In the BUILD step, medoids are initialized one-by-one by choosing each new medoid to be the one that would lower the loss (Equation \ref{eqn:total-loss}) the most. In the SWAP step, we consider swapping each of the medoid assignments with a non-medoid and perform the swap which would lower the loss (Equation \ref{eqn:total-loss}) the most. The BUILD step is run once and then the SWAP step is run multiple times until convergence.

\subsubsection{PAM BUILD step}
In the BUILD step, each of the medoids is greedily initialized by choosing the $l$th medoid, conditioned on the previous $l-1$ medoids, that reduces the total loss of every other point. 
\ilan{}
More formally, suppose the current set of medoids is $\mathcal{M} = \{m_1, \cdots, m_{l-1}\}$ and we wish to add the $l$th medoid $m_l$. Our goal is to identify a new medoid $m_l$ such that:

\begin{equation}
\label{eqn:build-next-medoid}
    m_l = \argmin_{x \in \mathcal{X} \setminus \mathcal{M}} \sum_{j=1}^n \min[d(x, x_j), \min_{m' \in \mathcal{M}} d(m', x_j)]. 
\end{equation}

Equivalently, we can find the find $m_l$ that minimizes the change in total loss:

\begin{equation}
\label{eqn:build-next-medoid-td}
    m_l = \argmin_{x \in \mathcal{X} \setminus \mathcal{M}} \sum_{j=1}^n  \Delta L_{x}(x_j)
\end{equation}

where

\begin{equation}
\label{eqn:build-td}
    \Delta L_{x}(x_j) = \min[d(x, x_j) - \min_{m' \in \mathcal{M}} d(m', x_j), 0]
\end{equation}

\ilan{Should we instead be defining the change to be positive? 
Saying ``minimizes the change in total loss'' sounds a bit weird to me, because it sounds like you want to make as little change as possible.}

represents the change in total loss for reference point $x_j$ induced by choosing $x$ as a new medoid. \martin{$\Delta L_{x}(x_j)$ is not well-defined because the dependency on $\mathcal{M}$ was omitted. How about $\Delta L_{x, \mathcal{M}}(x_j)$?} 

Computing $m_l$ from Equation \ref{eqn:build-next-medoid} \martin{Use \eqref{eqn:build-next-medoid}} requires computing $d$ for each candidate point $x \in \mathcal{X}\setminus\mathcal{M}$ to each other point in the dataset -- an $O(N^2)$ operation. Furthermore, this process must be repeated for each of the $k$ initial medoid assignments. As such, the PAM BUILD step requires $O(kN^2)$ computations of the distance function $d$; this is prohibitively expensive for complicated choices of $d$ such as Wasserstein distance.
\ilan{Maybe ``This is prohibitively expensive when the data is very high dimensional or for complicated choices of $d$ such as the Wasserstein distance.'' We don't want to give the impression that this is only relevant for non-trivial distances}

\subsubsection{PAM SWAP Step}
In the SWAP step, we consider swapping the assignment of any of the $k$ medoids with any of the $N-k$ non-medoids. For each of the possible $k(N-k)$ swaps, we calculate the total change in loss for each of the $N$ datapoints. We then perform the swap that would lower the total loss for the dataset. 

Specifically, our goal is to find a medoid-nonmedoid pair $(m^*, x^*)$ such that:

\begin{equation}
\label{eqn:next-swap}
    (m^*, x^*) = \argmin_{(m,x) \in \mathcal{M} \times (\mathcal{X} \setminus \mathcal{M}) } \sum_{j=1}^n \min[d(x, x_j), \min_{m' \in \mathcal{M}\setminus \{m\}} d(m', x_j)]. 
\end{equation}

Equivalently, we can find $(m^*, x^*)$ that minimizes:

\begin{equation}
\label{eqn:next-swap-td}
    (m^*, x^*) = \argmin_{(m,x) \in \mathcal{M} \times (\mathcal{X} \setminus \mathcal{M}) } \sum_{j=1}^n \Delta L_{m, x_i}(x_j)
\end{equation}

where

\begin{equation}
\label{eqn:swap-td}
    \Delta L_{m, x_i}(x_j) = \min[d(x_i, x_j) - \min_{m' \in \mathcal{M}\setminus \{m\}} d(m', x_j), 0]
\end{equation}

represents the induced change in loss for point $x_j$ by removing $m$ from the list of medoids and choosing $x_i$ as a new medoid. \martin{$\Delta L_{m, x_i}(x_j)$ is not well-defined because the dependency on $\mathcal{M}$ was omitted. How about $\Delta L_{m, x_i,\mathcal{M}}(x_j)$? Also, this is very similar to the $\Delta L$ in the BUILD step. Consider changing them to $\Delta L^{\text{BUILD}}$ and $\Delta L^{\text{SWAP}}$ for clarity.} 

The SWAP step is iterated until convergence. Similar to the BUILD step, each SWAP step requires $O(kN^2)$ distance computations, which is prohibitively expensive for complicated choices of $d$.

\subsection{FastPAM1}

Accelerating the PAM algorithm is an active area of research. Perhaps most closely related to our work is \ref{FastPAM}, which presents three independent optimizations to the original PAM algorithm. Of these three, only one (dubbed FastPAM1) optimization applied to the SWAP step, preserves the results as the original PAM algorithm.

In the FastPAM1 optimization, the distance from each point $x_j$ to its nearest medoid, $d_1(x_j)$, and to its \textit{second nearest} medoid, $d_2(x_j)$ is used to rewrite \ref{eqn:swap-td} \martin{\eqref{eqn:swap-td}} as:

\begin{equation}
\label{eqn:FastPam1-eqn}
    \Delta L_{m, x_i}(x_j) = - d_1(x_j)\mathbbm{1}_{x_j \in C_m} + d(x_i, x_j)\mathbbm{1}_{x_j \in C_{x_i}} + d_2(x_j)\mathbbm{1}_{x_j \notin C_{x_i}}
\end{equation}

\ilan{I find the notation with $x_i$ and $x_j$ a bit confusing. It's a bit weird that $m$ and $x_i$ are the things being swapped, while $x_j$ is just a general point}

where $C_m$ is the set of points assigned to medoid $m$ before the swap, and $C_{x_i}$ is the set of points that would be assigned to the new medoid $x_i$ if the swap were performed. 
Note that now the quantities $d_1(x_j)$ and $d_2(x_j)$ can be cached and that (\ref{eqn:FastPam1-eqn}) no longer depends on $m$. \ilan{I don't see that right away}
This optimization reduces the complexity of PAM by $O(k)$ in each SWAP step, but only when the clusters are roughly similar in size, each containing about $O(\frac{1}{k})$ points \textbf{why is balanced cluster distro necessary? Eqn 8 doesn't suggest that}. 
In our algorithm, UltraPAM, we see a $O(\frac{N}{logN})$ speedup under relatively mild assumptions and do not require the clusters to be balanced. \ilan{not the best place to mention UltraPAM for the first time.}
Furthermore, it is possible to combine the FastPAM1 optimization with UltraPAM; indeed, we do so in our reference implementation available at \{githublink\}.

\martin{Use $\mathcal{C}$ font to denote sets.}

\martin{Could you double check \eqref{eqn:FastPam1-eqn}? I have a different answer. Divide the points into four categories based on which medoid it assigned to before and after the SWAP: 
\begin{itemize}
\item Before $m$ and after $x_i$; point set $C_m \cap C_{x_i}$; delta loss $d(x_i,x_j) - d_1(x_j)$.
\item Before $m$ and after other medoids; point set $C_m \cap C_{x_i}^c$; delta loss $d_2(x_j) - d_1(x_j)$.
\item Before other medoids and after $x_i$; point set $C_m^c \cap C_{x_i}$; delta loss $d(x_i,x_j) - d_1(x_j)$.
\item Before other medoids and other medoids; point set $C_m^c \cap C_{x_i}^c$; delta loss $0$.
\end{itemize}
Therefore, 
\begin{equation}
    \Delta L_{m, x_i}(x_j) = - d_1(x_j)\mathbbm{1}_{\{x_j \in C_m \cup C_{x_i}\}} + d(x_i, x_j)\mathbbm{1}_{\{x_j \in C_{x_i}\}} + d_2(x_j)\mathbbm{1}_{\{x_j \in C_{m}\cap C_{x_i}^c\}}
\end{equation}
}

\ilan{
I checked, and I agree with this.
In particular, if $x_j$'s previous closest medoid was some $m' \ne m$ and $d(x_j,m') < d(x_j,x_i)$, the delta should be 0. In this case, $x_j \notin C_m$, $x_j \notin C_{x_i}$, so equation (9) gives $d_2(x_j)$, while (10) gives 0.
} 

\martin{\eqref{eqn:FastPam1-eqn} is hard to follow. Add more details (like the one I mentioned above). }

\subsection{Theoretical Motivation: Multi-Armed Bandits}

Add description of MAB problem. Theory from the multi-armed bandit (MAB) literature suggests that best arm among $N$ arms can be found with $O(NlogN)$ \martin{$O(N\log N)$} arm pulls, as in the UCB algorithm \{citation\}. \martin{Be more precise here. Include the success probability $\delta$ and the gaps between the best arm and other arms $\delta \mu_i$ in the expression.} This observation motivates the approach presented in this paper, in which we use an adaptation of the UCB algorithm to find medoids more quickly. 

\ilan{we take too long to get here}

Intuitively, in the BUILD step, we consider each of the $N$ candidate datapoints as an "arm", where an arm pull corresponds to computing the induced loss on a single reference datapoint by choosing the candidate in question as a medoid.  The multi-armed bandit (MAB) literature then suggests that we can identify the best medoid to assign with $O(NlogN)$ distance computations in each of the $k$ BUILD steps.

Similarly, in the SWAP step, we consider each of the $k(N-k)$ medoid-nonmedoid pairs as an "arm", and an arm pull corresponds to computing the loss induced on a reference point by swapping the medoid with the non-medoid. The multi-armed bandit (MAB) literature then suggests that we can identify the best swap to perform with $O(kNlogN)$ distance computations in each SWAP step.

Intuitively, in each of the BUILD and SWAP steps, we convert the computation of the sum for each candidate $m_l$ in \ref{eqn:build-next-medoid} or $(m,x)$ in \ref{eqn:swap-td} into a sampling problem. Instead of computing the sums exactly, we compute confidence intervals that contain the sum with high probability and explore promising arms more while expending less computation on unpromising arms. We expect such a UCB-based approach to recover the true best arm, thus matching the results of the greedy algorithm PAM, with high probability.  We formally describe the algorithm in Section \ref{algo}, along with theoretical guarantees for correctness in Section \ref{theory}.

\subsection{Main Contributions}

In this work, we:

\begin{enumerate}
    \item Propose a new algorithm, \algnamenospace, that uses a UCB-based algorithm to find a solution to the $k$-medoids problem,
    \item Provide theoretical guarantees as to when UltraPAM will return the same results as current state-of-the-art methods such as PAM, and
    \item Experimentally validate our approach on a number of real-world datasets.
\end{enumerate}


% \martin{END of martin's version of Intro+Formulation}

==> old/intro06-02.tex <==
% !TEX root = main.tex

% \martin{START of martin's version of Intro+Formulation}

% \martin{Introduction outline: 
% \begin{itemize}
%     \item Clustering is important and k-mean is one of the most popular clustering method. 
%     \item k-mean has two drawbacks.
%     \item First, it is only fast (linear for finding the centroid) when using $l_2^2$ or $l_1$ distance (the latter corresponds to k-median). However, for different applications, a different distance metric may be more appropriate (e.g. the editing distance for code.org)
%     \item Second, centroid is not a point in the dataset, while for some applications, having a representative for each cluster is important (e.g., a representative cell for single-cell RNA-seq)
%     \item Other clustering methods that allow for a user-defined distance matrix, like k-medoid, graph-based clustering methods (Louvain), requires precomputing of the distance matrix, which can be computationally and disk-space intensive. 
%     \item We consider an PAM  empirically preferable k-medoid algorithm PAM. (ref from wiki)
%     \item It is slow (need to quantify). We made it faster.
%     \item The algorithmic contributions are:
%     \item 1. We converted a deterministic computation problem into a random sampling problem, and used MAB to solve it. 
%     \item 2. The trick is to view each SWAP, instead of each data point, as an arm. 
%     \item 3. We adaptively chose the sub-Gaussian parameter for each stage and each arm to further increase speed. 
% \end{itemize}}

\section{Introduction}
\label{intro}

Clustering is a ubiquitous task in machine learning, whose goal is to partition a set of points into "clusters" such that points within each cluster are similar. \mo{Is this too general of a starting point?}
Many modern data science applications require clustering very-large-scale data, and for this reason, $k$-means clustering \cite{macqueen1967some,lloyd1982least} has been one of the most popular choices because of its computational efficiency.
% \mo{Not clear to me that large scale data makes $k$-means popular -- maybe just say $k$-means is a popular example method?}
In the clustering process, $k$-means clustering alternates between reassigning points to their nearest cluster centers and recomputing those centers. 
% \mo{$k$-means "alternates between reassigning points to their nearest cluster centers and recomputing those centers"}
Central to its success is the specific choice of the cluster center; for a set of points, $k$-means defines the cluster center be the point which has the smallest average \emph{squared Euclidean distance} from all other points in the set. 
Under such a definition, the cluster center turns out to be the arithmetic mean of the set of points, which can be computed efficiently. 
% \mo{remove the word "very"?}

% \martin{include k-medians here?} \ilan{I would say no. I like the flow as is}

While commonly used in practice, $k$-means clustering suffers from several drawbacks. 
First, while it can efficiently compute the cluster center under the squared Euclidean distance, it is not straightforward to generalize to other distance metrics. 
However,
% \mo{replace "However" with "Indeed"?} 
for different applications, we may want to use a different distance to quantify the similarity between points. 
Some examples would be $l_1$ and cosine distance for sparse data like in recommendation systems \cite{leskovec2020mining} and in single-cell RNA-seq analysis \cite{ntranos2016fast}; or edit distance for text data \cite{navarro2001guided}; or graph metrics for social network data \cite{mishra2007clustering}. 
Second, the cluster center in $k$-means clustering is in general not a point in the dataset and may not be interpretable in many applications. This is especially problematic when the data is structured like in computer vision, or when it is sparse like in recommendation systems \cite{leskovec2020mining}.

As an alternative choice, $k$-medoids clustering algorithms \cite{kaufman1987clustering,kaufman1990partitioning} use the \emph{medoid} to define the cluster center for a set of point. Given an arbitrary distance function, the medoid of a set of point is the point \emph{in the set} that minimizes the average distance to all the other points.
Note that the distance metric can be arbitrary; indeed, it needs not be a metric and could be an asymmetric dissimilarity measure
% So $k$-medoids clustering algorithms work for arbitrary distances \mo{I think this sentence can be changed to "Note that the distance metric can be arbitrary; indeed, it need not be a metric at all and could be an asymmetric dissimilarity measure"}. 
Moreover, unlike $k$-means, the cluster center in $k$-medoids, i.e., the medoid, is restricted to one of the points in the dataset, thus addressing the second drawback of k-means clustering. 

For $n$ data points $\mathcal{X} =  \{ x_1, x_2, \cdots, x_n \}$ and a user-specified distance function $d(\cdot, \cdot)$, the $k$-medoids problem aims to find a set of $k$ medoids $\mathcal{M} = \{m_1, \cdots, m_k \} \subset \mathcal{X}$ to minimize the overall distance of points from their closest medoids: 
\begin{equation} \label{eqn:sec_intro_total-loss}
	L(\mathcal{M}) =  \sum_{i=1}^n \min_{m_l \in \mathcal{M}} d(m_l, x_i)
\end{equation}
This problem is unfortunately NP-hard in general \cite{schubert2019faster}.
% \mo{in general. The Partionining Around Medoids...}., and the
The partitioning around medoids (PAM) algorithm \cite{kaufman1987clustering, kaufman1990partitioning} is one of the most widely-used heuristic $k$-medoids clustering algorithm.
In the BUILD step, it aims to find a good initial set of $k$ medoids by greedily selecting one point at a time that minimizes the overall loss in \eqref{eqn:sec_intro_total-loss}. 
Then in the SWAP step, it considers all $k(n-k)$ possible pairs of  medoid and non-medoid points, and swaps the pair that reduces the $k$-medoids clustering loss the most; it repeats such a step until no improvement can be made. 

PAM has been empirically shown to produce satisfactory results among popular $k$-medoids clustering algorithms \cite{reynolds2006clustering,schubert2019faster}.  
However, it can be computationally challenging, especially for large-scale datasets. 
Indeed, each SWAP iteration takes $O(k(n-k)^2)$ distance evaluations, for computing the change of loss for each of the $k(n-k)$ medoid-and-non-medoid pairs with respect to the rest $n-k$ non-medoid points. 
BUILD step is equivalent to one SWAP step.
Randomized algorithms like CLARA \cite{kaufman1990partitioning} and CLARANS \cite{ng2002clarans} have been proposed to improve computational efficiency, at the cost of deteriorated clustering quality.
More recently, Schubert et al. proposed a deterministic algorithm FastPAM \cite{schubert2019faster} that guarantees the same output as PAM but improves the complexity to $O(n^2)$ when the cluster sizes are similar. 
The factor $O(k)$ improvement is particularly important for large values of $k$.

\paragraph{Contribution.} We propose \algnamenospace, a new randomized $k$-medoids algorithm that takes \mo{$O(kn^2)$} \martin{thought we also have an improvement in BUILD step, no?} for the BUILD step and $O(  n^2 \wedge f(k) n \log n )$ for each SWAP step, while returning the same result as PAM with high probability under reasonable assumptions of the data. 
For a fixed $k$, \algname takes $O(n \log n)$ distance evaluations for each SWAP step, effectively improving the PAM SWAP step from quadratic to almost linear. 
\algname reduces to FastPAM for a large value of $k$. 
We also propose a variation \algaprname that slightly deviates from the PAM solution but has a much faster speed.
We experimentally validate our results on a number of real-world datasets, including Code.org Hour of Code, single-cell RNA-seq, and the MNIST handwritten digits datasets. We observe speedups of up to 50x in wall clock time over state-of-the-art algorithms. \martin{Update this paragraph after finishing the main paper}

The improvement is made by reformulating each step of PAM from a \emph{deterministic computational problem} to a \emph{statistical estimation problem}. 
In the SWAP step, for example, we need to decide among $k(n-k)$ possible medoid-and-non-medoid swaps, which one has the smallest loss. 
If we swap, e.g., medoid $m_l$ and and non-medoid $x_i$, the new set of medoids after excluding $m_l$ and including $x_i$ would be $\mathcal{M}-\{m_l\} + \{x_i\}$,
and the corresponding loss:
\begin{equation} \label{eqn:sec_intro_swap_loss}
	L(m_l, x_i; \mathcal{M}) = \sum_{j=1}^n \min_{m_l \in \mathcal{M}-\{m_l\} + \{x_i\}} d(m_l, x_j) \overset{\text{def}}{=} \sum_{j=1}^n g(x_j),
\end{equation}
where $g(\cdot)$ is a function that depends on $\mathcal{M}$, $m_l$, $x_i$.
Eq. \eqref{eqn:sec_intro_swap_loss} shows that the loss of a swap $L(m_l, x_i; \mathcal{M})$ be can written as the summation of the function value $g(\cdot)$, evaluated on all $n$ points. 
Therefore, $L(m_l, x_i; \mathcal{M})$ can be estimated by evaluating the function on a randomly sampled subset of $n' < n$ points, where the estimation accuracy depends on the size of the subsample $n'$. 

Recall that the goal of the SWAP step is to find the medoid-and-non-medoid swap with the smallest loss, which is different from computing the exact loss for every possible swap. 
So an estimation of the best swap with high confidence would suffice. 
Intuitively,  promising swaps with smaller loss should be estimated with a higher accuracy and less promising ones can be discarded without being evaluated on too many randomly-sampled data points. 

To design the adaptive sampling strategy, we show that both the BUILD step and each of the SWAP step can be formulated as a separate best-arm identification problem in the multi-armed bandits (MAB) literature \cite{audibert2010best,even2002pac,jamieson2014lil,jamieson2014best}. 
In a typical setting of the best-arm identification problem, we have $m$ arms. At time $t = 0,1,\cdots,$ we decide to pull an arm $A_t\in \{1,\cdots,m\}$, and receive a reward $R_t$ with $E[R_t] = \mu_{A_t}$ . The goal is to identify the arm with the largest expected reward with high probability while pulling as few arms as possible.
In the context of the PAM SWAP step, we can think of each possible medoid-and-non-medoid swap as an arm in the best-arm problem, totaling $k(n-k)$ arms. The arm parameter corresponds to the loss of the swap, and by pulling an arm, we observe the loss evaluated on a randomly-sampled data point. 
Then, the best swap can be estimated using existing best-arm algorithms like the Upper Confidence Bound (UCB) algorithm \cite{lai1985asymptotically}.

\subsection{Related works}

k-means clustering is one of the \emph{centroid}-based clustering algorithms, where the centroid of a set of point for a distance metric is defined as the point \emph{in the space}
% \mo{"among the datapoints"?}
that minimizes the overall distance from other points. So the key difference between centroid and medoid is that centroid needs not be one of the points in the set. 
k-means uses centroid for squared Euclidean distance to define the cluster center, which is the arithmetic mean and can be computed in linear time. 
Centroid for Bregman divergence is also the arithmetic mean and centroid for $l_1$ distance is the component-wise median; the latter is used by the $k$-medians clustering algorithm \cite{bradley1997clustering,jain1988algorithms}.
However, centroid for other distances is hard to compute.
For example, centroid for the unsquared Euclidean distance corresponds to the much harder Weber problem with no closed-form solution \cite{bradley1997clustering,overton1983quadratically}. 
\martin{Maybe delete this paragraph if we don't have enough space}

For other k-medoids clustering algorithms, Park et al. \cite{park2009simple} proposed a $k$-means-like algorithm that alternates between reassigning the points to their closest medoid and recomputing the medoid for each cluster, until the $k$-medoids clustering loss can no longer be improved.
However, it has been empirically shown to produce less satisfactory results as compared to PAM \cite{reynolds2006clustering,schubert2019faster}. 
Other proposals include optimizations for Euclidean space and tabu search heuristics \cite{estivill2001robust}.

The idea of algorithm acceleration by converting a computational problem into a statistical estimation problem and designing the adaptive sampling procedure via MAB has
witnessed a few successes,  including in Monte Carlo tree search \cite{chang2005adaptive,kocsis2006bandit}, hyper-parameter tuning \cite{li2016hyperband,jamieson2016non}, discrete optimization \cite{bagaria2018adaptive}, and permutation-based multiple testing \cite{zhang2019adaptive}. 
In the context of $k$-medoids clustering, previous works \cite{bagaria2018medoids,baharav2019ultra} have considered finding the medoid of a set points, namely the $1$-medoid problem.
In these works. the problem was also formulated as a best-arm identification problem, with each point being arm and its average distance to other points being the arm parameter. 

First, while the $1$-medoid problem can be solved exactly, the $k$-medoids problem is harder and can only rely on heuristic solutions. We hence focus on improving the computational efficiency of one of the most promising $k$-medoids algorithms PAM.
% In addition, it is not straighforward to generalize the best-arm problem formulation to the $k$-medoid problem neither.
Second, instead of having one best-arm identification problem, we reformulated PAM as a sequence of best-arm problems, treating different objects as the arm in different steps of PAM: each point is treated as an arm in the BUILD step and each medoid-and-non-medoid swap is treated as an arm in the SWAP step. 
Building on top of this, we further notice that the intrinsic difficulties of this sequence of best-arm problems are different, which can be exploited to further speed up the algorithm, as demonstrated in the later part the paper.

% Last but not the least, as demonstrated in the later part the paper, the intrinsic difficulty of different best-arm problems are different, and we can adapt to this to make significant improvement.   

The rest of the paper is organized as follows. \martin{Fill in later}

\section{Preliminaries}
\martin{I omitted the dimension $d$ because the points may not be represented by a vector}
For $n$ data points $\mathcal{X} =  \{ x_1, x_2, \cdots, x_n \}$ and a user-specified distance function $d(\cdot, \cdot)$, the $k$-medoids problem aims to find a set of $k$ medoids $\mathcal{M} = \{m_1, \cdots, m_k \} \subset \mathcal{X}$ to minimize the overall distance of points from their closest medoids:
\begin{equation} \label{eqn:total-loss}
	L(\mathcal{M}) =  \sum_{i=1}^n \min_{m_l \in \mathcal{M}} d(m_l, x_i)
\end{equation}
Note that in the above definition, $d$ does not need to be a distance metric that satisfies symmetry, triangle inequality, or positivity. 

\subsection{Partitioning Around Medoids}
% In this paper, we consider accelerating the PAM algorithm . 
PAM \cite{kaufman1987clustering, kaufman1990partitioning} first initializes the set of $k$ medoids via the BUILD step and then repeatedly performs the SWAP step to improve the loss until convergence. 

% \subsection{Partitioning Around Medoids (PAM)}
% The $k$-medoids problem is, in general, NP-hard. As such, iterative greedy algorithms are often used.  The state-of-the-art algorithm for the $k$-medoids problem, Partitioning Around Medoids (PAM), takes a greedy approach, divided into two steps: BUILD and SWAP. In the BUILD step, medoids are initialized one-by-one by choosing each new medoid to be the one that would lower the loss (Equation \ref{eqn:total-loss}) the most. In the SWAP step, we consider swapping each of the medoid assignments with a non-medoid and perform the swap which would lower the loss (Equation \ref{eqn:total-loss}) the most. The BUILD step is run once and then the SWAP step is run multiple times until convergence.

% \subsubsection{PAM BUILD step}

% In the BUILD step, it aims to find a good initial set of $k$ medoids by greedily selecting one point at a time that minimizes the overall loss in \eqref{eqn:sec_intro_total-loss}. 
% Then in the SWAP step, it considers all $k(n-k)$ possible medoid-and-non-medoid point pairs for swap and swap the pair that reduces the loss the most; it repeats such a step until no improvement can be made. 

\paragraph{BUILD step} Select an initial set of $k$ medoids by greedily adding one point at a time that minimizes the overall loss \eqref{eqn:total-loss}. 
% each of the medoids is greedily initialized by choosing the $l$th medoid, conditioned on the previous $l-1$ medoids, that reduces the total loss of every other point. 
The first point to add is the medoid of all $n$ points.
Given the current set of $l-1$ medoids $\mathcal{M}_{l-1} = \{m_1, \cdots, m_{l-1}\}$, the next point to add $m_l$ can be written as
\begin{equation}
\label{eqn:build-next-medoid}
    m_l = \argmin_{x \in \mathcal{X} \setminus \mathcal{M}_{l-1}} \sum_{j=1}^n \min[d(x, x_j), \min_{m' \in \mathcal{M}_{l-1}} d(m', x_j)]. 
\end{equation}

% Equivalently, we can find the find $m_l$ by minimizing the change in total loss:
% \begin{equation}
% \label{eqn:build-next-medoid-td}
%     m_l = \argmin_{x \in \mathcal{X} \setminus \mathcal{M}} \sum_{j=1}^n  \Delta L_{x}(x_j)
% \end{equation}

% where

% \begin{equation}
% \label{eqn:build-td}
%     \Delta L_{x}(x_j) = \min[d(x, x_j) - \min_{m' \in \mathcal{M}} d(m', x_j), 0]
% \end{equation}

% \ilan{Should we instead be defining the change to be positive? 
% Saying ``minimizes the change in total loss'' sounds a bit weird to me, because it sounds like you want to make as little change as possible.}

% represents the change in total loss for reference point $x_j$ induced by choosing $x$ as a new medoid. \martin{$\Delta L_{x}(x_j)$ is not well-defined because the dependency on $\mathcal{M}$ was omitted. How about $\Delta L_{x, \mathcal{M}}(x_j)$?} 

Computing $m_l$ from Eq. \eqref{eqn:build-next-medoid} requires computing the distance $d$ between each candidate point $x \in \mathcal{X}\setminus\mathcal{M}_{l-1}$ and all other points in the dataset---effectively an $O(n^2)$ operation. 
PAM BUILD step repeats such a search $k$ times, totalling $O(kn^2)$ distance computations. This is prohibitively expensive when the distance evaluation is costly, e.g., high-dimensional data or complicated choices of $d$ such as the Wasserstein distance.

% Furthermore, this process must be repeated for each of the $k$ initial medoid assignments. As such, the PAM BUILD step requires $O(kN^2)$ computations of the distance function $d$; this is prohibitively expensive for complicated choices of $d$ such as Wasserstein distance.
% \ilan{Maybe ``This is prohibitively expensive when the data is very high dimensional or for complicated choices of $d$ such as the Wasserstein distance.'' We don't want to give the impression that this is only relevant for non-trivial distances}

\paragraph{SWAP step} Among all possible $k(n-k)$ pairs of medoid and non-medoid, swap the one that would reduce the loss the most.
% In the SWAP step, we consider swapping the assignment of any of the $k$ medoids with any of the $N-k$ non-medoids. For each of the possible $k(N-k)$ swaps, we calculate the total change in loss for each of the $N$ datapoints. We then perform the swap that would lower the total loss for the dataset. 
Let $\mathcal{M}$ be the current set of $k$ medoids. The best pair to swap can be written as:
% pecifically, our goal is to find a medoid-nonmedoid pair $(m^*, x^*)$ such that:
\begin{equation}
\label{eqn:next-swap}
    (m^*, x^*) = \argmin_{(m,x) \in \mathcal{M} \times (\mathcal{X} \setminus \mathcal{M}) } \sum_{j=1}^n \min[d(x, x_j), \min_{m' \in \mathcal{M}\setminus \{m\}} d(m', x_j)]. 
\end{equation}

% Equivalently, we can find $(m^*, x^*)$ that minimizes:

% \begin{equation}
% \label{eqn:next-swap-td}
%     (m^*, x^*) = \argmin_{(m,x) \in \mathcal{M} \times (\mathcal{X} \setminus \mathcal{M}) } \sum_{j=1}^n \Delta L_{m, x_i}(x_j)
% \end{equation}

% where

% \begin{equation}
% \label{eqn:swap-td}
%     \Delta L_{m, x_i}(x_j) = \min[d(x_i, x_j) - \min_{m' \in \mathcal{M}\setminus \{m\}} d(m', x_j), 0]
% \end{equation}

% represents the induced change in loss for point $x_j$ by removing $m$ from the list of medoids and choosing $x_i$ as a new medoid. \martin{$\Delta L_{m, x_i}(x_j)$ is not well-defined because the dependency on $\mathcal{M}$ was omitted. How about $\Delta L_{m, x_i,\mathcal{M}}(x_j)$? Also, this is very similar to the $\Delta L$ in the BUILD step. Consider changing them to $\Delta L^{\text{BUILD}}$ and $\Delta L^{\text{SWAP}}$ for clarity.} 

The SWAP step is iterated until convergence. Similar to the BUILD step, each SWAP step requires $O(k(n-k)^2)$ distance computations.
% , which is prohibitively expensive for complicated choices of $d$.


% \subsection{Formal $k$-medoids Problem Statement}
% Formally, let $\mathcal{X} =  \{ x_1, x_2, \cdots, x_N \}$ be a set of $N$ points in $d$ dimensions, $k$ be the number of clusters to find, and $d(\cdot, \cdot)$, a distance function. For a given set of $k$ medoids $\mathcal{M} = \{m_1, \cdots, m_k \} \subset \mathcal{X}$, the objective function of the $k$-medoids problem is the sum of distances from each point to its closest medoid: \martin{Both $N$ and $n$ are used to denote the number of data points. I suggest to consistently use $n$ because other quantities like $d$ and $k$ are both lower-case.} \martin{$d$ was used to denote both the number of dimensions and the distance metric. Schubert et al. 2018 also overloaded $d$, but this hurts clarity. Maybe changing the distance function to $dist$?}
% \begin{equation}
% \label{eqn:total-loss}
% 	L(\mathcal{M}) =  \sum_{i=1}^n \min_{m_l \in \mathcal{M}} d(m_l, x_i)
% \end{equation}

% The $k$-medoids problem is then to determine the optimal assignment of medoids $\mathcal{M}$, i.e. $\argmin_{\mathcal{M}}L({\mathcal{M}})$

% Note that while $d$ is often a distance metric such as $L_2$ distance, it need not be so; in fact, any arbitrary dissimilarity metric (even an asymmetric one) could be provided above. In general, this problem is NP-Hard \ref{citation}. As such, this problem is generally tackled with greedy iterative algorithms, which we discuss Section \ref{priorwork}.

% \subsection{Comparison to $k$-means}

% At first glance, the problem specification of $k$-medoids may appear very similar to $k$-means, where a similar objective function is used:

% \begin{equation}
% \label{eqn:total-loss-means}
% 	L_{kmeans}(\{\mu_1, \dots, \mu_k\}) =  \sum_{i=1}^n \min_{\mu \in \{\mu_1, \dots, \mu_k\}} ||d(\mu, x_i)||^2
% \end{equation}

% Crucially, however, in $k$-means the optimization of $L_{kmeans}$ is performed over all possible sets of vectors $U = \{\mu_1, \dots, \mu_k\} \subset \mathbb{R}^d$ and the means $\mu_i$ are not required to be actual datapoints. \martin{Use text format for subscript that is not a variable, e.g. $L_{\text{kmeans}}$.}

% Naturally, one might ask if we could reduce the $k$-medoids problem to the $k$-means problem by choosing the medoids to be the real datapoints closest to the means $\{\mu_1, \dots, \mu_k\}$. However, this approach is more susceptible to outliers due to the squaring of the individual loss terms in \ref{eqn:total-loss-means} and will not return the same results as the $k$-medoids problem. It is straightforward to construct small examples where the results of this approach disagree with the solution of the $k$-medoids problem. In fact, it is well-known that $k$-means is more susceptible to noise and outliers than $k$-medoids \ref{citation}.

% In the $k$-means algorithm, $d$ in Equation \ref{eqn:total-loss-means} is usually $L_2$ distance. For completeness, we also mention the \textbf{$k$-medians} problem, in which $d$ is instead the $L_1$ distance, which is less susceptible to noise and outliers than the usual $L_2$ distance. This (rather specific) problem permits an EM-style decomposition which results in an algorithmic complexity similar to the one shown in this paper \ref{citation}; however, the loss function being optimized is different from that in the $k$-medoids problem. Furthermore, the approach presented in our work applies more generally to arbitrary $d$, even those which are not metrics such as $L_1$ or other popular metrics.

% \ilan{The paragraph above is not very clear to me. Are we sure that $k$-medians is generally understood to be $k$-means with $L_1$ instead $L_2$ distances?}

% \section{Prior Work} \martin{Put prior work as a subsection of the Introduction section}
% \label{priorwork}

% \subsection{Partitioning Around Medoids (PAM)}
% The $k$-medoids problem is, in general, NP-hard. As such, iterative greedy algorithms are often used.  The state-of-the-art algorithm for the $k$-medoids problem, Partitioning Around Medoids (PAM), takes a greedy approach, divided into two steps: BUILD and SWAP. In the BUILD step, medoids are initialized one-by-one by choosing each new medoid to be the one that would lower the loss (Equation \ref{eqn:total-loss}) the most. In the SWAP step, we consider swapping each of the medoid assignments with a non-medoid and perform the swap which would lower the loss (Equation \ref{eqn:total-loss}) the most. The BUILD step is run once and then the SWAP step is run multiple times until convergence.

% \subsubsection{PAM BUILD step}
% In the BUILD step, each of the medoids is greedily initialized by choosing the $l$th medoid, conditioned on the previous $l-1$ medoids, that reduces the total loss of every other point. 
% \ilan{}
% More formally, suppose the current set of medoids is $\mathcal{M} = \{m_1, \cdots, m_{l-1}\}$ and we wish to add the $l$th medoid $m_l$. Our goal is to identify a new medoid $m_l$ such that:

% \begin{equation}
% \label{eqn:build-next-medoid}
%     m_l = \argmin_{x \in \mathcal{X} \setminus \mathcal{M}} \sum_{j=1}^n \min[d(x, x_j), \min_{m' \in \mathcal{M}} d(m', x_j)]. 
% \end{equation}

% Equivalently, we can find the find $m_l$ that minimizes the change in total loss:

% \begin{equation}
% \label{eqn:build-next-medoid-td}
%     m_l = \argmin_{x \in \mathcal{X} \setminus \mathcal{M}} \sum_{j=1}^n  \Delta L_{x}(x_j)
% \end{equation}

% where

% \begin{equation}
% \label{eqn:build-td}
%     \Delta L_{x}(x_j) = \min[d(x, x_j) - \min_{m' \in \mathcal{M}} d(m', x_j), 0]
% \end{equation}

% \ilan{Should we instead be defining the change to be positive? 
% Saying ``minimizes the change in total loss'' sounds a bit weird to me, because it sounds like you want to make as little change as possible.}

% represents the change in total loss for reference point $x_j$ induced by choosing $x$ as a new medoid. \martin{$\Delta L_{x}(x_j)$ is not well-defined because the dependency on $\mathcal{M}$ was omitted. How about $\Delta L_{x, \mathcal{M}}(x_j)$?} 

% Computing $m_l$ from Equation \ref{eqn:build-next-medoid} \martin{Use \eqref{eqn:build-next-medoid}} requires computing $d$ for each candidate point $x \in \mathcal{X}\setminus\mathcal{M}$ to each other point in the dataset -- an $O(N^2)$ operation. Furthermore, this process must be repeated for each of the $k$ initial medoid assignments. As such, the PAM BUILD step requires $O(kN^2)$ computations of the distance function $d$; this is prohibitively expensive for complicated choices of $d$ such as Wasserstein distance.
% \ilan{Maybe ``This is prohibitively expensive when the data is very high dimensional or for complicated choices of $d$ such as the Wasserstein distance.'' We don't want to give the impression that this is only relevant for non-trivial distances}

% \subsubsection{PAM SWAP Step}
% In the SWAP step, we consider swapping the assignment of any of the $k$ medoids with any of the $N-k$ non-medoids. For each of the possible $k(N-k)$ swaps, we calculate the total change in loss for each of the $N$ datapoints. We then perform the swap that would lower the total loss for the dataset. 

% Specifically, our goal is to find a medoid-nonmedoid pair $(m^*, x^*)$ such that:

% \begin{equation}
% \label{eqn:next-swap}
%     (m^*, x^*) = \argmin_{(m,x) \in \mathcal{M} \times (\mathcal{X} \setminus \mathcal{M}) } \sum_{j=1}^n \min[d(x, x_j), \min_{m' \in \mathcal{M}\setminus \{m\}} d(m', x_j)]. 
% \end{equation}

% Equivalently, we can find $(m^*, x^*)$ that minimizes:

% \begin{equation}
% \label{eqn:next-swap-td}
%     (m^*, x^*) = \argmin_{(m,x) \in \mathcal{M} \times (\mathcal{X} \setminus \mathcal{M}) } \sum_{j=1}^n \Delta L_{m, x_i}(x_j)
% \end{equation}

% where

% \begin{equation}
% \label{eqn:swap-td}
%     \Delta L_{m, x_i}(x_j) = \min[d(x_i, x_j) - \min_{m' \in \mathcal{M}\setminus \{m\}} d(m', x_j), 0]
% \end{equation}

% represents the induced change in loss for point $x_j$ by removing $m$ from the list of medoids and choosing $x_i$ as a new medoid. \martin{$\Delta L_{m, x_i}(x_j)$ is not well-defined because the dependency on $\mathcal{M}$ was omitted. How about $\Delta L_{m, x_i,\mathcal{M}}(x_j)$? Also, this is very similar to the $\Delta L$ in the BUILD step. Consider changing them to $\Delta L^{\text{BUILD}}$ and $\Delta L^{\text{SWAP}}$ for clarity.} 

% The SWAP step is iterated until convergence. Similar to the BUILD step, each SWAP step requires $O(kN^2)$ distance computations, which is prohibitively expensive for complicated choices of $d$.

% \subsection{FastPAM1}

% Accelerating the PAM algorithm is an active area of research. Perhaps most closely related to our work is \ref{FastPAM}, which presents three independent optimizations to the original PAM algorithm. Of these three, only one (dubbed FastPAM1) optimization applied to the SWAP step, preserves the results as the original PAM algorithm.

% In the FastPAM1 optimization, the distance from each point $x_j$ to its nearest medoid, $d_1(x_j)$, and to its \textit{second nearest} medoid, $d_2(x_j)$ is used to rewrite \ref{eqn:swap-td} \martin{\eqref{eqn:swap-td}} as:

% \begin{equation}
% \label{eqn:FastPam1-eqn}
%     \Delta L_{m, x_i}(x_j) = - d_1(x_j)\mathbbm{1}_{x_j \in C_m} + d(x_i, x_j)\mathbbm{1}_{x_j \in C_{x_i}} + d_2(x_j)\mathbbm{1}_{x_j \notin C_{x_i}}
% \end{equation}

% \ilan{I find the notation with $x_i$ and $x_j$ a bit confusing. It's a bit weird that $m$ and $x_i$ are the things being swapped, while $x_j$ is just a general point}

% where $C_m$ is the set of points assigned to medoid $m$ before the swap, and $C_{x_i}$ is the set of points that would be assigned to the new medoid $x_i$ if the swap were performed. 
% Note that now the quantities $d_1(x_j)$ and $d_2(x_j)$ can be cached and that (\ref{eqn:FastPam1-eqn}) no longer depends on $m$. \ilan{I don't see that right away}
% This optimization reduces the complexity of PAM by $O(k)$ in each SWAP step, but only when the clusters are roughly similar in size, each containing about $O(\frac{1}{k})$ points \textbf{why is balanced cluster distro necessary? Eqn 8 doesn't suggest that}. 
% In our algorithm, UltraPAM, we see a $O(\frac{N}{logN})$ speedup under relatively mild assumptions and do not require the clusters to be balanced. \ilan{not the best place to mention UltraPAM for the first time.}
% Furthermore, it is possible to combine the FastPAM1 optimization with UltraPAM; indeed, we do so in our reference implementation available at \{githublink\}.

% \martin{Use $\mathcal{C}$ font to denote sets.}

% \martin{Could you double check \eqref{eqn:FastPam1-eqn}? I have a different answer. Divide the points into four categories based on which medoid it assigned to before and after the SWAP: 
% \begin{itemize}
% \item Before $m$ and after $x_i$; point set $C_m \cap C_{x_i}$; delta loss $d(x_i,x_j) - d_1(x_j)$.
% \item Before $m$ and after other medoids; point set $C_m \cap C_{x_i}^c$; delta loss $d_2(x_j) - d_1(x_j)$.
% \item Before other medoids and after $x_i$; point set $C_m^c \cap C_{x_i}$; delta loss $d(x_i,x_j) - d_1(x_j)$.
% \item Before other medoids and other medoids; point set $C_m^c \cap C_{x_i}^c$; delta loss $0$.
% \end{itemize}
% Therefore, 
% \begin{equation}
%     \Delta L_{m, x_i}(x_j) = - d_1(x_j)\mathbbm{1}_{\{x_j \in C_m \cup C_{x_i}\}} + d(x_i, x_j)\mathbbm{1}_{\{x_j \in C_{x_i}\}} + d_2(x_j)\mathbbm{1}_{\{x_j \in C_{m}\cap C_{x_i}^c\}}
% \end{equation}
% }

% \ilan{
% I checked, and I agree with this.
% In particular, if $x_j$'s previous closest medoid was some $m' \ne m$ and $d(x_j,m') < d(x_j,x_i)$, the delta should be 0. In this case, $x_j \notin C_m$, $x_j \notin C_{x_i}$, so equation (9) gives $d_2(x_j)$, while (10) gives 0.
% } 

% \martin{\eqref{eqn:FastPam1-eqn} is hard to follow. Add more details (like the one I mentioned above). }

% \subsection{Theoretical Motivation: Multi-Armed Bandits}

% Add description of MAB problem. Theory from the multi-armed bandit (MAB) literature suggests that best arm among $N$ arms can be found with $O(NlogN)$ \martin{$O(N\log N)$} arm pulls, as in the UCB algorithm \{citation\}. \martin{Be more precise here. Include the success probability $\delta$ and the gaps between the best arm and other arms $\delta \mu_i$ in the expression.} This observation motivates the approach presented in this paper, in which we use an adaptation of the UCB algorithm to find medoids more quickly. 

% \ilan{we take too long to get here}

% Intuitively, in the BUILD step, we consider each of the $N$ candidate datapoints as an "arm", where an arm pull corresponds to computing the induced loss on a single reference datapoint by choosing the candidate in question as a medoid.  The multi-armed bandit (MAB) literature then suggests that we can identify the best medoid to assign with $O(NlogN)$ distance computations in each of the $k$ BUILD steps.

% Similarly, in the SWAP step, we consider each of the $k(N-k)$ medoid-nonmedoid pairs as an "arm", and an arm pull corresponds to computing the loss induced on a reference point by swapping the medoid with the non-medoid. The multi-armed bandit (MAB) literature then suggests that we can identify the best swap to perform with $O(kNlogN)$ distance computations in each SWAP step.

% Intuitively, in each of the BUILD and SWAP steps, we convert the computation of the sum for each candidate $m_l$ in \ref{eqn:build-next-medoid} or $(m,x)$ in \ref{eqn:swap-td} into a sampling problem. Instead of computing the sums exactly, we compute confidence intervals that contain the sum with high probability and explore promising arms more while expending less computation on unpromising arms. We expect such a UCB-based approach to recover the true best arm, thus matching the results of the greedy algorithm PAM, with high probability.  We formally describe the algorithm in Section \ref{algo}, along with theoretical guarantees for correctness in Section \ref{theory}.

% \subsection{Main Contributions}

% In this work, we:

% \begin{enumerate}
%     \item Propose a new algorithm, \algnamenospace, that uses a UCB-based algorithm to find a solution to the $k$-medoids problem,
%     \item Provide theoretical guarantees as to when UltraPAM will return the same results as current state-of-the-art methods such as PAM, and
%     \item Experimentally validate our approach on a number of real-world datasets.
% \end{enumerate}


% \martin{END of martin's version of Intro+Formulation}

==> old/intro06-02b.tex <==
% !TEX root = main.tex

% \martin{START of martin's version of Intro+Formulation}

% \martin{Introduction outline: 
% \begin{itemize}
%     \item Clustering is important and k-mean is one of the most popular clustering method. 
%     \item k-mean has two drawbacks.
%     \item First, it is only fast (linear for finding the centroid) when using $l_2^2$ or $l_1$ distance (the latter corresponds to k-median). However, for different applications, a different distance metric may be more appropriate (e.g. the editing distance for code.org)
%     \item Second, centroid is not a point in the dataset, while for some applications, having a representative for each cluster is important (e.g., a representative cell for single-cell RNA-seq)
%     \item Other clustering methods that allow for a user-defined distance matrix, like k-medoid, graph-based clustering methods (Louvain), requires precomputing of the distance matrix, which can be computationally and disk-space intensive. 
%     \item We consider an PAM  empirically preferable k-medoid algorithm PAM. (ref from wiki)
%     \item It is slow (need to quantify). We made it faster.
%     \item The algorithmic contributions are:
%     \item 1. We converted a deterministic computation problem into a random sampling problem, and used MAB to solve it. 
%     \item 2. The trick is to view each SWAP, instead of each data point, as an arm. 
%     \item 3. We adaptively chose the sub-Gaussian parameter for each stage and each arm to further increase speed. 
% \end{itemize}}

\section{Introduction}
\label{intro}

Clustering is a ubiquitous task in machine learning, whose goal is to partition a set of points into ``clusters'' such that points within each cluster are similar. \mo{Is this too general of a starting point?} \ilan{yes, we could remove the first sentence}

Many modern data science applications require clustering of very-large-scale data. 
Due to its computational efficiency, 
% and for this reason, 
$k$-means clustering \cite{macqueen1967some,lloyd1982least} became one of the most popular choices of algorithm.
% because of its computational efficiency.
% \mo{Not clear to me that large scale data makes $k$-means popular -- maybe just say $k$-means is a popular example method?}
In the clustering process, $k$-means clustering alternates between reassigning points to their nearest cluster centers and recomputing those centers. 
% \mo{$k$-means "alternates between reassigning points to their nearest cluster centers and recomputing those centers"}
Central to its success is the specific choice of the cluster center; for a set of points, $k$-means defines the cluster center be the point which has the smallest average \emph{squared Euclidean distance} from all other points in the set. 
Under such a definition, the cluster center turns out to be the arithmetic mean of the set of points, which can be computed efficiently. 
% \mo{remove the word "very"?}

% \martin{include k-medians here?} \ilan{I would say no. I like the flow as is}

While commonly used in practice, $k$-means clustering suffers from several drawbacks. 
First, while it can efficiently compute the cluster center under the squared Euclidean distance, it is not straightforward to generalize to other distance metrics. 
However,
% \mo{replace "However" with "Indeed"?} 
for different applications, we may want to use a different distance to quantify the similarity between points. 
Some examples would be $l_1$ and cosine distance for sparse data like in recommendation systems \cite{leskovec2020mining} and in single-cell RNA-seq analysis \cite{ntranos2016fast}; or edit distance for text data \cite{navarro2001guided}; or graph metrics for social network data \cite{mishra2007clustering}. 
Second, the cluster center in $k$-means clustering is in general not a point in the dataset and may not be interpretable in many applications. This is especially problematic when the data is structured like in computer vision, or when it is sparse like in recommendation systems \cite{leskovec2020mining}.

As an alternative choice, $k$-medoids clustering algorithms \cite{kaufman1987clustering,kaufman1990partitioning} use the \emph{medoid} to define the cluster center for a set of point. Given an arbitrary distance function, the medoid of a set of point is the point \emph{in the set} that minimizes the average distance to all the other points.
Note that the distance metric can be arbitrary; indeed, it needs not be a metric and could be an asymmetric dissimilarity measure
% So $k$-medoids clustering algorithms work for arbitrary distances \mo{I think this sentence can be changed to "Note that the distance metric can be arbitrary; indeed, it need not be a metric at all and could be an asymmetric dissimilarity measure"}. 
Moreover, unlike $k$-means, the cluster center in $k$-medoids, i.e., the medoid, is restricted to one of the points in the dataset, thus addressing the second drawback of k-means clustering. 

For $n$ data points $\mathcal{X} =  \{ x_1, x_2, \cdots, x_n \}$ and a user-specified distance function $d(\cdot, \cdot)$, the $k$-medoids problem aims to find a set of $k$ medoids $\mathcal{M} = \{m_1, \cdots, m_k \} \subset \mathcal{X}$ to minimize the overall distance of points from their closest medoids: 
\begin{equation} \label{eqn:sec_intro_total-loss}
	L(\mathcal{M}) =  \sum_{i=1}^n \min_{m_l \in \mathcal{M}} d(m_l, x_i)
\end{equation}
This problem is unfortunately NP-hard in general \cite{schubert2019faster}.
% \mo{in general. The Partionining Around Medoids...}., and the
The partitioning around medoids (PAM) algorithm \cite{kaufman1987clustering, kaufman1990partitioning} is one of the most widely-used heuristic $k$-medoids clustering algorithm.
In the BUILD step, it aims to find a good initial set of $k$ medoids by greedily selecting one point at a time that minimizes the overall loss in \eqref{eqn:sec_intro_total-loss}. 
Then in the SWAP step, it considers all $k(n-k)$ possible pairs of  medoid and non-medoid points, and swaps the pair that reduces the $k$-medoids clustering loss the most; it repeats such a step until no improvement can be made. 

PAM has been empirically shown to produce satisfactory results among popular $k$-medoids clustering algorithms \cite{reynolds2006clustering,schubert2019faster}.  
However, it can be computationally challenging, especially for large-scale datasets. 
Indeed, each SWAP iteration takes $O(k(n-k)^2)$ distance evaluations, for computing the change of loss for each of the $k(n-k)$ medoid-and-non-medoid pairs with respect to the rest $n-k$ non-medoid points. 
BUILD step is equivalent to one SWAP step.
Randomized algorithms like CLARA \cite{kaufman1990partitioning} and CLARANS \cite{ng2002clarans} have been proposed to improve computational efficiency, at the cost of deteriorated clustering quality.
More recently, Schubert et al. proposed a deterministic algorithm FastPAM \cite{schubert2019faster} that guarantees the same output as PAM but improves the complexity to $O(n^2)$ when the cluster sizes are similar. 
The factor $O(k)$ improvement is particularly important for large values of $k$.

\paragraph{Contribution.} We propose \algnamenospace, a new randomized $k$-medoids algorithm that takes \mo{$O(kn^2)$} \martin{thought we also have an improvement in BUILD step, no?} for the BUILD step and $O(  n^2 \wedge f(k) n \log n )$ for each SWAP step, while returning the same result as PAM with high probability under reasonable assumptions of the data. 
For a fixed $k$, \algname takes $O(n \log n)$ distance evaluations for each SWAP step, effectively improving the PAM SWAP step from quadratic to almost linear. 
\algname reduces to FastPAM for a large value of $k$. 
We also propose a variation \algaprname that slightly deviates from the PAM solution but has a much faster speed.
We experimentally validate our results on a number of real-world datasets, including Code.org Hour of Code, single-cell RNA-seq, and the MNIST handwritten digits datasets. We observe speedups of up to 50x in wall clock time over state-of-the-art algorithms. \martin{Update this paragraph after finishing the main paper}

The improvement is made by reformulating each step of PAM from a \emph{deterministic computational problem} to a \emph{statistical estimation problem}. 
In the SWAP step, for example, we need to decide among $k(n-k)$ possible medoid-and-non-medoid swaps, which one has the smallest loss. 
If we swap, e.g., medoid $m_l$ and and non-medoid $x_i$, the new set of medoids after excluding $m_l$ and including $x_i$ would be $\mathcal{M}-\{m_l\} + \{x_i\}$,
and the corresponding loss:
\begin{equation} \label{eqn:sec_intro_swap_loss}
	L(m_l, x_i; \mathcal{M}) = \sum_{j=1}^n \min_{m_l \in \mathcal{M}-\{m_l\} + \{x_i\}} d(m_l, x_j) \overset{\text{def}}{=} \sum_{j=1}^n g(x_j),
\end{equation}
where $g(\cdot)$ is a function that depends on $\mathcal{M}$, $m_l$, $x_i$.
Eq. \eqref{eqn:sec_intro_swap_loss} shows that the loss of a swap $L(m_l, x_i; \mathcal{M})$ be can written as the summation of the function value $g(\cdot)$, evaluated on all $n$ points. 
Therefore, $L(m_l, x_i; \mathcal{M})$ can be estimated by evaluating the function on a randomly sampled subset of $n' < n$ points, where the estimation accuracy depends on the size of the subsample $n'$. 

Recall that the goal of the SWAP step is to find the medoid-and-non-medoid swap with the smallest loss, which is different from computing the exact loss for every possible swap. 
So an estimation of the best swap with high confidence would suffice. 
Intuitively,  promising swaps with smaller loss should be estimated with a higher accuracy and less promising ones can be discarded without being evaluated on too many randomly-sampled data points. 

To design the adaptive sampling strategy, we show that both the BUILD step and each of the SWAP step can be formulated as a separate best-arm identification problem in the multi-armed bandits (MAB) literature \cite{audibert2010best,even2002pac,jamieson2014lil,jamieson2014best}. 
In a typical setting of the best-arm identification problem, we have $m$ arms. At time $t = 0,1,\cdots,$ we decide to pull an arm $A_t\in \{1,\cdots,m\}$, and receive a reward $R_t$ with $E[R_t] = \mu_{A_t}$ . The goal is to identify the arm with the largest expected reward with high probability while pulling as few arms as possible.
In the context of the PAM SWAP step, we can think of each possible medoid-and-non-medoid swap as an arm in the best-arm problem, totaling $k(n-k)$ arms. The arm parameter corresponds to the loss of the swap, and by pulling an arm, we observe the loss evaluated on a randomly-sampled data point. 
Then, the best swap can be estimated using existing best-arm algorithms like the Upper Confidence Bound (UCB) algorithm \cite{lai1985asymptotically}.

\subsection{Related works}

k-means clustering is one of the \emph{centroid}-based clustering algorithms, where the centroid of a set of point for a distance metric is defined as the point \emph{in the space}
% \mo{"among the datapoints"?}
that minimizes the overall distance from other points. So the key difference between centroid and medoid is that centroid needs not be one of the points in the set. 
k-means uses centroid for squared Euclidean distance to define the cluster center, which is the arithmetic mean and can be computed in linear time. 
Centroid for Bregman divergence is also the arithmetic mean and centroid for $l_1$ distance is the component-wise median; the latter is used by the $k$-medians clustering algorithm \cite{bradley1997clustering,jain1988algorithms}.
However, centroid for other distances is hard to compute.
For example, centroid for the unsquared Euclidean distance corresponds to the much harder Weber problem with no closed-form solution \cite{bradley1997clustering,overton1983quadratically}. 
\martin{Maybe delete this paragraph if we don't have enough space}

For other k-medoids clustering algorithms, Park et al. \cite{park2009simple} proposed a $k$-means-like algorithm that alternates between reassigning the points to their closest medoid and recomputing the medoid for each cluster, until the $k$-medoids clustering loss can no longer be improved.
However, it has been empirically shown to produce less satisfactory results as compared to PAM \cite{reynolds2006clustering,schubert2019faster}. 
Other proposals include optimizations for Euclidean space and tabu search heuristics \cite{estivill2001robust}.

The idea of algorithm acceleration by converting a computational problem into a statistical estimation problem and designing the adaptive sampling procedure via MAB has
witnessed a few successes,  including in Monte Carlo tree search \cite{chang2005adaptive,kocsis2006bandit}, hyper-parameter tuning \cite{li2016hyperband,jamieson2016non}, discrete optimization \cite{bagaria2018adaptive}, and permutation-based multiple testing \cite{zhang2019adaptive}. 
In the context of $k$-medoids clustering, previous works \cite{bagaria2018medoids,baharav2019ultra} have considered finding the medoid of a set points, namely the $1$-medoid problem.
In these works. the problem was also formulated as a best-arm identification problem, with each point being arm and its average distance to other points being the arm parameter. 

First, while the $1$-medoid problem can be solved exactly, the $k$-medoids problem is harder and can only rely on heuristic solutions. We hence focus on improving the computational efficiency of one of the most promising $k$-medoids algorithms PAM.
% In addition, it is not straighforward to generalize the best-arm problem formulation to the $k$-medoid problem neither.
Second, instead of having one best-arm identification problem, we reformulated PAM as a sequence of best-arm problems, treating different objects as the arm in different steps of PAM: each point is treated as an arm in the BUILD step and each medoid-and-non-medoid swap is treated as an arm in the SWAP step. 
Building on top of this, we further notice that the intrinsic difficulties of this sequence of best-arm problems are different, which can be exploited to further speed up the algorithm, as demonstrated in the later part the paper.

% Last but not the least, as demonstrated in the later part the paper, the intrinsic difficulty of different best-arm problems are different, and we can adapt to this to make significant improvement.   

The rest of the paper is organized as follows. \martin{Fill in later}

\section{Preliminaries}
\martin{I omitted the dimension $d$ because the points may not be represented by a vector}
For $n$ data points $\mathcal{X} =  \{ x_1, x_2, \cdots, x_n \}$ and a user-specified distance function $d(\cdot, \cdot)$, the $k$-medoids problem aims to find a set of $k$ medoids $\mathcal{M} = \{m_1, \cdots, m_k \} \subset \mathcal{X}$ to minimize the overall distance of points from their closest medoids:
\begin{equation} \label{eqn:total-loss}
	L(\mathcal{M}) =  \sum_{i=1}^n \min_{m_l \in \mathcal{M}} d(m_l, x_i)
\end{equation}
Note that in the above definition, $d$ does not need to be a distance metric that satisfies symmetry, triangle inequality, or positivity. 

\subsection{Partitioning Around Medoids}
% In this paper, we consider accelerating the PAM algorithm . 
PAM \cite{kaufman1987clustering, kaufman1990partitioning} first initializes the set of $k$ medoids via the BUILD step and then repeatedly performs the SWAP step to improve the loss until convergence. 

\paragraph{BUILD step} Select an initial set of $k$ medoids by greedily adding one point at a time that minimizes the overall loss \eqref{eqn:total-loss}. 
% each of the medoids is greedily initialized by choosing the $l$th medoid, conditioned on the previous $l-1$ medoids, that reduces the total loss of every other point. 
The first point to add is the medoid of all $n$ points.
Given the current set of $l-1$ medoids $\mathcal{M}_{l-1} = \{m_1, \cdots, m_{l-1}\}$, the next point to add $m_l$ can be written as
\begin{equation}
\label{eqn:build-next-medoid}
    m_l = \argmin_{x \in \mathcal{X} \setminus \mathcal{M}_{l-1}} \sum_{j=1}^n \min[d(x, x_j), \min_{m' \in \mathcal{M}_{l-1}} d(m', x_j)]. 
\end{equation}

Computing $m_l$ from Eq. \eqref{eqn:build-next-medoid} requires computing the distance $d$ between each candidate point $x \in \mathcal{X}\setminus\mathcal{M}_{l-1}$ and all other points in the dataset---effectively $O(n^2)$ computations. 
PAM BUILD step repeats such a search $k$ times, totalling $O(kn^2)$ distance computations. This is prohibitively expensive when the distance evaluation is costly, e.g., high-dimensional data or complicated choices of $d$ such as the Wasserstein distance.

% Furthermore, this process must be repeated for each of the $k$ initial medoid assignments. As such, the PAM BUILD step requires $O(kN^2)$ computations of the distance function $d$; this is prohibitively expensive for complicated choices of $d$ such as Wasserstein distance.
% \ilan{Maybe ``This is prohibitively expensive when the data is very high dimensional or for complicated choices of $d$ such as the Wasserstein distance.'' We don't want to give the impression that this is only relevant for non-trivial distances}

\paragraph{SWAP step} Among all possible $k(n-k)$ pairs of medoid and non-medoid points, swap the one that would reduce the loss the most.
Let $\mathcal{M}$ be the current set of $k$ medoids. The best pair to swap can be written as:
\begin{equation}
\label{eqn:next-swap}
    (m^*, x^*) = \argmin_{(m,x) \in \mathcal{M} \times (\mathcal{X} \setminus \mathcal{M}) } \sum_{j=1}^n \min[d(x, x_j), \min_{m' \in \mathcal{M}\setminus \{m\}} d(m', x_j)]. 
\end{equation}

The SWAP step is repeated until convergence. Similar to the BUILD step, each SWAP step requires $O(k(n-k)^2)$ distance computations.


% \subsection{Formal $k$-medoids Problem Statement}
% Formally, let $\mathcal{X} =  \{ x_1, x_2, \cdots, x_N \}$ be a set of $N$ points in $d$ dimensions, $k$ be the number of clusters to find, and $d(\cdot, \cdot)$, a distance function. For a given set of $k$ medoids $\mathcal{M} = \{m_1, \cdots, m_k \} \subset \mathcal{X}$, the objective function of the $k$-medoids problem is the sum of distances from each point to its closest medoid: \martin{Both $N$ and $n$ are used to denote the number of data points. I suggest to consistently use $n$ because other quantities like $d$ and $k$ are both lower-case.} \martin{$d$ was used to denote both the number of dimensions and the distance metric. Schubert et al. 2018 also overloaded $d$, but this hurts clarity. Maybe changing the distance function to $dist$?}
% \begin{equation}
% \label{eqn:total-loss}
% 	L(\mathcal{M}) =  \sum_{i=1}^n \min_{m_l \in \mathcal{M}} d(m_l, x_i)
% \end{equation}

% The $k$-medoids problem is then to determine the optimal assignment of medoids $\mathcal{M}$, i.e. $\argmin_{\mathcal{M}}L({\mathcal{M}})$

% Note that while $d$ is often a distance metric such as $L_2$ distance, it need not be so; in fact, any arbitrary dissimilarity metric (even an asymmetric one) could be provided above. In general, this problem is NP-Hard \ref{citation}. As such, this problem is generally tackled with greedy iterative algorithms, which we discuss Section \ref{priorwork}.

% \subsection{Comparison to $k$-means}

% At first glance, the problem specification of $k$-medoids may appear very similar to $k$-means, where a similar objective function is used:

% \begin{equation}
% \label{eqn:total-loss-means}
% 	L_{kmeans}(\{\mu_1, \dots, \mu_k\}) =  \sum_{i=1}^n \min_{\mu \in \{\mu_1, \dots, \mu_k\}} ||d(\mu, x_i)||^2
% \end{equation}

% Crucially, however, in $k$-means the optimization of $L_{kmeans}$ is performed over all possible sets of vectors $U = \{\mu_1, \dots, \mu_k\} \subset \mathbb{R}^d$ and the means $\mu_i$ are not required to be actual datapoints. \martin{Use text format for subscript that is not a variable, e.g. $L_{\text{kmeans}}$.}

% Naturally, one might ask if we could reduce the $k$-medoids problem to the $k$-means problem by choosing the medoids to be the real datapoints closest to the means $\{\mu_1, \dots, \mu_k\}$. However, this approach is more susceptible to outliers due to the squaring of the individual loss terms in \ref{eqn:total-loss-means} and will not return the same results as the $k$-medoids problem. It is straightforward to construct small examples where the results of this approach disagree with the solution of the $k$-medoids problem. In fact, it is well-known that $k$-means is more susceptible to noise and outliers than $k$-medoids \ref{citation}.

% In the $k$-means algorithm, $d$ in Equation \ref{eqn:total-loss-means} is usually $L_2$ distance. For completeness, we also mention the \textbf{$k$-medians} problem, in which $d$ is instead the $L_1$ distance, which is less susceptible to noise and outliers than the usual $L_2$ distance. This (rather specific) problem permits an EM-style decomposition which results in an algorithmic complexity similar to the one shown in this paper \ref{citation}; however, the loss function being optimized is different from that in the $k$-medoids problem. Furthermore, the approach presented in our work applies more generally to arbitrary $d$, even those which are not metrics such as $L_1$ or other popular metrics.

% \ilan{The paragraph above is not very clear to me. Are we sure that $k$-medians is generally understood to be $k$-means with $L_1$ instead $L_2$ distances?}

% \section{Prior Work} \martin{Put prior work as a subsection of the Introduction section}
% \label{priorwork}

% \subsection{Partitioning Around Medoids (PAM)}
% The $k$-medoids problem is, in general, NP-hard. As such, iterative greedy algorithms are often used.  The state-of-the-art algorithm for the $k$-medoids problem, Partitioning Around Medoids (PAM), takes a greedy approach, divided into two steps: BUILD and SWAP. In the BUILD step, medoids are initialized one-by-one by choosing each new medoid to be the one that would lower the loss (Equation \ref{eqn:total-loss}) the most. In the SWAP step, we consider swapping each of the medoid assignments with a non-medoid and perform the swap which would lower the loss (Equation \ref{eqn:total-loss}) the most. The BUILD step is run once and then the SWAP step is run multiple times until convergence.

% \subsubsection{PAM BUILD step}
% In the BUILD step, each of the medoids is greedily initialized by choosing the $l$th medoid, conditioned on the previous $l-1$ medoids, that reduces the total loss of every other point. 
% \ilan{}
% More formally, suppose the current set of medoids is $\mathcal{M} = \{m_1, \cdots, m_{l-1}\}$ and we wish to add the $l$th medoid $m_l$. Our goal is to identify a new medoid $m_l$ such that:

% \begin{equation}
% \label{eqn:build-next-medoid}
%     m_l = \argmin_{x \in \mathcal{X} \setminus \mathcal{M}} \sum_{j=1}^n \min[d(x, x_j), \min_{m' \in \mathcal{M}} d(m', x_j)]. 
% \end{equation}

% Equivalently, we can find the find $m_l$ that minimizes the change in total loss:

% \begin{equation}
% \label{eqn:build-next-medoid-td}
%     m_l = \argmin_{x \in \mathcal{X} \setminus \mathcal{M}} \sum_{j=1}^n  \Delta L_{x}(x_j)
% \end{equation}

% where

% \begin{equation}
% \label{eqn:build-td}
%     \Delta L_{x}(x_j) = \min[d(x, x_j) - \min_{m' \in \mathcal{M}} d(m', x_j), 0]
% \end{equation}

% \ilan{Should we instead be defining the change to be positive? 
% Saying ``minimizes the change in total loss'' sounds a bit weird to me, because it sounds like you want to make as little change as possible.}

% represents the change in total loss for reference point $x_j$ induced by choosing $x$ as a new medoid. \martin{$\Delta L_{x}(x_j)$ is not well-defined because the dependency on $\mathcal{M}$ was omitted. How about $\Delta L_{x, \mathcal{M}}(x_j)$?} 

% Computing $m_l$ from Equation \ref{eqn:build-next-medoid} \martin{Use \eqref{eqn:build-next-medoid}} requires computing $d$ for each candidate point $x \in \mathcal{X}\setminus\mathcal{M}$ to each other point in the dataset -- an $O(N^2)$ operation. Furthermore, this process must be repeated for each of the $k$ initial medoid assignments. As such, the PAM BUILD step requires $O(kN^2)$ computations of the distance function $d$; this is prohibitively expensive for complicated choices of $d$ such as Wasserstein distance.
% \ilan{Maybe ``This is prohibitively expensive when the data is very high dimensional or for complicated choices of $d$ such as the Wasserstein distance.'' We don't want to give the impression that this is only relevant for non-trivial distances}

% \subsubsection{PAM SWAP Step}
% In the SWAP step, we consider swapping the assignment of any of the $k$ medoids with any of the $N-k$ non-medoids. For each of the possible $k(N-k)$ swaps, we calculate the total change in loss for each of the $N$ datapoints. We then perform the swap that would lower the total loss for the dataset. 

% Specifically, our goal is to find a medoid-nonmedoid pair $(m^*, x^*)$ such that:

% \begin{equation}
% \label{eqn:next-swap}
%     (m^*, x^*) = \argmin_{(m,x) \in \mathcal{M} \times (\mathcal{X} \setminus \mathcal{M}) } \sum_{j=1}^n \min[d(x, x_j), \min_{m' \in \mathcal{M}\setminus \{m\}} d(m', x_j)]. 
% \end{equation}

% Equivalently, we can find $(m^*, x^*)$ that minimizes:

% \begin{equation}
% \label{eqn:next-swap-td}
%     (m^*, x^*) = \argmin_{(m,x) \in \mathcal{M} \times (\mathcal{X} \setminus \mathcal{M}) } \sum_{j=1}^n \Delta L_{m, x_i}(x_j)
% \end{equation}

% where

% \begin{equation}
% \label{eqn:swap-td}
%     \Delta L_{m, x_i}(x_j) = \min[d(x_i, x_j) - \min_{m' \in \mathcal{M}\setminus \{m\}} d(m', x_j), 0]
% \end{equation}

% represents the induced change in loss for point $x_j$ by removing $m$ from the list of medoids and choosing $x_i$ as a new medoid. \martin{$\Delta L_{m, x_i}(x_j)$ is not well-defined because the dependency on $\mathcal{M}$ was omitted. How about $\Delta L_{m, x_i,\mathcal{M}}(x_j)$? Also, this is very similar to the $\Delta L$ in the BUILD step. Consider changing them to $\Delta L^{\text{BUILD}}$ and $\Delta L^{\text{SWAP}}$ for clarity.} 

% The SWAP step is iterated until convergence. Similar to the BUILD step, each SWAP step requires $O(kN^2)$ distance computations, which is prohibitively expensive for complicated choices of $d$.

% \subsection{FastPAM1}

% Accelerating the PAM algorithm is an active area of research. Perhaps most closely related to our work is \ref{FastPAM}, which presents three independent optimizations to the original PAM algorithm. Of these three, only one (dubbed FastPAM1) optimization applied to the SWAP step, preserves the results as the original PAM algorithm.

% In the FastPAM1 optimization, the distance from each point $x_j$ to its nearest medoid, $d_1(x_j)$, and to its \textit{second nearest} medoid, $d_2(x_j)$ is used to rewrite \ref{eqn:swap-td} \martin{\eqref{eqn:swap-td}} as:

% \begin{equation}
% \label{eqn:FastPam1-eqn}
%     \Delta L_{m, x_i}(x_j) = - d_1(x_j)\mathbbm{1}_{x_j \in C_m} + d(x_i, x_j)\mathbbm{1}_{x_j \in C_{x_i}} + d_2(x_j)\mathbbm{1}_{x_j \notin C_{x_i}}
% \end{equation}

% \ilan{I find the notation with $x_i$ and $x_j$ a bit confusing. It's a bit weird that $m$ and $x_i$ are the things being swapped, while $x_j$ is just a general point}

% where $C_m$ is the set of points assigned to medoid $m$ before the swap, and $C_{x_i}$ is the set of points that would be assigned to the new medoid $x_i$ if the swap were performed. 
% Note that now the quantities $d_1(x_j)$ and $d_2(x_j)$ can be cached and that (\ref{eqn:FastPam1-eqn}) no longer depends on $m$. \ilan{I don't see that right away}
% This optimization reduces the complexity of PAM by $O(k)$ in each SWAP step, but only when the clusters are roughly similar in size, each containing about $O(\frac{1}{k})$ points \textbf{why is balanced cluster distro necessary? Eqn 8 doesn't suggest that}. 
% In our algorithm, UltraPAM, we see a $O(\frac{N}{logN})$ speedup under relatively mild assumptions and do not require the clusters to be balanced. \ilan{not the best place to mention UltraPAM for the first time.}
% Furthermore, it is possible to combine the FastPAM1 optimization with UltraPAM; indeed, we do so in our reference implementation available at \{githublink\}.

% \martin{Use $\mathcal{C}$ font to denote sets.}

% \martin{Could you double check \eqref{eqn:FastPam1-eqn}? I have a different answer. Divide the points into four categories based on which medoid it assigned to before and after the SWAP: 
% \begin{itemize}
% \item Before $m$ and after $x_i$; point set $C_m \cap C_{x_i}$; delta loss $d(x_i,x_j) - d_1(x_j)$.
% \item Before $m$ and after other medoids; point set $C_m \cap C_{x_i}^c$; delta loss $d_2(x_j) - d_1(x_j)$.
% \item Before other medoids and after $x_i$; point set $C_m^c \cap C_{x_i}$; delta loss $d(x_i,x_j) - d_1(x_j)$.
% \item Before other medoids and other medoids; point set $C_m^c \cap C_{x_i}^c$; delta loss $0$.
% \end{itemize}
% Therefore, 
% \begin{equation}
%     \Delta L_{m, x_i}(x_j) = - d_1(x_j)\mathbbm{1}_{\{x_j \in C_m \cup C_{x_i}\}} + d(x_i, x_j)\mathbbm{1}_{\{x_j \in C_{x_i}\}} + d_2(x_j)\mathbbm{1}_{\{x_j \in C_{m}\cap C_{x_i}^c\}}
% \end{equation}
% }

% \ilan{
% I checked, and I agree with this.
% In particular, if $x_j$'s previous closest medoid was some $m' \ne m$ and $d(x_j,m') < d(x_j,x_i)$, the delta should be 0. In this case, $x_j \notin C_m$, $x_j \notin C_{x_i}$, so equation (9) gives $d_2(x_j)$, while (10) gives 0.
% } 

% \martin{\eqref{eqn:FastPam1-eqn} is hard to follow. Add more details (like the one I mentioned above). }

% \subsection{Theoretical Motivation: Multi-Armed Bandits}

% Add description of MAB problem. Theory from the multi-armed bandit (MAB) literature suggests that best arm among $N$ arms can be found with $O(NlogN)$ \martin{$O(N\log N)$} arm pulls, as in the UCB algorithm \{citation\}. \martin{Be more precise here. Include the success probability $\delta$ and the gaps between the best arm and other arms $\delta \mu_i$ in the expression.} This observation motivates the approach presented in this paper, in which we use an adaptation of the UCB algorithm to find medoids more quickly. 

% \ilan{we take too long to get here}

% Intuitively, in the BUILD step, we consider each of the $N$ candidate datapoints as an "arm", where an arm pull corresponds to computing the induced loss on a single reference datapoint by choosing the candidate in question as a medoid.  The multi-armed bandit (MAB) literature then suggests that we can identify the best medoid to assign with $O(NlogN)$ distance computations in each of the $k$ BUILD steps.

% Similarly, in the SWAP step, we consider each of the $k(N-k)$ medoid-nonmedoid pairs as an "arm", and an arm pull corresponds to computing the loss induced on a reference point by swapping the medoid with the non-medoid. The multi-armed bandit (MAB) literature then suggests that we can identify the best swap to perform with $O(kNlogN)$ distance computations in each SWAP step.

% Intuitively, in each of the BUILD and SWAP steps, we convert the computation of the sum for each candidate $m_l$ in \ref{eqn:build-next-medoid} or $(m,x)$ in \ref{eqn:swap-td} into a sampling problem. Instead of computing the sums exactly, we compute confidence intervals that contain the sum with high probability and explore promising arms more while expending less computation on unpromising arms. We expect such a UCB-based approach to recover the true best arm, thus matching the results of the greedy algorithm PAM, with high probability.  We formally describe the algorithm in Section \ref{algo}, along with theoretical guarantees for correctness in Section \ref{theory}.

% \subsection{Main Contributions}

% In this work, we:

% \begin{enumerate}
%     \item Propose a new algorithm, \algnamenospace, that uses a UCB-based algorithm to find a solution to the $k$-medoids problem,
%     \item Provide theoretical guarantees as to when UltraPAM will return the same results as current state-of-the-art methods such as PAM, and
%     \item Experimentally validate our approach on a number of real-world datasets.
% \end{enumerate}


% \martin{END of martin's version of Intro+Formulation}

==> old/preliminaries06-04.tex <==
% !TEX root = 0-main.tex

\section{Preliminaries}
\label{sec:prelims}
% \martin{I omitted the dimension $d$ because the points may not be represented by a vector}
For $n$ data points $\mathcal{X} =  \{ x_1, x_2, \cdots, x_n \}$ and a user-specified distance function $d(\cdot, \cdot)$, the $k$-medoids problem aims to find a set of $k$ medoids $\mathcal{M} = \{m_1, \cdots, m_k \} \subset \mathcal{X}$ to minimize the overall distance of points from their closest medoids:
% , as described in Eq.~\eqref{eqn:sec_intro_total-loss}.
% \martin{I think it's better to have a formal statement here}
\begin{equation} \label{eqn:total-loss}
	L(\mathcal{M}) =  \sum_{i=1}^n \min_{m_l \in \mathcal{M}} d(m_l, x_i)
\end{equation}
Note that one could use an arbitrary $d$ above, even one that is not a distance function ($d$ does not need to satisfy symmetry, triangle inequality, or positivity). 
For the rest of the paper, we use $[n]$ to denote the set $\{1,\cdots,n\}$.
For a set $\mathcal{S}$, $\vert \mathcal{S} \vert$ represents its cardinality.
For two scalars $a,b$, $a\wedge b = \min(a,b)$ and $a\vee b = \max(a,b)$.

% We first describe the original PAM algorithm \cite{kaufman1987clustering, kaufman1990partitioning}, and then describe our algorithm that is built upon PAM.

\subsection{Partitioning Around Medoids (PAM)}
The original PAM algorithm \cite{kaufman1987clustering, kaufman1990partitioning} first initializes the set of $k$ medoids via the BUILD step and then repeatedly performs the SWAP step to improve the loss \eqref{eqn:total-loss} until convergence.
% \mo{Reinforce that PAM is best quality}
% The BUILD step and the SWAP step are detailed as below. 

\paragraph{BUILD:} In the BUILD step, PAM selects an initial set of $k$ medoids by greedily adding one point at a time so as to minimize the overall loss \eqref{eqn:total-loss}. 
The first point added in this manner is the medoid of all $n$ points.
Given the current set of $l$ medoids $\mathcal{M}_{l} = \{m_1, \cdots, m_{l}\}$, the next point to add $m^*$ can be written as
\begin{equation}
\label{eqn:build-next-medoid}
    \text{BUILD~search:~~~~}m^* = \argmin_{x \in \mathcal{X} \setminus \mathcal{M}_{l}} \frac{1}{n} \sum_{j=1}^n \left[d(x, x_j) \wedge \min_{m' \in \mathcal{M}_{l}} d(m', x_j)\right]. 
\end{equation}

\paragraph{SWAP:} In the SWAP step, PAM swaps the medoid-nonmedoid pair that would reduce the loss \eqref{eqn:total-loss} the most among all possible $k(n-k)$  such pairs.
Let $\mathcal{M}$ be the current set of $k$ medoids. Then the best pair to swap is
\begin{equation}
\label{eqn:next-swap}
    \text{SWAP~search:~~~~}(m^*, x^*) = \argmin_{(m,x) \in \mathcal{M} \times (\mathcal{X} \setminus \mathcal{M}) } \frac{1}{n} \sum_{j=1}^n \left[d(x, x_j) \wedge \min_{m' \in \mathcal{M}\setminus \{m\}} d(m', x_j) \right]. 
\end{equation}

The second term in \eqref{eqn:build-next-medoid}, namely $\min_{m' \in \mathcal{M}_{l}} d(m', x_j)$, can be determined by caching the smallest distance from each point to the previous set of medoids $\mathcal{M}_{l}$.
Similarly, the second term \eqref{eqn:next-swap}, namely $\min_{m' \in \mathcal{M}\setminus \{m\}} d(m', x_j)$, can be determined by caching the smallest and the second smallest distances from each point to the previous set of medoids $\mathcal{M}$.
Therefore, in for both \eqref{eqn:build-next-medoid} and \eqref{eqn:next-swap}, we only need to compute the distance once for each term in the summation.
As a result, the time complexity of PAM is $O(kn^2)$ for $k$ greedy searches in the entire BUILD subroutine and $O(kn^2)$ for each SWAP iteration. We refer to the sequence of medoids selected by the BUILD step and the swaps performed by the SWAP step as the optimization trajectory of PAM.

==> old/theory05-28.tex <==
% !TEX root = main.tex

\martin{State and discuss all assumptions first before stating the theorems.}

In this section, we provide theoretical guarantees for when the UltraPAM algorithm will return the same results as PAM. 

Intuitively, in the BUILD step we reduce the problem of finding the best new medoid amongst all candidates to a best-arm identification problem. In this analogy, the contribution of a reference point $x_{ref}$ to the total loss \ref{TotalLoss} if we were to add candidate $x_c$ as a medoid corresponds to a reward from pulling the arm labeled $x_c$. With high probability, UltraPAM's BUILD step then returns the same initialized medoids as PAM. We formalize this in Theorem 1.

\paragraph{Theorem 1:} Given a finite, bounded dataset $D$. Suppose that given any $\mathcal{M}$, the minimizer of Equation \ref{build-next-medoid} is unique and that for each $x_i$, $\Delta TD_{x_i}$ (as defined in Equation \ref{build-TD}) is a $\sigma$-sub-Gaussian random variable. Then Algorithm 1 terminates in $O(kNlogN)$ calls to the distance metric $d$ and returns the same results as PAM with probability at least $1 - kN\delta$.

\paragraph{Proof of Theorem 1:} The proof is a relatively straightforward adaptation of the proof for best-arm-identification algorithms and is provided in the Appendix.

In the SWAP step, we again reduce the problem of finding the best medoid-nonmedoid pair $(x_m, x_o)$ to a a best-arm identification problem. In this analogy, the contribution of a reference point $x_{ref}$ to the total loss \ref{TotalLoss} if we were to swap medoid $x_m$ with non-medoid $x_o$ corresponds to a reward from pulling the arm labeled by the pair $(x_m, x_o)$. With high probability, UltraPAM then swaps the same medoid-nonmedoid pair that PAM would. We formalize this in Theorem 2.

\paragraph{Theorem 2:} Given a finite, bounded dataset $D$ and initial set of medoids $\mathcal{M'}$, where $|\mathcal{M}| = k$. Suppose that given any $\mathcal{M}$, the minimizer of Equation 6 is unique and that for each pair $(x_m, x_o)$, $\Delta TD_{(x_m, x_o)}$ (as defined in Equation 7) is a $\sigma$-sub-Gaussian random variable. Then Algorithm 2 terminates in $O(kNlogN)$ calls to the distance metric $d$ and returns the same results as PAM with probability at least $1 - kN\delta$.

\paragraph{Proof of Theorem 2:} Similar to the proof of Theorem 1, the proof of Theorem 2 is a relatively straightforward adaptation of the proof for best-arm-identification algorithms and is provided in the Appendix.

We note that the assumptions of Theorems 1 and 2 are unnecessarily strong and can probably be relaxed; we discuss these relaxations in the Future Work and Appendix sections.

\paragraph{Corollary 1:} Let $T$ be the number of SWAP steps performed by the PAM algorithm. With probability at least $1 - (T+1)kN\delta$, the entire UltraPAM algorithm returns the same result as PAM.

\paragraph{Proof of Corollary 1:} From Theorem 1, the probability of UltraPAM and PAM disagreeing in the BUILD step is at most $kN\delta$. Similarly, from Theorem 2, the probability of UltraPAM and PAM disagreeing in each SWAP step is also at most $kN\delta$. Note that if UltraPAM takes more than $T$ SWAP steps to complete, then UltraPAM disagreed with PAM in either the BUILD step or one of the first $T$ SWAP steps. The result then follows by a union bound over the probabilities of error in the BUILD step or any of the first $T$ SWAP steps.

The above results provide conditions under which UltraPAM returns the same results as PAM with high probability. In practice, the authors observe that $T$ is usually very small and almost always smaller than $k$. If necessary, a maximum on the number of SWAP steps or similar early stopping criteria can be specified (such as required decrease in total loss per swap step), as is often the case in practice with iterative algorithms.

==> old/theory06-03.tex <==
% !TEX root = 0-main.tex

\section{Analysis of the Algorithm}
\label{theory}

\mo{I feel that we should be more explicit about what "optimization trajectory" is earlier in the paper}
The goal of \algname
% , described in Algorithms~\ref{alg:ultrapam-build} and \ref{alg:ultrapam-swap} seeks 
is to track the optimization trajectory of the standard PAM algorithm, ultimately identifying the same set of $k$ medoids as PAM with high probability.
In this section, we formalize this statement
and provide bounds on the total number of distance computations required by Bandit-PAM.

Suppose that the standard PAM algorithm is run on a dataset $\X = \{x_1,...,x_n\}$.
Let $\tilde \M_{\rm B} = \{\tilde m_1,...,\tilde m_k\}$ be the $k$ medoids identified in the BUILD step of PAM.
From (\ref{eqn:build-next-medoid}) and (\ref{eqn:build-next-medoid-td}), we see that if we define $\bar L_x = \frac1n \sum_{j=1}^n L_{x}(x_j)$, then the $l$th medoid is given by $\tilde m_l = \argmin_{x \in \mathcal{X} \setminus \mathcal{M}} \bar L_x$.
Moreover, if $J$ is a random variable, chosen uniformly at random from $\{1,...,n\}$, $E[L_x(x_J)]= \bar L_x$.
As described in Algorithm~\ref{alg:ultrapam-build}, we estimate $\bar L_x$ by averaging $L_x(x_J)$ for several randomly chosen indices.



\begin{algorithm}[t]
\caption{\texttt{\algname BUILD($\X, \mathcal{M} = \{m_1, \cdots, m_{l-1}\},\batchsize$):} 
%\Comment{Dataset $X$ of size $N$, number of medoids $k_{max}$, distance function $d$} 
\label{alg:build-step}}
\begin{algorithmic}[1]
\State $\arms \leftarrow \X - \M$
\State $N \gets 0$  % \Comment{Number of times each arm has been pulled}
\State $\hat L = (0, ..., 0)$, $C_i = (\infty,...,\infty)$ \Comment{Initial mean and confidence interval for each arm}
% \While{{\bf true}}
% \While{$|\arms| > 1$} % and $C_y > 0$ for some arm $y$}
\While{$N < n$ and $|\arms| > 1$} % and $C_y > 0$ for some arm $y$}
        \State Draw a random sample (with replacement) of $\batchsize$ reference points $\X_{\rm ref} \subset \X$ 
        \ForAll{$x \in \arms$}
            \State $\hat L_x \leftarrow \frac{ N \hat L_x + \sum_{y \in \X_{\rm ref}}L_{x}(y)}{N + \batchsize }$ \Comment{Update running average}
            \State $C_x \gets \sigma_x \sqrt{  \frac{ 2 \log(\frac{1}{\delta}) } {N + \batchsize }}$
            \Comment{Update confidence interval}        
        \EndFor
    \State $\arms \leftarrow \{x : \hat L_x - C_x \leq \min_{y}(\hat L_{y} + C_{y})\}$ \Comment{Remove arms that can no longer be chosen}
    \State $N \leftarrow N + \batchsize$
\EndWhile
\If{|\arms| = 1}
    \State \textbf{return} $x^* \in \arms$
\Else
    \State Compute $\bar L_x$ (exactly) for all $x \in \arms$
    \State \textbf{return} $x^* \argmin_{x \in \arms} \bar L_x$
\EndIf
% \ForAll{$x \in \arms$} 
%     \State Set $\hat L_x = \frac1n \sum_{j = 1}^n L_{x}(x_j)$ and $C_x = 0$
%     \Comment Arm return is computed exactly
% \EndFor    
% % \State Append $x_i$ to $\mathcal{M}$, where $i = \argmin_iB_i$
% % \State \textbf{return} $\mathcal{M}$
% \State \textbf{return} $x \in \arms$
\end{algorithmic}
\end{algorithm}


% \begin{algorithm}[t]
% \caption{\texttt{\algname BUILD($\X, \mathcal{M} = \{m_1, \cdots, m_{l-1}\},\batchsize$):} 
% %\Comment{Dataset $X$ of size $N$, number of medoids $k_{max}$, distance function $d$} 
% \label{alg:build-step}}
% \begin{algorithmic}[1]
% \State $\arms \leftarrow \X - \M$
% \State $T \leftarrow (0, ..., 0)$ \Comment{Number of times each arm has been pulled}
% \State $\hat L = (0, ..., 0)$, $C_i = (\infty,...,\infty)$ \Comment{Initial mean and confidence interval for each arm}
% % \While{{\bf true}}
% \While{$|\arms| > 1$} % and $C_y > 0$ for some arm $y$}
% % \While{$N > 1$} % and $C_y > 0$ for some arm $y$}
%         \ForAll{arms $x$ with $T_x \geq n$} 
%             \State Set $\hat L_x = \frac1n \sum_{j = 1}^n L_{x}(x_j)$ and $C_x = 0$
%             \Comment Arm return is computed exactly
%         % \State Compute $\sum_{j = 1}^N \Delta L_{x_i}(x_j)$ exactly \Comment Over all datapoints
%         % \State Set $B_i = M_i = U_i = \sum_{j = 1}^N \Delta L_{x_i}(x_j)$ \Comment Arm return is known exactly
%         \EndFor
%         \State Draw a random sample (with replacement) of $\batchsize$ reference points $\X_{\rm ref} \subset \X$ 
%         \ForAll{arms $x$ with $T_x < n$}
%             \State $\hat L_x \leftarrow \frac{ T_x \hat L_x + \sum_{y \in \X_{\rm ref}}L_{x}(y)}{T_x + \batchsize }$ \Comment{Update running average}
%             \State $T_x \leftarrow T_x + \batchsize$
%             \State $C_x \gets \sigma_x \sqrt{  \frac{ 2 \log(\frac{1}{\delta}) } {T_x}}$
%             \Comment{Update confidence interval}        
%         % \State $M_i \leftarrow \frac{ T_iM_i + \sum_{x_{\rm ref}}\Delta L_{x_i}(x_{\rm ref})}{T_i + batch\_size}$ \Comment{Update running average}
%         % \State $T_i \leftarrow T_i + batch\_size$
%         % \State $C_i \leftarrow \sigma_i \sqrt{ \frac{ \log(\frac{1}{\delta}) } {T_i}}$
%         % \State $B_i \leftarrow M_i - C_i$, $U_i \leftarrow M_i + C_i$ \Comment{Update confidence interval}
%         \EndFor
%     % \State $\arms \leftarrow \{i : B_i \leq \min_i(U_i)\}$ \Comment{Arms to pull must overlap with lowest CI}
%     \State $\arms \leftarrow \{x : \hat L_x - C_x \leq \min_{y}(\hat L_{y} + C_{y})\}$ \Comment{Remove arms that can no longer be chosen}
% \EndWhile
% % \State Append $x_i$ to $\mathcal{M}$, where $i = \argmin_iB_i$
% % \State \textbf{return} $\mathcal{M}$
% \State \textbf{return} $x \in \arms$
% \end{algorithmic}
% \end{algorithm}




% \begin{algorithm}[t]
% \caption{\texttt{\algname BUILD($\X, \mathcal{M} = \{m_1, \cdots, m_{l-1}\}, \delta$):} 
% %\Comment{Dataset $X$ of size $N$, number of medoids $k_{max}$, distance function $d$} 
% \label{alg:build-step}}
% \begin{algorithmic}[1]
% \State $\arms \leftarrow \X - \M$
% \State $T \leftarrow (0, ..., 0)$ \Comment{Number of times each arm has been pulled}
% \State $\hat L = (0, ..., 0)$, $C_i = (\infty,...,\infty)$ \Comment{Initial mean and confidence interval for each arm}
% % \While{{\bf true}}
% \While{$|\arms| > 1$ and $C_y > 0$ for some arm $y$}
%     \State Choose arm $x = \argmin_{y \in \arms} \hat L_y - C_y$
%     \If{$T_x = n$}
%         % \State Compute $L_{x}(x_j)$ for all $x_j \in \X$ \Comment Over all datapoints
%         \State Set $\hat L_x = \frac1n \sum_{j = 1}^n L_{x}(x_j)$ and $C_x = 0$
%         \Comment Arm return is computed exactly
%     \Else    
%         \State Draw a reference point $x_{\rm ref}$ uniformly at random from $\X$  
%         \State $\hat L_x \leftarrow \frac{ T_x \hat L_x + L_{x}(x_{\rm ref})}{T_x + 1 }$ \Comment{Update running average}
%         \State $T_x \leftarrow T_x + 1$
%         \State $C_x \gets \sigma_x \sqrt{  \frac{ 2 \log(\frac{1}{\delta}) } {T_x}}$
%         \Comment{Update confidence interval}
%     \EndIf
% \State $\arms \leftarrow \{x : \hat L_x - C_x \leq \min_{y}(\hat L_{y} + C_{y})\}$ \Comment{Remove arms that can no longer be chosen}
% \EndWhile
% % \State Append $x_i$ to $\mathcal{M}$, where $i = \argmin_iB_i$
% % \State \textbf{return} $\mathcal{M}$
% \State \textbf{return} $x \in \arms$
% \end{algorithmic}
% \end{algorithm}




% \ilan{One issue is that current Algorithm 1 tries to learn $\sigma_x$, but we don't want to have to analyze that. 
% Algorithm 3 corresponds to a single build step.
% We may want to move the longer ``actual'' algorithm to the appendix.
% Maybe we should combine BUILD and SWAP steps into the same algorithm? We can then remark that BUILD is a SWAP step where some of the medoids is set to infinity.}



In order to provide a guarantee on the number of distance computations required to identify the $l$th medoid, we let $\Delta_x = \bar L_x - \bar L_{\tilde m_\ell}$.
Moreover, we assume that the random variable $Y = L_x(x_J)$ is $\sigma$-sub-Gaussian; i.e., that $\Pr(|Y-E[Y]| > t) < 2 \exp\left(-t^2/(2 \sigma^2)\right)$.
Notice that, strictly speaking, $Y = L_x(x_J)$ only takes value in a finite set and must be $\sigma$-sub-Gaussian for some $\sigma$. \martin{We need it to not depend on $n$} \ilan{The statement of the theorem is for a fixed $n$, so it still holds if $\sigma$ is a function of $n$. We could add a line after the theorem saying that, if $sigma_x^2/\Delta_x^2 = \Theta(1)$ for all $x$, then $M$ is $O(n\log n)$ with high probability.}
As we illustrate in Section~\ref{sec:experiments}, in practice $\sigma$ can be estimated from the data.
We also point out that $\sigma$ will be different for different arms (i.e., each candidate new medoid $x$) and will depend on which BUILD step we are in.
We then have the following guarantee.


\begin{theorem}
For $\delta = n^{-3}$, with probability at least $1-2/n$, Algorithm~\ref{alg:build-step} chooses the same $l$th medoid as PAM using a total of $M$ distance computations, where
% \aln{
% N \leq \sum_{x \in \X} \min \left( \frac{ 24 \sigma_x^2}{\Delta_x^2} \log n , 2n \right).
% }
\aln{
M \leq \sum_{x \in \X} \min \left[ \frac{24}{\Delta_x^2} \left(\sigma_x+\frac{ \sigma_{x^*}}{\sigma_x}\right)^2 \log n + \batchsize, 2n \right]
.
}
\end{theorem}
\martin{$M$ is a random variable. The bound here is a bit funny}
\ilan{I followed the statement of meddit. Is it not clear that ``with prob. $1-2/n$'' applies to the bound on $M$?}
\martin{I think a standard way is to upper bound $\mathbb{E}[M]$ ($\mathbb{E}[M] = \mathbb{E}[M \vert \text{bound holds}] + \mathbb{E}[M \vert \text{bound does not hold }] * \frac{2}{n}$)}

\begin{proof}
% Notice that, if more than $n$ distance computations are performed for a given arm $x$, the algorithm abandons the current estimate $\hat L_x$ and computes $\bar L_x$ exactly (which requires additional $n$ computations), setting $C_x = 0$.
% This guarantees that the algorithm must terminate.
% At the end, for arm $x$, the total number of distance computations will be either $T_x$ or $2n$. % if $T_x = n$.
First, we show that, with probability $1-1/n$, all confidence intervals computed throughout the algorithm are true confidence intervals. \mo{need to be more explicit about what is "true" CI}
To see this, notice that for a fixed $x$ and a fixed iteration of the algorithm, $\hat L_x$ is the average of $N$ i.i.d.~samples of a $\sigma_x$-sub-Gaussian distribution.
From Hoeffding's inequality, 
\aln{
\Pr\left( \left| \bar L_x - \hat L_x \right| > C_x \right) \leq 2 \exp \left({-\frac{N C_x^2}{2\sigma_x^2}}\right)  = 2 \delta.
% \\
% \sigma_x \sqrt{ \frac{2 \log(\frac{1}{\delta}) } {T_x}}
}
Notice that there are at most $n^2/\batchsize \leq n^2$ such confidence intervals computed across all arms and all steps of the algorithm.
If we set $\delta = 1/n^3$, we see that $\bar L_x \in [\hat L_x - C_x, \hat L_x + C_x]$ for every $x$ and for every step of the algorithm with probability at least $1-2/n$, by the union bound.

Let $x^* = \argmin_{x \in \arms} \bar L_x$.
Notice that if all confidence intervals throughout the algorithm are correct, it is impossible for $x^*$ to be removed from the set of candidate arms. 
Moreover, it is clear that the main while loop in the algorithm can only run $n/\batchsize$ times and that the algorithm must terminate.
Hence, $x^*$ (or some $y$ with $\bar L_y = \bar L_{x^*}$) must be returned upon termination.


% Now consider a suboptimal arm $x \ne x^*$. 
Let $N$ be the total number of arm pulls computed for each of the arms remaining in the set of candidate arms at some point in the algorithm.
Notice that, for any suboptimal arm $x \ne x^*$ that has not left the set of candidate arms, we must have
\aln{
C_x = \sigma_x \sqrt{ 2 \log(\tfrac{1}{\delta}) /N } = \frac{\sigma_{x}}{\sigma_{x^*}} C_{x^*}.
}
% Hence, if $N$
Moreover, if $N > \frac{24}{\Delta_x^2} \left(\sigma_x+\frac{ \sigma_{x^*}}{\sigma_x}\right)^2 \log n$,
% if $N > (24 \sigma_x^2 \log n)/(\Delta_x^2 \sigma_{x^*}^2) \log n$, 
we have that
\aln{
2(C_x + C_{x^*}) = 2 \left( \sigma_x + \frac{\sigma_{x^*}}{\sigma_x}\right) \sqrt{  \frac{ 2 \log(n^3) } {N  }} \leq \bar L_x - \bar L_{x^*} = \Delta_x,
}
we have that
$
\hat L_x - C_x > \bar L_x - 2C_x = \bar L_{x^*} + \Delta_x - 2C_x 
\geq \bar L_{x^*} + 2 C_{x^*} > \hat L_{x^*} + C_{x^*},
$
% \aln{
% \hat L_x - C_x & > \bar L_x - 2C_x = \bar L_{x^*} + \Delta_x - 2C_x 
% = \bar L_{x^*} + \Delta_x - {2\sigma_x} \sqrt{  2 \log(n^3) / N } \\
% & > \bar L_{x^*} + \Delta_x - {2\sigma_x} \Delta_x \frac{ \sigma_x }{2 + \sigma_{x^*}} = 
% \\
% & \geq \bar L_{x^*} + 2 C_{x^*} = \hat L_{x^*} + C_{x^*},
% }
implying that $x$ must be removed from the set of candidate arms at the end of that iteration.
Hence, the number of distance computations required for each arm $x \ne x^*$ is at most
\aln{
\min \left[ \frac{24}{\Delta_x^2} \left(\sigma_x+\frac{ \sigma_{x^*}}{\sigma_x}\right)^2 \log n + \batchsize, 2n \right],
}
concluding the proof of the theorem.
\end{proof}


\martin{Need a theorem giving $O(n \log n)$ from the instance-specific bound $M \leq \sum_{x \in \X} \min \left[ \frac{24}{\Delta_x^2} \left(\sigma_x+\frac{ \sigma_{x^*}}{\sigma_x}\right)^2 \log n + \batchsize, 2n \right]
.$}

\martin{Need a theorem giving the overall correctness assuming the number of SWAP iterations $T$.}


--- OLD STUFF



\noindent {\bf Assumptions:} 
Similar to the work by Bagaria et al.~\cite{bagaria2018medoids}, which focuses on the computation of a single medoid, we need an assumption regarding the distribution of pairwise distances.
We assume that the $n$ data points belong to true clusters $\Ct_1, \Ct_2, ..., \Ct_k$ \ilan{different $k$?}.
For a pair of points $x_1$ and $x_2$, their distance $d(x_1,x_2)$ is assumed to be a $\sigma_{\rm in}$-sub-Gaussian random variable if $x_1$ and $x_2$ are in the same true cluster, while it is a a $\sigma_{\rm out}$-sub-Gaussian random variable if $x_1$ and $x_2$ are in different clusters, for $\sigma_{\rm in} < \sigma_{\rm out}$.
The true clusters $\Ct_1, \Ct_2, ..., \Ct_k$ and the parameters $\sigma_{\rm in}$ and $\sigma_{\rm out}$ are not known a priori.
\ilan{maybe a single $\sigma$ is ok}

% \ilan{we may have to be a bit careful with whether $\sigma$ is known for the theoretical results}

% \ilan{one theorem for BUILD and one for SWAP? Or one for equality with PAM and one for number of distance computations?}



% \ilan{Maybe the best approach will be to assume, for the theory, part that all distances have a bounded support, like $[0,1]$. But then the adaptive $\sigma$ doesn't make sense...}




\martin{State and discuss all assumptions first before stating the theorems.}

In this section, we provide theoretical guarantees for when the UltraPAM algorithm will return the same results as PAM. 

Intuitively, in the BUILD step we reduce the problem of finding the best new medoid amongst all candidates to a best-arm identification problem. In this analogy, the contribution of a reference point $x_{ref}$ to the total loss \ref{TotalLoss} if we were to add candidate $x_c$ as a medoid corresponds to a reward from pulling the arm labeled $x_c$. With high probability, UltraPAM's BUILD step then returns the same initialized medoids as PAM. We formalize this in Theorem 1.

\paragraph{Theorem 1:} Given a finite, bounded dataset $D$. Suppose that given any $\mathcal{M}$, the minimizer of Equation \ref{build-next-medoid} is unique and that for each $x_i$, $\Delta TD_{x_i}$ (as defined in Equation \ref{build-TD}) is a $\sigma$-sub-Gaussian random variable. Then Algorithm 1 terminates in $O(kNlogN)$ calls to the distance metric $d$ and returns the same results as PAM with probability at least $1 - kN\delta$.

\paragraph{Proof of Theorem 1:} The proof is a relatively straightforward adaptation of the proof for best-arm-identification algorithms and is provided in the Appendix.

In the SWAP step, we again reduce the problem of finding the best medoid-nonmedoid pair $(x_m, x_o)$ to a a best-arm identification problem. In this analogy, the contribution of a reference point $x_{ref}$ to the total loss \ref{TotalLoss} if we were to swap medoid $x_m$ with non-medoid $x_o$ corresponds to a reward from pulling the arm labeled by the pair $(x_m, x_o)$. With high probability, UltraPAM then swaps the same medoid-nonmedoid pair that PAM would. We formalize this in Theorem 2.

\paragraph{Theorem 2:} Given a finite, bounded dataset $D$ and initial set of medoids $\mathcal{M'}$, where $|\mathcal{M}| = k$. Suppose that given any $\mathcal{M}$, the minimizer of Equation 6 is unique and that for each pair $(x_m, x_o)$, $\Delta TD_{(x_m, x_o)}$ (as defined in Equation 7) is a $\sigma$-sub-Gaussian random variable. Then Algorithm 2 terminates in $O(kNlogN)$ calls to the distance metric $d$ and returns the same results as PAM with probability at least $1 - kN\delta$.

\paragraph{Proof of Theorem 2:} Similar to the proof of Theorem 1, the proof of Theorem 2 is a relatively straightforward adaptation of the proof for best-arm-identification algorithms and is provided in the Appendix.

We note that the assumptions of Theorems 1 and 2 are unnecessarily strong and can probably be relaxed; we discuss these relaxations in the Future Work and Appendix sections.

\paragraph{Corollary 1:} Let $T$ be the number of SWAP steps performed by the PAM algorithm. With probability at least $1 - (T+1)kN\delta$, the entire UltraPAM algorithm returns the same result as PAM.

\paragraph{Proof of Corollary 1:} From Theorem 1, the probability of UltraPAM and PAM disagreeing in the BUILD step is at most $kN\delta$. Similarly, from Theorem 2, the probability of UltraPAM and PAM disagreeing in each SWAP step is also at most $kN\delta$. Note that if UltraPAM takes more than $T$ SWAP steps to complete, then UltraPAM disagreed with PAM in either the BUILD step or one of the first $T$ SWAP steps. The result then follows by a union bound over the probabilities of error in the BUILD step or any of the first $T$ SWAP steps.

The above results provide conditions under which UltraPAM returns the same results as PAM with high probability. In practice, the authors observe that $T$ is usually very small and almost always smaller than $k$. If necessary, a maximum on the number of SWAP steps or similar early stopping criteria can be specified (such as required decrease in total loss per swap step), as is often the case in practice with iterative algorithms.

==> old/theory06-04.tex <==
% !TEX root = 0-main.tex

\section{Analysis of the Algorithm}
\label{sec:theory}

% \mo{I feel that we should be more explicit about what "optimization trajectory" is earlier in the paper}
The goal of \algname
% , described in Algorithms~\ref{alg:ultrapam-build} and \ref{alg:ultrapam-swap} seeks 
is to track the optimization trajectory of the standard PAM algorithm, ultimately identifying the same set of $k$ medoids as PAM with high probability.
In this section, we formalize this statement
and provide bounds on the total number of distance computations required by Bandit-PAM.

Suppose that PAM is run on a dataset $\X = \{x_1,...,x_n\}$.
Let $\tilde \M_{\rm B} = \{\tilde m_1,...,\tilde m_k\}$ be the $k$ medoids identified in the BUILD step of PAM, and let $(x_{i_1},y_{i_1}),(x_{i_2},y_{i_2}),...,(x_{i_T},y_{T_1})$ \martin{$y_{T_1}$ should be $y_{i_T}$?} be the full sequence of PAM SWAPS, for $\left(x_{i_j}, y_{i_j}\right) \in \X \times \X$, $j=1,..., T$.
Both the set of initial medoids found by BUILD and the set of SWAP steps for PAM can be recursively defined via \eqref{eqn:build_search} and \eqref{eqn:swap_search}.
% 
This means that, provided that \algname picks the same initial $k$ medoids and performs the same swaps as PAM, $k + T$ calls to Algorithm~\ref{alg:bandit_based_search} will be performed.

Consider one such call to Algorithm~\ref{alg:bandit_based_search} and suppose $x^*$ is the optimal target point (i.e., the one with minimum $\mu_x$).
% In order to provide a guarantee on the total number of distance computations required by \algnamenospace, we consider each of the calls to Algorithm~\ref{alg:bandit_based_search} individually.
For another target point $x \in \Star$,
% in a given call to Algorithm~\ref{alg:bandit_based_search}, 
let $\Delta_x = \mu_x - \mu_{x^*}$.
To state the next result, we will assume that, for a randomly sampled reference point, say $x_J$,
the random variable $Y = g_x(x_J)$ is $\sigma$-sub-Gaussian; i.e., that $\Pr(|Y-E[Y]| > t) < 2 \exp\left(-t^2/(2 \sigma^2)\right)$.
%and that 
% Notice that, strictly speaking, $Y = L_x(x_J)$ only takes value in a finite set and must be $\sigma$-sub-Gaussian for some $\sigma$. \martin{We need it to not depend on $n$} \ilan{The statement of the theorem is for a fixed $n$, so it still holds if $\sigma$ is a function of $n$. We could add a line after the theorem saying that, if $sigma_x^2/\Delta_x^2 = \Theta(1)$ for all $x$, then $M$ is $O(n\log n)$ with high probability.}
Moreover, we assume that $\sigma/\min_x \Delta_x = O(1)$ for all calls to Algorithm~\ref{alg:bandit_based_search}.
Later, we discuss the practical implications of these assumptions\iscomment{}.
% As we illustrate in Section~\ref{sec:exps}, in practice $\sigma$ can be estimated from the data.
% We then have the following result.


\begin{theorem} \label{thm:nlogn}
Suppose that, on a dataset $\X$, the PAM algorithm converges after $T$ SWAP steps.
If \algname is run on $\X$ with $\delta = n^{-3}$, then it returns the same set of $k$ medoids as PAM with probability $1-2(k+T)/n$. 
Furthermore, with probability $1-2(k+T)/n$, the total number of distance computations $M$ required 
\al{
M = O\left( (k+T) n \log n \right).
}
\end{theorem}
\ilan{it's a bit tricky to get an expected result for theorem 1, since in principle Bandit-PAM could keep running forever. one solution would be to only allow $\log n$ SWAPS}

When the number of desired medoids $k$ is a constant and the number of PAM SWAP steps is small (which is often the case in practice), 
Theorem~\ref{thm:nlogn} implies that only $O(n \log n)$ distance computations are necessary to reproduce the results of PAM with high probability.

In order to prove Theorem~\ref{thm:nlogn}, we prove a more detailed result for each call that \algname does to Algorithm~\ref{alg:bandit_based_search}.
For this more specific case, we assume that, for target point $x$, $g_x(x_J)$ is $\sigma_x$-sub-Gaussian, where $\sigma_x$ is a parameter specific to $x$ (and can change across different calls to Algorithm~\ref{alg:bandit_based_search}).
As it turns out, in practice one can estimate each $\sigma_x$ by performing a small number of distance computations.
As we show in Section~\ref{sec:exps}, allowing $\sigma_x$ to be estimated separately for each arm, is beneficial in practice.


% As we illustrate in Section~\ref{sec:exps}, in practice $\sigma$ can be estimated from the data.

% \ilan{say this later}
% We also point out that $\sigma$ will be different for different target points $x$, and will be different across different calls to Algorithm~\ref{alg:bandit_based_search}.
% % arms (i.e., each candidate new medoid $x$) and will depend on which BUILD step we are in.
% We then have the following guarantee.


\begin{theorem} \label{thm:specific}
For $\delta = n^{-3}$, with probability at least $1-\tfrac{2}{n}$, Algorithm~\ref{alg:bandit_based_search}
returns the correct solution to \eqref{eqn:build_search} (for a BUILD step) or \eqref{eqn:swap_search} (for a SWAP step),
using a total of $M$ distance computations, where
% \aln{
% N \leq \sum_{x \in \X} \min \left( \frac{ 24 \sigma_x^2}{\Delta_x^2} \log n , 2n \right).
% }
% \aln{
% M \leq \sum_{x \in \X} \min \left[ \frac{24}{\Delta_x^2} \left(\sigma_x+\frac{ \sigma_{x^*}}{\sigma_x}\right)^2 \log n + \batchsize, 2n \right]
% .
% }
\aln{
E[M] \leq 4n + \sum_{x \in \X}  \min \left[ \frac{24}{\Delta_x^2} \left(\sigma_x+\sigma_{x^*} \right)^2 \log n + \batchsize, 2n \right].
}
\end{theorem}
% \martin{$M$ is a random variable. The bound here is a bit funny}
% \ilan{I followed the statement of meddit. Is it not clear that ``with prob. $1-2/n$'' applies to the bound on $M$?}
% \martin{I think a standard way is to upper bound $\mathbb{E}[M]$ ($\mathbb{E}[M] = \mathbb{E}[M \vert \text{bound holds}] + \mathbb{E}[M \vert \text{bound does not hold }] * \frac{2}{n}$)}

\begin{proof}[Proof of Theorem~\ref{thm:specific}]
% Notice that, if more than $n$ distance computations are performed for a given arm $x$, the algorithm abandons the current estimate $\hat L_x$ and computes $\bar L_x$ exactly (which requires additional $n$ computations), setting $C_x = 0$.
% This guarantees that the algorithm must terminate.
% At the end, for arm $x$, the total number of distance computations will be either $T_x$ or $2n$. % if $T_x = n$.
First, we show that, with probability $1-\tfrac{2}{n}$, all confidence intervals computed throughout the algorithm are true confidence intervals, in the sense that they contain the true parameter $\mu_x$.
% \mo{need to be more explicit about what is "true" CI}
To see this, notice that for a fixed $x$ and a fixed iteration of the algorithm, $\hat \mu_x$ is the average of $\nuref$ i.i.d.~samples of a $\sigma_x$-sub-Gaussian distribution.
From Hoeffding's inequality, 
\aln{
\Pr\left( \left| \mu_x - \hat \mu_x \right| > C_x \right) \leq 2 \exp \left({-\frac{\nuref C_x^2}{2\sigma_x^2}}\right)  = 2 \delta.
% \\
% \sigma_x \sqrt{ \frac{2 \log(\frac{1}{\delta}) } {T_x}}
}
Notice that there are at most $n^2/\batchsize \leq n^2$ such confidence intervals computed across all target points (i.e., arms) and all steps of the algorithm.
If we set $\delta = 1/n^3$, we see that $\mu_x \in [\hat \mu_x - C_x, \hat \mu_x + C_x]$ for every $x$ and for every step of the algorithm with probability at least $1-2/n$, by the union bound.

Let $x^* = \argmin_{x \in \Star} \mu_x$.
Notice that if all confidence intervals throughout the algorithm are correct, it is impossible for $x^*$ to be removed from the set of candidate target points. 
Moreover, it is clear that the main while loop in the algorithm can only run $n/\batchsize$ times and that the algorithm must terminate.
Hence, $x^*$ (or some $y \in \Star$ with $\mu_y = \mu_{x^*}$) must be returned upon termination.


% Now consider a suboptimal arm $x \ne x^*$. 
Let $\nuref$ be the total number of arm pulls computed for each of the arms remaining in the set of candidate arms at some point in the algorithm.
Notice that, for any suboptimal arm $x \ne x^*$ that has not left the set of candidate arms, we must have
$C_x = \sigma_x \sqrt{ 2 \log(\tfrac{1}{\delta}) /\nuref}$.
% Hence, if $N$
Moreover, if $\nuref > \frac{24}{\Delta_x^2} \left(\sigma_x+\sigma_{x^*}\right)^2 \log n$,
% if $N > (24 \sigma_x^2 \log n)/(\Delta_x^2 \sigma_{x^*}^2) \log n$, 
we have that
\aln{
2(C_x + C_{x^*}) = 2 \left( \sigma_x + \sigma_{x^*}\right) \sqrt{  { 2 \log(n^3) } / {\nuref  }} < \Delta_x = \mu_x - \mu_{x^*},
}
and 
$
\hat \mu_x - C_x > \mu_x - 2C_x = \mu_{x^*} + \Delta_x - 2C_x 
\geq \mu_{x^*} + 2 C_{x^*} > \hat \mu_{x^*} + C_{x^*},
$
% \aln{
% \hat L_x - C_x & > \bar L_x - 2C_x = \bar L_{x^*} + \Delta_x - 2C_x 
% = \bar L_{x^*} + \Delta_x - {2\sigma_x} \sqrt{  2 \log(n^3) / N } \\
% & > \bar L_{x^*} + \Delta_x - {2\sigma_x} \Delta_x \frac{ \sigma_x }{2 + \sigma_{x^*}} = 
% \\
% & \geq \bar L_{x^*} + 2 C_{x^*} = \hat L_{x^*} + C_{x^*},
% }
implying that $x$ must be removed from the set of candidate arms at the end of that iteration.
Hence, the number of distance computations $M_x$ required for target point $x \ne x^*$ is at most
\aln{
M_x \leq \min \left[ \frac{24}{\Delta_x^2} \left( \sigma_x + \sigma_{x^*}\right)^2 \log n + \batchsize, 2n \right].
}
Notice that this holds simultaneously for all $x \in \Star$ with probability $1-\tfrac{2}{n}$.
We conclude that the total number of distance computations $M$ satisfies
\aln{
E[M] & \leq E[M | \text{ all confidence intervals are correct}] + \frac{2}{n} (2n^2) \\
& \leq 4n + \sum_{x \in \X}  \min \left[ \frac{24}{\Delta_x^2} \left( \sigma_x + \sigma_{x^*}\right)^2 \log n + \batchsize, 2n \right],
}
where we used the fact that the maximum number of distance computations per target point is $2n$.
% , if the confidence intervals are not all correct throughout the algorithm, which occurs with probability at most $\tfrac2\delta$, then we may use at most $2n$ computations per target point.
\end{proof}


% \martin{Need a theorem giving $O(n \log n)$ from the instance-specific bound $M \leq \sum_{x \in \X} \min \left[ \frac{24}{\Delta_x^2} \left(\sigma_x+\frac{ \sigma_{x^*}}{\sigma_x}\right)^2 \log n + \batchsize, 2n \right]
% .$}

% \martin{Need a theorem giving the overall correctness assuming the number of SWAP iterations $T$.}


While the assumption that $\sigma_x$ is known for every $x$ may seem excessive, it is worth pointing out that Algorithm~\ref{alg:bandit_based_search} does not need to know all $\sigma_x$s exactly and an upper bound is sufficient.
Notice that, if a random variable is $\sigma$-sub-Gaussian, it is also $\sigma'$-sub-Gaussian for $\sigma' > \sigma$.
Hence, if we have a universal upper bound $\sigma_{\rm ub}> \sigma_x$ for all $x$, the algorithm can be run assuming that with $\sigma_{\rm ub}$ replacing each $\sigma_x$.
In that case, a direct consequence of Theorem~\ref{thm:specific} is that the total number of distance computations would satisfy
\aln{
E[M] & \leq 4n + \sum_{x \in \X}  96 \frac{\sigma^2_{\rm ub}}{\Delta_x^2} \log n + \batchsize 
% \\
% & 
\leq  4n + 96 \left(\frac{\sigma_{\rm ub}}{\min_x \Delta_x}\right)^2
% \sum_{x \in \X}  \min (\log n + \batchsize, 2n)
n \log n.
}
Therefore, as long as $\sigma_{\rm ub}/\min_x \Delta_x = O(1)$,
each call to Algorithm~\ref{alg:bandit_based_search} requires, in expectation, $O(n \log n)$.
Moreover, from Theorem~\ref{thm:specific}, the probability that Algorithm~\ref{alg:bandit_based_search} does not return the target point with the smallest value is at most $2/n$.
Hence, if we assume that the PAM algorithm converges after $T$ SWAP steps, from the union bound, the probability that \algname does not return the same set of $k$ medoids as PAM is at most $2(k+T)/n$.
Provided that \algname correctly tracks the optimization trajectory of PAM (which occurs with probability $1-2(k+T)/n$), the total number of distance computations will be $M = O((k+T)n \log n)$.
This proves Theorem~\ref{thm:nlogn}.
\ilan{}





==> old/theory_05-30.tex <==
% !TEX root = main.tex


The goal of \algname
% , described in Algorithms~\ref{alg:ultrapam-build} and \ref{alg:ultrapam-swap} seeks 
is to track the optimization trajectory of the standard PAM algorithm, ultimately identifying the same set of $k$ medoids as PAM with high probability.
In this section, we formalize this statement
and provide bounds on the total number of distance computations required by Bandit-PAM.

Suppose that the standard PAM algorithm is run on a dataset $\X = \{x_1,...,x_n\}$.
Let $\tilde \M_{\rm B} = \{\tilde m_1,...,\tilde m_k\}$ be the $k$ medoids identified in the BUILD step of PAM.
From (\ref{eqn:build-next-medoid}) and (\ref{eqn:build-next-medoid-td}), we see that if we define $\bar L_x = \frac1n \sum_{j=1}^n L_{x}(x_j)$, then the $l$th medoid is given by $\tilde m_l = \argmin_{x \in \mathcal{X} \setminus \mathcal{M}} \bar L_x$.
Moreover, if $J$ is a random variable, chosen uniformly at random from $\{1,...,n\}$, $E[L_x(x_J)]= \bar L_x$.
As described in Algorithm~\ref{alg:ultrapam-build}, we estimate $\bar L_x$ by averaging $L_x(x_J)$ for several randomly chosen indices.



\begin{algorithm}[t]
\caption{\texttt{\algname BUILD($\X, \mathcal{M} = \{m_1, \cdots, m_{l-1}\},\batchsize$):} 
%\Comment{Dataset $X$ of size $N$, number of medoids $k_{max}$, distance function $d$} 
\label{alg:build-step}}
\begin{algorithmic}[1]
\State $\arms \leftarrow \X - \M$
\State $T \leftarrow (0, ..., 0)$ \Comment{Number of times each arm has been pulled}
\State $\hat L = (0, ..., 0)$, $C_i = (\infty,...,\infty)$ \Comment{Initial mean and confidence interval for each arm}
% \While{{\bf true}}
\While{$|\arms| > 1$} % and $C_y > 0$ for some arm $y$}
        \ForAll{arms $x$ with $T_x \geq n$} 
            \State Set $\hat L_x = \frac1n \sum_{j = 1}^n L_{x}(x_j)$ and $C_x = 0$
            \Comment Arm return is computed exactly
        % \State Compute $\sum_{j = 1}^N \Delta L_{x_i}(x_j)$ exactly \Comment Over all datapoints
        % \State Set $B_i = M_i = U_i = \sum_{j = 1}^N \Delta L_{x_i}(x_j)$ \Comment Arm return is known exactly
        \EndFor
        \State Draw a random sample (with replacement) of $\batchsize$ reference points $\X_{\rm ref} \subset \X$ 
        \ForAll{arms $x$ with $T_x < n$}
            \State $\hat L_x \leftarrow \frac{ T_x \hat L_x + \sum_{\X_{\rm ref}}L_{x}(x_{\rm ref})}{T_x + \batchsize }$ \Comment{Update running average}
            \State $T_x \leftarrow T_x + \batchsize$
            \State $C_x \gets \sigma_x \sqrt{  \frac{ 2 \log(\frac{1}{\delta}) } {T_x}}$
            \Comment{Update confidence interval}        
        % \State $M_i \leftarrow \frac{ T_iM_i + \sum_{x_{\rm ref}}\Delta L_{x_i}(x_{\rm ref})}{T_i + batch\_size}$ \Comment{Update running average}
        % \State $T_i \leftarrow T_i + batch\_size$
        % \State $C_i \leftarrow \sigma_i \sqrt{ \frac{ \log(\frac{1}{\delta}) } {T_i}}$
        % \State $B_i \leftarrow M_i - C_i$, $U_i \leftarrow M_i + C_i$ \Comment{Update confidence interval}
        \EndFor
    % \State $\arms \leftarrow \{i : B_i \leq \min_i(U_i)\}$ \Comment{Arms to pull must overlap with lowest CI}
    \State $\arms \leftarrow \{x : \hat L_x - C_x \leq \min_{y}(\hat L_{y} + C_{y})\}$ \Comment{Remove arms that can no longer be chosen}
\EndWhile
% \State Append $x_i$ to $\mathcal{M}$, where $i = \argmin_iB_i$
% \State \textbf{return} $\mathcal{M}$
\State \textbf{return} $x \in \arms$
\end{algorithmic}
\end{algorithm}




\begin{algorithm}[t]
\caption{\texttt{\algname BUILD($\X, \mathcal{M} = \{m_1, \cdots, m_{l-1}\}, \delta$):} 
%\Comment{Dataset $X$ of size $N$, number of medoids $k_{max}$, distance function $d$} 
\label{alg:build-step}}
\begin{algorithmic}[1]
\State $\arms \leftarrow \X - \M$
\State $T \leftarrow (0, ..., 0)$ \Comment{Number of times each arm has been pulled}
\State $\hat L = (0, ..., 0)$, $C_i = (\infty,...,\infty)$ \Comment{Initial mean and confidence interval for each arm}
% \While{{\bf true}}
\While{$|\arms| > 1$ and $C_y > 0$ for some arm $y$}
    \State Choose arm $x = \argmin_{y \in \arms} \hat L_y - C_y$
    \If{$T_x = n$}
        % \State Compute $L_{x}(x_j)$ for all $x_j \in \X$ \Comment Over all datapoints
        \State Set $\hat L_x = \frac1n \sum_{j = 1}^n L_{x}(x_j)$ and $C_x = 0$
        \Comment Arm return is computed exactly
    \Else    
        \State Draw a reference point $x_{\rm ref}$ uniformly at random from $\X$  
        \State $\hat L_x \leftarrow \frac{ T_x \hat L_x + L_{x}(x_{\rm ref})}{T_x + 1 }$ \Comment{Update running average}
        \State $T_x \leftarrow T_x + 1$
        \State $C_x \gets \sigma_x \sqrt{  \frac{ 2 \log(\frac{1}{\delta}) } {T_x}}$
        \Comment{Update confidence interval}
    \EndIf
\State $\arms \leftarrow \{x : \hat L_x - C_x \leq \min_{y}(\hat L_{y} + C_{y})\}$ \Comment{Remove arms that can no longer be chosen}
\EndWhile
% \State Append $x_i$ to $\mathcal{M}$, where $i = \argmin_iB_i$
% \State \textbf{return} $\mathcal{M}$
\State \textbf{return} $x \in \arms$
\end{algorithmic}
\end{algorithm}




\ilan{One issue is that current Algorithm 1 tries to learn $\sigma_x$, but we don't want to have to analyze that. 
Algorithm 3 corresponds to a single build step.
We may want to move the longer ``actual'' algorithm to the appendix.
Maybe we should combine BUILD and SWAP steps into the same algorithm? We can then remark that BUILD is a SWAP step where some of the medoids is set to infinity.}



In order to provide a guarantee on the number of distance computations required to identify the $l$th medoid, we let $\Delta_x = \bar L_x - \bar L_{\tilde m_\ell}$.
Moreover, we assume that the random variable $Y = L_x(x_J)$ is $\sigma$-sub-Gaussian; i.e., that $\Pr(|Y-E[Y]| > t) < 2 \exp\left(-t^2/(2 \sigma^2)\right)$.
Notice that, strictly speaking, $Y = L_x(x_J)$ only takes value in a finite set and must be $\sigma$-sub-Gaussian for some $\sigma$.
As we illustrate in Section~\ref{sec:experiments}, in practice $\sigma$ can be estimated from the data.
We also point out that $\sigma$ will be different for different arms (i.e., each candidate new medoid $x$) and will depend on which BUILD step we are in.
We then have the following guarantee.


\begin{theorem}
For $\delta = n^{-3}$, with probability at least $1-2/n$, Algorithm~\ref{alg:build-step} chooses the same $l$th medoid as PAM using a total of $N$ distance computations, where
\aln{
N \leq \sum_{x \in \X} \min \left( \frac{ 24 \sigma_x^2}{\Delta_x^2} \log n , 2n \right).
}
\end{theorem}


\begin{proof}
% Algorithm~\ref{alg:build-step} proceeds by reducing the confidence interval of each arm $x$ until $\hat L_x - C_x > \min_{y}(\hat L_{y} + C_{y})\}$.
Notice that, if more than $n$ distance computations are performed for a given arm $x$, the algorithm abandons the current estimate $\hat L_x$ and computes $\bar L_x$ exactly (which requires additional $n$ computations), setting $C_x = 0$.
This guarantees that the algorithm must terminate.
At the end, for arm $x$, the total number of distance computations will be either $T_x \leq n$ or $2n$. % if $T_x = n$.

First, we show that, with probability $1-1/n$, all confidence intervals computed throughout the algorithm are true confidence intervals.
To see this, notice that for a fixed $x$ and a fixed iteration of the algorithm, $\hat L_x$ is the average of $T_x$ i.i.d.~samples of a $\sigma_x$-sub-Gaussian distribution.
From Hoeffding's inequality, 
\aln{
\Pr\left( \left| \bar L_x - \hat L_x \right| > C_x \right) \leq 2 \exp \left({-\frac{T_x C_x^2}{2\sigma_x^2}}\right)  = 2 \delta.
% \\
% \sigma_x \sqrt{ \frac{2 \log(\frac{1}{\delta}) } {T_x}}
}
Since there are at most $n^2$ such confidence intervals computed across all arms and all steps of the algorithm, 
for $\delta = 1/n^3$, we see that $\bar L_x \in [\hat L_x - C_x, \hat L_x + C_x]$ for every $x$ and for every step of the algorithm with probability at least $1-2/n$.

Let $x^* = \argmin_{x \in \arms} \bar L_x$.
Notice that if all confidence intervals throughout the algorithm are correct, it is impossible for $x^*$ to be removed from the set of candidate arms, and $x^*$ (or some $y$ with $\bar L_y = \bar L_{x^*}$) must be returned at the end.
Now consider another arm $x \ne x^*$ for which $T_x \leq n$ at the end of the algorithm.
At the last iteration in which arm $x$ was pulled, we must have had 
\aln{
\hat L_x - C_x \leq \hat L_{x^*} - C_{x^*} \leq \bar L_{x^*}.
}
Moreover, since $\bar L_x \leq \hat L_x + C_x$, we have that
\aln{
\Delta_x = \bar L_x - \bar L_{x^*} \leq (\hat L_x + C_x) - (\hat L_x - C_x) = 2 C_x = 
\sqrt{  \frac{ 8 \sigma_x^2 \log(n^3) } {T_x}} = 
\sqrt{  \frac{ 24 \sigma_x^2 \log n } {T_x}} ,
}
which implies that $T_x \leq \frac{ 24 \sigma_x^2 } {\Delta_x^2} \log n$.
This implies the theorem.
\end{proof}



--- OLD STUFF FROM PROBLEM FORMULATION FOR REFERENCE

In the BUILD step, each of the medoids is greedily initialized by choosing the $l$th medoid, conditioned on the previous $l-1$ medoids, that reduces the total loss of every other point. 
\ilan{}
More formally, suppose the current set of medoids is $\mathcal{M} = \{m_1, \cdots, m_{l-1}\}$ and we wish to add the $l$th medoid $m_l$. Our goal is to identify a new medoid $m_l$ such that:

\begin{equation}
\label{eqn:build-next-medoid}
    m_l = \argmin_{x \in \mathcal{X} \setminus \mathcal{M}} \sum_{j=1}^n \min[d(x, x_j), \min_{m' \in \mathcal{M}} d(m', x_j)]. 
\end{equation}

Equivalently, we can find the find $m_l$ that minimizes the change in total loss:

\begin{equation}
\label{eqn:build-next-medoid-td}
    m_l = \argmin_{x \in \mathcal{X} \setminus \mathcal{M}} \sum_{j=1}^n   L_{x}(x_j)
\end{equation}

where

\begin{equation}
\label{eqn:build-td}
    L_{x}(x_j) = \min[d(x, x_j) - \min_{m' \in \mathcal{M}} d(m', x_j), 0]
\end{equation}





--- OLD STUFF



\noindent {\bf Assumptions:} 
Similar to the work by Bagaria et al.~\cite{bagaria2018medoids}, which focuses on the computation of a single medoid, we need an assumption regarding the distribution of pairwise distances.
We assume that the $n$ data points belong to true clusters $\Ct_1, \Ct_2, ..., \Ct_k$ \ilan{different $k$?}.
For a pair of points $x_1$ and $x_2$, their distance $d(x_1,x_2)$ is assumed to be a $\sigma_{\rm in}$-sub-Gaussian random variable if $x_1$ and $x_2$ are in the same true cluster, while it is a a $\sigma_{\rm out}$-sub-Gaussian random variable if $x_1$ and $x_2$ are in different clusters, for $\sigma_{\rm in} < \sigma_{\rm out}$.
The true clusters $\Ct_1, \Ct_2, ..., \Ct_k$ and the parameters $\sigma_{\rm in}$ and $\sigma_{\rm out}$ are not known a priori.
\ilan{maybe a single $\sigma$ is ok}

% \ilan{we may have to be a bit careful with whether $\sigma$ is known for the theoretical results}

% \ilan{one theorem for BUILD and one for SWAP? Or one for equality with PAM and one for number of distance computations?}



% \ilan{Maybe the best approach will be to assume, for the theory, part that all distances have a bounded support, like $[0,1]$. But then the adaptive $\sigma$ doesn't make sense...}




\martin{State and discuss all assumptions first before stating the theorems.}

In this section, we provide theoretical guarantees for when the UltraPAM algorithm will return the same results as PAM. 

Intuitively, in the BUILD step we reduce the problem of finding the best new medoid amongst all candidates to a best-arm identification problem. In this analogy, the contribution of a reference point $x_{ref}$ to the total loss \ref{TotalLoss} if we were to add candidate $x_c$ as a medoid corresponds to a reward from pulling the arm labeled $x_c$. With high probability, UltraPAM's BUILD step then returns the same initialized medoids as PAM. We formalize this in Theorem 1.

\paragraph{Theorem 1:} Given a finite, bounded dataset $D$. Suppose that given any $\mathcal{M}$, the minimizer of Equation \ref{build-next-medoid} is unique and that for each $x_i$, $\Delta TD_{x_i}$ (as defined in Equation \ref{build-TD}) is a $\sigma$-sub-Gaussian random variable. Then Algorithm 1 terminates in $O(kNlogN)$ calls to the distance metric $d$ and returns the same results as PAM with probability at least $1 - kN\delta$.

\paragraph{Proof of Theorem 1:} The proof is a relatively straightforward adaptation of the proof for best-arm-identification algorithms and is provided in the Appendix.

In the SWAP step, we again reduce the problem of finding the best medoid-nonmedoid pair $(x_m, x_o)$ to a a best-arm identification problem. In this analogy, the contribution of a reference point $x_{ref}$ to the total loss \ref{TotalLoss} if we were to swap medoid $x_m$ with non-medoid $x_o$ corresponds to a reward from pulling the arm labeled by the pair $(x_m, x_o)$. With high probability, UltraPAM then swaps the same medoid-nonmedoid pair that PAM would. We formalize this in Theorem 2.

\paragraph{Theorem 2:} Given a finite, bounded dataset $D$ and initial set of medoids $\mathcal{M'}$, where $|\mathcal{M}| = k$. Suppose that given any $\mathcal{M}$, the minimizer of Equation 6 is unique and that for each pair $(x_m, x_o)$, $\Delta TD_{(x_m, x_o)}$ (as defined in Equation 7) is a $\sigma$-sub-Gaussian random variable. Then Algorithm 2 terminates in $O(kNlogN)$ calls to the distance metric $d$ and returns the same results as PAM with probability at least $1 - kN\delta$.

\paragraph{Proof of Theorem 2:} Similar to the proof of Theorem 1, the proof of Theorem 2 is a relatively straightforward adaptation of the proof for best-arm-identification algorithms and is provided in the Appendix.

We note that the assumptions of Theorems 1 and 2 are unnecessarily strong and can probably be relaxed; we discuss these relaxations in the Future Work and Appendix sections.

\paragraph{Corollary 1:} Let $T$ be the number of SWAP steps performed by the PAM algorithm. With probability at least $1 - (T+1)kN\delta$, the entire UltraPAM algorithm returns the same result as PAM.

\paragraph{Proof of Corollary 1:} From Theorem 1, the probability of UltraPAM and PAM disagreeing in the BUILD step is at most $kN\delta$. Similarly, from Theorem 2, the probability of UltraPAM and PAM disagreeing in each SWAP step is also at most $kN\delta$. Note that if UltraPAM takes more than $T$ SWAP steps to complete, then UltraPAM disagreed with PAM in either the BUILD step or one of the first $T$ SWAP steps. The result then follows by a union bound over the probabilities of error in the BUILD step or any of the first $T$ SWAP steps.

The above results provide conditions under which UltraPAM returns the same results as PAM with high probability. In practice, the authors observe that $T$ is usually very small and almost always smaller than $k$. If necessary, a maximum on the number of SWAP steps or similar early stopping criteria can be specified (such as required decrease in total loss per swap step), as is often the case in practice with iterative algorithms.
